HAT-P-34b -- HAT-P-37b: Four Transiting Planets More Massive Than Jupiter Orbiting Moderately Bright Stars

We report the discovery of four transiting extrasolar planets (HAT-P-34b - HAT-P-37b) with masses ranging from 1.05 to 3.33 MJ and periods from 1.33 to 5.45 days. These planets orbit relatively bright F and G dwarf stars (from V = 10.16 to V = 13.2). Of particular interest is HAT-P-34b which is moderately massive (3.33 MJ), has a high eccentricity of e = 0.441 +/- 0.032 at P = 5.4526540+/-0.000016 d period, and shows hints of an outer component. The other three planets have properties that are typical of hot Jupiters.

==> Makefile <==
TARGET=hatp34-37_V09
PRINTER=peyton_ps

all: $(TARGET).pdf

SUB=submit_v1

.PHONY: all clean save print

$(TARGET).dvi: *.tex *.cls
	latex $(TARGET).tex
	latex $(TARGET).tex
	latex $(TARGET).tex

$(TARGET).ps: $(TARGET).dvi
	dvips -t letter $(TARGET).dvi -o

$(TARGET).pdf: $(TARGET).ps
	ps2pdf $< $@

save:
	tar cvf $(TARGET).tar *
	gzip $(TARGET).tar
	mv $(TARGET).tar.gz $(TARGET).tgz

sub:
	test -d $(SUB) || mkdir $(SUB)
	test -d $(SUB)/img || mkdir $(SUB)/img
	cp $(TARGET).tex $(SUB)/hatpxx.tex
	cp img/*.eps $(SUB)/img

clean:
	rm -f *.ps *.dvi *.aux *.log *.pdf \
        $(TARGET).idx $(TARGET).inx $(TARGET).toc $(TARGET).tgz 

print: $(TARGET).ps
	lpr -P$(PRINTER) $<
	


==> data/HTR114-005_phfu_tab.tex <==
$ 55616.96855 $ & $   0.02527 $ & $   0.00133 $ & $  12.41350 $ & $ i$\\
$ 55616.97081 $ & $   0.02387 $ & $   0.00135 $ & $  12.41200 $ & $ i$\\
$ 55616.97308 $ & $   0.02220 $ & $   0.00133 $ & $  12.41020 $ & $ i$\\
$ 55616.97540 $ & $   0.02311 $ & $   0.00131 $ & $  12.41290 $ & $ i$\\
$ 55616.97774 $ & $   0.02297 $ & $   0.00132 $ & $  12.41110 $ & $ i$\\
$ 55616.97986 $ & $   0.02149 $ & $   0.00133 $ & $  12.40940 $ & $ i$\\
$ 55616.98176 $ & $   0.02186 $ & $   0.00133 $ & $  12.40980 $ & $ i$\\
$ 55616.98366 $ & $   0.01909 $ & $   0.00131 $ & $  12.40740 $ & $ i$\\
$ 55616.98555 $ & $   0.02301 $ & $   0.00132 $ & $  12.41180 $ & $ i$\\
$ 55616.98744 $ & $   0.02165 $ & $   0.00129 $ & $  12.40910 $ & $ i$\\
$ 55616.98933 $ & $   0.02058 $ & $   0.00130 $ & $  12.40830 $ & $ i$\\
$ 55616.99125 $ & $   0.02047 $ & $   0.00131 $ & $  12.40830 $ & $ i$\\
$ 55616.99315 $ & $   0.01888 $ & $   0.00129 $ & $  12.40710 $ & $ i$\\
$ 55616.99503 $ & $   0.02211 $ & $   0.00130 $ & $  12.41140 $ & $ i$\\
$ 55616.99693 $ & $   0.02249 $ & $   0.00128 $ & $  12.41160 $ & $ i$\\
$ 55616.99884 $ & $   0.02099 $ & $   0.00126 $ & $  12.40860 $ & $ i$\\
$ 55617.00074 $ & $   0.01727 $ & $   0.00128 $ & $  12.40550 $ & $ i$\\
$ 55617.00265 $ & $   0.01190 $ & $   0.00127 $ & $  12.39970 $ & $ i$\\
$ 55617.00456 $ & $   0.01252 $ & $   0.00127 $ & $  12.40170 $ & $ i$\\
$ 55617.00645 $ & $   0.01024 $ & $   0.00128 $ & $  12.39830 $ & $ i$\\
$ 55617.00837 $ & $   0.00780 $ & $   0.00127 $ & $  12.39450 $ & $ i$\\
$ 55617.01025 $ & $   0.00310 $ & $   0.00127 $ & $  12.39050 $ & $ i$\\
$ 55617.01214 $ & $   0.00178 $ & $   0.00127 $ & $  12.39020 $ & $ i$\\
$ 55617.01405 $ & $   0.00030 $ & $   0.00127 $ & $  12.38850 $ & $ i$\\
$ 55617.01595 $ & $  -0.00268 $ & $   0.00125 $ & $  12.38540 $ & $ i$\\
$ 55617.01786 $ & $   0.00297 $ & $   0.00125 $ & $  12.39200 $ & $ i$\\
$ 55617.01977 $ & $  -0.00140 $ & $   0.00126 $ & $  12.38720 $ & $ i$\\
$ 55617.02167 $ & $  -0.00157 $ & $   0.00126 $ & $  12.38730 $ & $ i$\\
$ 55617.02356 $ & $   0.00043 $ & $   0.00125 $ & $  12.38860 $ & $ i$\\
$ 55617.02547 $ & $  -0.00215 $ & $   0.00127 $ & $  12.38650 $ & $ i$\\
$ 55617.02736 $ & $   0.00039 $ & $   0.00126 $ & $  12.38940 $ & $ i$\\
$ 55617.02925 $ & $   0.00075 $ & $   0.00127 $ & $  12.38910 $ & $ i$\\
$ 55617.03116 $ & $   0.00147 $ & $   0.00127 $ & $  12.39010 $ & $ i$\\
$ 55617.03303 $ & $   0.00118 $ & $   0.00130 $ & $  12.39060 $ & $ i$\\
$ 55617.03494 $ & $   0.00080 $ & $   0.00130 $ & $  12.38900 $ & $ i$\\
$ 55617.03685 $ & $   0.00040 $ & $   0.00130 $ & $  12.38950 $ & $ i$\\
$ 55617.03874 $ & $  -0.00263 $ & $   0.00134 $ & $  12.38690 $ & $ i$\\
$ 55644.89591 $ & $   0.00363 $ & $   0.00146 $ & $  12.40580 $ & $ i$\\
$ 55644.89747 $ & $   0.00298 $ & $   0.00150 $ & $  12.40500 $ & $ i$\\
$ 55644.89901 $ & $   0.00788 $ & $   0.00147 $ & $  12.40980 $ & $ i$\\
$ 55644.90066 $ & $   0.00804 $ & $   0.00146 $ & $  12.41050 $ & $ i$\\
$ 55644.90221 $ & $   0.01111 $ & $   0.00146 $ & $  12.41460 $ & $ i$\\
$ 55644.90378 $ & $   0.01589 $ & $   0.00147 $ & $  12.42020 $ & $ i$\\
$ 55644.90531 $ & $   0.01694 $ & $   0.00149 $ & $  12.42120 $ & $ i$\\
$ 55644.90688 $ & $   0.01893 $ & $   0.00148 $ & $  12.42270 $ & $ i$\\
$ 55644.90844 $ & $   0.01856 $ & $   0.00146 $ & $  12.42220 $ & $ i$\\
$ 55644.90999 $ & $   0.01815 $ & $   0.00146 $ & $  12.42140 $ & $ i$\\
$ 55644.91153 $ & $   0.01795 $ & $   0.00144 $ & $  12.42180 $ & $ i$\\
$ 55644.91308 $ & $   0.02085 $ & $   0.00145 $ & $  12.42450 $ & $ i$\\
$ 55644.91466 $ & $   0.02175 $ & $   0.00144 $ & $  12.42620 $ & $ i$\\
$ 55644.91622 $ & $   0.02086 $ & $   0.00145 $ & $  12.42450 $ & $ i$\\
$ 55644.91777 $ & $   0.02084 $ & $   0.00146 $ & $  12.42390 $ & $ i$\\
$ 55644.91933 $ & $   0.02226 $ & $   0.00143 $ & $  12.42650 $ & $ i$\\
$ 55644.92088 $ & $   0.02318 $ & $   0.00147 $ & $  12.42700 $ & $ i$\\
$ 55644.92243 $ & $   0.02212 $ & $   0.00147 $ & $  12.42630 $ & $ i$\\
$ 55644.92395 $ & $   0.02135 $ & $   0.00148 $ & $  12.42520 $ & $ i$\\
$ 55644.92550 $ & $   0.02337 $ & $   0.00147 $ & $  12.42830 $ & $ i$\\
$ 55644.92712 $ & $   0.02245 $ & $   0.00145 $ & $  12.42620 $ & $ i$\\
$ 55644.92868 $ & $   0.02332 $ & $   0.00145 $ & $  12.42840 $ & $ i$\\
$ 55644.93025 $ & $   0.02296 $ & $   0.00145 $ & $  12.42810 $ & $ i$\\
$ 55644.93180 $ & $   0.02221 $ & $   0.00143 $ & $  12.42690 $ & $ i$\\
$ 55644.93333 $ & $   0.02176 $ & $   0.00144 $ & $  12.42760 $ & $ i$\\
$ 55644.93486 $ & $   0.02416 $ & $   0.00144 $ & $  12.42990 $ & $ i$\\
$ 55644.93640 $ & $   0.02348 $ & $   0.00144 $ & $  12.43020 $ & $ i$\\
$ 55644.93795 $ & $   0.02282 $ & $   0.00145 $ & $  12.42680 $ & $ i$\\
$ 55644.93949 $ & $   0.02368 $ & $   0.00143 $ & $  12.42920 $ & $ i$\\
$ 55644.94106 $ & $   0.02387 $ & $   0.00144 $ & $  12.42950 $ & $ i$\\
$ 55644.94262 $ & $   0.02356 $ & $   0.00144 $ & $  12.42930 $ & $ i$\\
$ 55644.94416 $ & $   0.02277 $ & $   0.00145 $ & $  12.42930 $ & $ i$\\
$ 55644.94571 $ & $   0.02316 $ & $   0.00143 $ & $  12.42880 $ & $ i$\\
$ 55644.94726 $ & $   0.02201 $ & $   0.00142 $ & $  12.42820 $ & $ i$\\
$ 55644.94882 $ & $   0.02147 $ & $   0.00145 $ & $  12.42810 $ & $ i$\\
$ 55644.95037 $ & $   0.02346 $ & $   0.00144 $ & $  12.42890 $ & $ i$\\
$ 55644.95192 $ & $   0.02285 $ & $   0.00143 $ & $  12.42890 $ & $ i$\\
$ 55644.95348 $ & $   0.02315 $ & $   0.00145 $ & $  12.42900 $ & $ i$\\
$ 55644.95501 $ & $   0.02401 $ & $   0.00143 $ & $  12.43000 $ & $ i$\\
$ 55644.95657 $ & $   0.02090 $ & $   0.00144 $ & $  12.42640 $ & $ i$\\
$ 55644.95903 $ & $   0.02485 $ & $   0.00145 $ & $  12.43240 $ & $ i$\\
$ 55644.96058 $ & $   0.02384 $ & $   0.00145 $ & $  12.43050 $ & $ i$\\
$ 55644.96211 $ & $   0.02171 $ & $   0.00143 $ & $  12.42770 $ & $ i$\\
$ 55644.96366 $ & $   0.01883 $ & $   0.00142 $ & $  12.42530 $ & $ i$\\
$ 55644.96521 $ & $   0.02089 $ & $   0.00142 $ & $  12.42670 $ & $ i$\\
$ 55644.96676 $ & $   0.01950 $ & $   0.00143 $ & $  12.42550 $ & $ i$\\
$ 55644.96828 $ & $   0.02102 $ & $   0.00142 $ & $  12.42780 $ & $ i$\\
$ 55644.96985 $ & $   0.02111 $ & $   0.00142 $ & $  12.42730 $ & $ i$\\
$ 55644.97142 $ & $   0.02035 $ & $   0.00142 $ & $  12.42760 $ & $ i$\\
$ 55644.97294 $ & $   0.01940 $ & $   0.00142 $ & $  12.42590 $ & $ i$\\
$ 55644.97449 $ & $   0.01686 $ & $   0.00141 $ & $  12.42380 $ & $ i$\\
$ 55644.97605 $ & $   0.01545 $ & $   0.00140 $ & $  12.42270 $ & $ i$\\
$ 55644.97760 $ & $   0.01335 $ & $   0.00140 $ & $  12.42250 $ & $ i$\\
$ 55644.97914 $ & $   0.01243 $ & $   0.00140 $ & $  12.41960 $ & $ i$\\
$ 55644.98070 $ & $   0.00935 $ & $   0.00139 $ & $  12.41650 $ & $ i$\\
$ 55644.98226 $ & $   0.00637 $ & $   0.00138 $ & $  12.41370 $ & $ i$\\
$ 55644.98380 $ & $   0.00349 $ & $   0.00137 $ & $  12.41010 $ & $ i$\\
$ 55644.98535 $ & $   0.00506 $ & $   0.00137 $ & $  12.41240 $ & $ i$\\
$ 55644.98690 $ & $   0.00103 $ & $   0.00138 $ & $  12.40890 $ & $ i$\\
$ 55644.98845 $ & $   0.00116 $ & $   0.00138 $ & $  12.40910 $ & $ i$\\
$ 55644.99269 $ & $  -0.00273 $ & $   0.00139 $ & $  12.40500 $ & $ i$\\
$ 55644.99424 $ & $   0.00028 $ & $   0.00138 $ & $  12.40880 $ & $ i$\\
$ 55644.99579 $ & $   0.00044 $ & $   0.00139 $ & $  12.40800 $ & $ i$\\
$ 55644.99731 $ & $   0.00272 $ & $   0.00138 $ & $  12.40950 $ & $ i$\\
$ 55644.99887 $ & $   0.00015 $ & $   0.00138 $ & $  12.40780 $ & $ i$\\
$ 55645.00043 $ & $  -0.00332 $ & $   0.00138 $ & $  12.40410 $ & $ i$\\
$ 55645.00197 $ & $   0.00028 $ & $   0.00138 $ & $  12.40720 $ & $ i$\\
$ 55645.00351 $ & $  -0.00058 $ & $   0.00137 $ & $  12.40680 $ & $ i$\\
$ 55645.00534 $ & $   0.00230 $ & $   0.00137 $ & $  12.41040 $ & $ i$\\
$ 55645.00697 $ & $  -0.00113 $ & $   0.00138 $ & $  12.40620 $ & $ i$\\
$ 55645.00879 $ & $   0.00120 $ & $   0.00137 $ & $  12.40750 $ & $ i$\\
$ 55645.01034 $ & $  -0.00047 $ & $   0.00138 $ & $  12.40620 $ & $ i$\\
$ 55645.01189 $ & $  -0.00056 $ & $   0.00138 $ & $  12.40690 $ & $ i$\\
$ 55658.84356 $ & $  -0.00165 $ & $   0.00126 $ & $  12.06430 $ & $ i$\\
$ 55658.84510 $ & $  -0.00440 $ & $   0.00126 $ & $  12.06250 $ & $ i$\\
$ 55658.84665 $ & $  -0.00107 $ & $   0.00125 $ & $  12.06600 $ & $ i$\\
$ 55658.84820 $ & $   0.00190 $ & $   0.00125 $ & $  12.06910 $ & $ i$\\
$ 55658.84975 $ & $   0.00013 $ & $   0.00125 $ & $  12.06730 $ & $ i$\\
$ 55658.85130 $ & $  -0.00095 $ & $   0.00124 $ & $  12.06550 $ & $ i$\\
$ 55658.85284 $ & $  -0.00002 $ & $   0.00123 $ & $  12.06720 $ & $ i$\\
$ 55658.85438 $ & $   0.00145 $ & $   0.00122 $ & $  12.06870 $ & $ i$\\
$ 55658.85593 $ & $   0.00331 $ & $   0.00124 $ & $  12.06980 $ & $ i$\\
$ 55658.85748 $ & $   0.00012 $ & $   0.00123 $ & $  12.06600 $ & $ i$\\
$ 55658.85903 $ & $  -0.00061 $ & $   0.00124 $ & $  12.06740 $ & $ i$\\
$ 55658.86060 $ & $   0.00468 $ & $   0.00123 $ & $  12.07040 $ & $ i$\\
$ 55658.86213 $ & $  -0.00112 $ & $   0.00122 $ & $  12.06590 $ & $ i$\\
$ 55658.86367 $ & $  -0.00085 $ & $   0.00123 $ & $  12.06650 $ & $ i$\\
$ 55658.86522 $ & $  -0.00016 $ & $   0.00122 $ & $  12.06700 $ & $ i$\\
$ 55658.86676 $ & $   0.00158 $ & $   0.00122 $ & $  12.06860 $ & $ i$\\
$ 55658.86830 $ & $   0.00166 $ & $   0.00121 $ & $  12.06720 $ & $ i$\\
$ 55658.86985 $ & $  -0.00179 $ & $   0.00122 $ & $  12.06450 $ & $ i$\\
$ 55658.87139 $ & $   0.00017 $ & $   0.00120 $ & $  12.06680 $ & $ i$\\
$ 55658.87291 $ & $  -0.00068 $ & $   0.00120 $ & $  12.06830 $ & $ i$\\
$ 55658.87462 $ & $  -0.00247 $ & $   0.00121 $ & $  12.06420 $ & $ i$\\
$ 55658.87617 $ & $   0.00011 $ & $   0.00121 $ & $  12.06750 $ & $ i$\\
$ 55658.87773 $ & $   0.00147 $ & $   0.00121 $ & $  12.06730 $ & $ i$\\
$ 55658.87929 $ & $   0.00142 $ & $   0.00120 $ & $  12.06820 $ & $ i$\\
$ 55658.88084 $ & $  -0.00006 $ & $   0.00120 $ & $  12.06740 $ & $ i$\\
$ 55658.88239 $ & $  -0.00013 $ & $   0.00120 $ & $  12.06690 $ & $ i$\\
$ 55658.88393 $ & $   0.00311 $ & $   0.00122 $ & $  12.06970 $ & $ i$\\
$ 55658.88546 $ & $   0.00548 $ & $   0.00120 $ & $  12.07250 $ & $ i$\\
$ 55658.88702 $ & $   0.00762 $ & $   0.00121 $ & $  12.07590 $ & $ i$\\
$ 55658.88857 $ & $   0.01178 $ & $   0.00119 $ & $  12.07990 $ & $ i$\\
$ 55658.89011 $ & $   0.01100 $ & $   0.00120 $ & $  12.07810 $ & $ i$\\
$ 55658.89167 $ & $   0.01526 $ & $   0.00120 $ & $  12.08440 $ & $ i$\\
$ 55658.89324 $ & $   0.01762 $ & $   0.00121 $ & $  12.08560 $ & $ i$\\
$ 55658.89480 $ & $   0.01963 $ & $   0.00121 $ & $  12.08710 $ & $ i$\\
$ 55658.89635 $ & $   0.01857 $ & $   0.00121 $ & $  12.08580 $ & $ i$\\
$ 55658.89789 $ & $   0.01983 $ & $   0.00120 $ & $  12.08760 $ & $ i$\\
$ 55658.89943 $ & $   0.01919 $ & $   0.00121 $ & $  12.08730 $ & $ i$\\
$ 55658.90096 $ & $   0.02305 $ & $   0.00120 $ & $  12.09160 $ & $ i$\\
$ 55658.90252 $ & $   0.02334 $ & $   0.00120 $ & $  12.09110 $ & $ i$\\
$ 55658.90408 $ & $   0.02241 $ & $   0.00120 $ & $  12.09030 $ & $ i$\\
$ 55658.90571 $ & $   0.02151 $ & $   0.00121 $ & $  12.09050 $ & $ i$\\
$ 55658.90724 $ & $   0.01999 $ & $   0.00119 $ & $  12.08860 $ & $ i$\\
$ 55658.90880 $ & $   0.02348 $ & $   0.00121 $ & $  12.09170 $ & $ i$\\
$ 55658.91034 $ & $   0.02420 $ & $   0.00121 $ & $  12.09210 $ & $ i$\\
$ 55658.91188 $ & $   0.02226 $ & $   0.00121 $ & $  12.09020 $ & $ i$\\
$ 55658.91343 $ & $   0.02151 $ & $   0.00120 $ & $  12.08980 $ & $ i$\\
$ 55658.91499 $ & $   0.02239 $ & $   0.00121 $ & $  12.09080 $ & $ i$\\
$ 55658.91653 $ & $   0.01992 $ & $   0.00120 $ & $  12.08780 $ & $ i$\\
$ 55658.91808 $ & $   0.02064 $ & $   0.00121 $ & $  12.08900 $ & $ i$\\
$ 55658.91961 $ & $   0.02124 $ & $   0.00121 $ & $  12.08940 $ & $ i$\\
$ 55658.92116 $ & $   0.02260 $ & $   0.00120 $ & $  12.09100 $ & $ i$\\
$ 55658.92272 $ & $   0.02484 $ & $   0.00121 $ & $  12.09350 $ & $ i$\\
$ 55658.92426 $ & $   0.02448 $ & $   0.00121 $ & $  12.09270 $ & $ i$\\
$ 55658.92580 $ & $   0.02307 $ & $   0.00122 $ & $  12.09090 $ & $ i$\\
$ 55658.92737 $ & $   0.02559 $ & $   0.00123 $ & $  12.09350 $ & $ i$\\
$ 55658.92891 $ & $   0.02596 $ & $   0.00123 $ & $  12.09430 $ & $ i$\\
$ 55658.93044 $ & $   0.02139 $ & $   0.00121 $ & $  12.09000 $ & $ i$\\
$ 55658.93198 $ & $   0.02223 $ & $   0.00121 $ & $  12.08770 $ & $ i$\\
$ 55658.93352 $ & $   0.02395 $ & $   0.00121 $ & $  12.09170 $ & $ i$\\
$ 55658.93510 $ & $   0.02289 $ & $   0.00121 $ & $  12.09220 $ & $ i$\\
$ 55658.93669 $ & $   0.02328 $ & $   0.00122 $ & $  12.09320 $ & $ i$\\
$ 55658.93823 $ & $   0.02090 $ & $   0.00120 $ & $  12.08960 $ & $ i$\\
$ 55658.93978 $ & $   0.02325 $ & $   0.00121 $ & $  12.09220 $ & $ i$\\
$ 55658.94131 $ & $   0.02474 $ & $   0.00121 $ & $  12.09380 $ & $ i$\\
$ 55658.94288 $ & $   0.02163 $ & $   0.00121 $ & $  12.08980 $ & $ i$\\
$ 55658.94444 $ & $   0.02421 $ & $   0.00121 $ & $  12.09320 $ & $ i$\\
$ 55658.94601 $ & $   0.02115 $ & $   0.00120 $ & $  12.08980 $ & $ i$\\
$ 55658.94755 $ & $   0.02169 $ & $   0.00122 $ & $  12.09030 $ & $ i$\\
$ 55658.94909 $ & $   0.01987 $ & $   0.00120 $ & $  12.08810 $ & $ i$\\
$ 55658.95065 $ & $   0.02121 $ & $   0.00120 $ & $  12.08870 $ & $ i$\\
$ 55658.95218 $ & $   0.02060 $ & $   0.00120 $ & $  12.08870 $ & $ i$\\
$ 55658.95373 $ & $   0.01968 $ & $   0.00121 $ & $  12.08770 $ & $ i$\\
$ 55658.95528 $ & $   0.02413 $ & $   0.00122 $ & $  12.09070 $ & $ i$\\
$ 55658.95683 $ & $   0.01989 $ & $   0.00122 $ & $  12.08750 $ & $ i$\\
$ 55658.95839 $ & $   0.01770 $ & $   0.00121 $ & $  12.08510 $ & $ i$\\
$ 55658.95992 $ & $   0.02110 $ & $   0.00121 $ & $  12.08820 $ & $ i$\\
$ 55658.96151 $ & $   0.01785 $ & $   0.00121 $ & $  12.08570 $ & $ i$\\
$ 55658.96305 $ & $   0.01462 $ & $   0.00120 $ & $  12.08290 $ & $ i$\\
$ 55658.96458 $ & $   0.01454 $ & $   0.00120 $ & $  12.08250 $ & $ i$\\
$ 55658.96614 $ & $   0.01295 $ & $   0.00122 $ & $  12.08070 $ & $ i$\\
$ 55658.96774 $ & $   0.00925 $ & $   0.00119 $ & $  12.07760 $ & $ i$\\
$ 55658.96929 $ & $   0.00945 $ & $   0.00120 $ & $  12.07730 $ & $ i$\\
$ 55658.97083 $ & $   0.00543 $ & $   0.00121 $ & $  12.07380 $ & $ i$\\
$ 55658.97237 $ & $   0.00018 $ & $   0.00120 $ & $  12.06810 $ & $ i$\\
$ 55658.97393 $ & $  -0.00215 $ & $   0.00120 $ & $  12.06550 $ & $ i$\\
$ 55658.97548 $ & $   0.00122 $ & $   0.00120 $ & $  12.06880 $ & $ i$\\
$ 55658.97704 $ & $  -0.00015 $ & $   0.00120 $ & $  12.06680 $ & $ i$\\
$ 55658.97858 $ & $  -0.00181 $ & $   0.00119 $ & $  12.06550 $ & $ i$\\
$ 55658.98012 $ & $  -0.00035 $ & $   0.00119 $ & $  12.06690 $ & $ i$\\
$ 55658.98168 $ & $  -0.00038 $ & $   0.00120 $ & $  12.06830 $ & $ i$\\
$ 55658.98324 $ & $  -0.00116 $ & $   0.00120 $ & $  12.06560 $ & $ i$\\
$ 55658.98479 $ & $   0.00400 $ & $   0.00121 $ & $  12.07080 $ & $ i$\\
$ 55658.98631 $ & $  -0.00107 $ & $   0.00121 $ & $  12.06660 $ & $ i$\\
$ 55658.98786 $ & $   0.00094 $ & $   0.00121 $ & $  12.06830 $ & $ i$\\
$ 55658.98942 $ & $   0.00028 $ & $   0.00120 $ & $  12.06860 $ & $ i$\\
$ 55658.99098 $ & $  -0.00245 $ & $   0.00122 $ & $  12.06480 $ & $ i$\\
$ 55658.99251 $ & $   0.00085 $ & $   0.00121 $ & $  12.06720 $ & $ i$\\
$ 55658.99406 $ & $  -0.00165 $ & $   0.00121 $ & $  12.06570 $ & $ i$\\
$ 55658.99562 $ & $  -0.00048 $ & $   0.00120 $ & $  12.06660 $ & $ i$\\
$ 55658.99716 $ & $   0.00397 $ & $   0.00122 $ & $  12.07070 $ & $ i$\\
$ 55658.99873 $ & $   0.00129 $ & $   0.00121 $ & $  12.06900 $ & $ i$\\
$ 55659.00028 $ & $  -0.00040 $ & $   0.00123 $ & $  12.06610 $ & $ i$\\


==> data/HTR114-005_phfu_tab_short.tex <==
$ 55616.96855 $ & $   0.02527 $ & $   0.00133 $ & $  12.41350 $ & $ i$\\
$ 55616.97081 $ & $   0.02387 $ & $   0.00135 $ & $  12.41200 $ & $ i$\\
$ 55616.97308 $ & $   0.02220 $ & $   0.00133 $ & $  12.41020 $ & $ i$\\
$ 55616.97540 $ & $   0.02311 $ & $   0.00131 $ & $  12.41290 $ & $ i$\\
$ 55616.97774 $ & $   0.02297 $ & $   0.00132 $ & $  12.41110 $ & $ i$\\
$ 55616.97986 $ & $   0.02149 $ & $   0.00133 $ & $  12.40940 $ & $ i$\\
$ 55616.98176 $ & $   0.02186 $ & $   0.00133 $ & $  12.40980 $ & $ i$\\
$ 55616.98366 $ & $   0.01909 $ & $   0.00131 $ & $  12.40740 $ & $ i$\\
$ 55616.98555 $ & $   0.02301 $ & $   0.00132 $ & $  12.41180 $ & $ i$\\
$ 55616.98744 $ & $   0.02165 $ & $   0.00129 $ & $  12.40910 $ & $ i$\\


==> data/HTR114-005_rvtable.tex <==
$ 1646.92799 $ & $   146.43 $ & $    35.50 $ & $    26.20 $ & $    16.30 $ & $   0.710 $\\
$ 1648.01278 $ & $  -111.17 $ & $    24.60 $ & $   -28.00 $ & $    16.30 $ & $   0.098 $\\
$ 1648.91342 $ & $   -88.77 $ & $    23.20 $ & $     0.60 $ & $    22.20 $ & $   0.420 $\\
$ 1649.89870 $ & $   172.53 $ & $    29.40 $ & $     8.30 $ & $    24.10 $ & $   0.772 $\\
$ 1650.96241 $ & $  -102.97 $ & $    17.50 $ & $    12.30 $ & $    16.90 $ & $   0.153 $\\
$ 1652.92638 $ & $   128.33 $ & $    26.30 $ & $   -13.70 $ & $    15.00 $ & $   0.855 $\\
$ 1656.98738 $ & $  -238.57 $ & $    12.80 $ & $   -28.70 $ & $    23.90 $ & $   0.306 $\\
$ 1658.96338 $ & $   -19.87 $ & $    20.90 $ & $    -9.00 $ & $    17.00 $ & $   0.013 $\\
$ 1663.90569 $ & $   169.23 $ & $    20.60 $ & $    -5.60 $ & $    15.10 $ & $   0.779 $\\
$ 1664.91140 $ & $  -163.77 $ & $    25.40 $ & $   -28.30 $ & $    19.50 $ & $   0.139 $\\
$ 1665.91961 $ & $    62.93 $ & $    32.60 $ & $   -29.50 $ & $    16.80 $ & $   0.499 $\\
$ 1671.84933 $ & $   125.23 $ & $    35.30 $ & $    47.40 $ & $    27.20 $ & $   0.619 $\\
$ 1698.79464 $ & $  -143.97 $ & $    25.00 $ & $    48.00 $ & $    16.20 $ & $   0.251 $\\


==> data/HTR143-001_phfu_tab.tex <==
$ 55555.84870 $ & $   0.00224 $ & $   0.00081 $ & $  10.95490 $ & $ i$\\
$ 55555.85050 $ & $   0.00850 $ & $   0.00083 $ & $  10.96050 $ & $ i$\\
$ 55555.85205 $ & $   0.00708 $ & $   0.00078 $ & $  10.96100 $ & $ i$\\
$ 55555.85362 $ & $   0.01319 $ & $   0.00079 $ & $  10.96370 $ & $ i$\\
$ 55555.85516 $ & $   0.01106 $ & $   0.00079 $ & $  10.96260 $ & $ i$\\
$ 55555.85671 $ & $   0.01432 $ & $   0.00079 $ & $  10.96600 $ & $ i$\\
$ 55555.85826 $ & $   0.01600 $ & $   0.00078 $ & $  10.96760 $ & $ i$\\
$ 55555.85981 $ & $   0.01730 $ & $   0.00079 $ & $  10.96870 $ & $ i$\\
$ 55555.86135 $ & $   0.01491 $ & $   0.00078 $ & $  10.96410 $ & $ i$\\
$ 55555.86292 $ & $   0.01605 $ & $   0.00078 $ & $  10.96540 $ & $ i$\\
$ 55555.86446 $ & $   0.01351 $ & $   0.00078 $ & $  10.96510 $ & $ i$\\
$ 55555.86599 $ & $   0.01609 $ & $   0.00078 $ & $  10.96580 $ & $ i$\\
$ 55555.86753 $ & $   0.01808 $ & $   0.00079 $ & $  10.96670 $ & $ i$\\
$ 55555.86910 $ & $   0.01420 $ & $   0.00077 $ & $  10.96370 $ & $ i$\\
$ 55555.87066 $ & $   0.01921 $ & $   0.00078 $ & $  10.96770 $ & $ i$\\
$ 55555.87220 $ & $   0.01561 $ & $   0.00078 $ & $  10.96390 $ & $ i$\\
$ 55555.87378 $ & $   0.01641 $ & $   0.00078 $ & $  10.96420 $ & $ i$\\
$ 55555.87534 $ & $   0.01687 $ & $   0.00078 $ & $  10.96620 $ & $ i$\\
$ 55555.87692 $ & $   0.01464 $ & $   0.00077 $ & $  10.96380 $ & $ i$\\
$ 55555.87846 $ & $   0.01605 $ & $   0.00078 $ & $  10.96430 $ & $ i$\\
$ 55555.88001 $ & $   0.01537 $ & $   0.00077 $ & $  10.96390 $ & $ i$\\
$ 55555.88156 $ & $   0.01728 $ & $   0.00079 $ & $  10.96650 $ & $ i$\\
$ 55555.88311 $ & $   0.01984 $ & $   0.00077 $ & $  10.96950 $ & $ i$\\
$ 55555.88468 $ & $   0.01781 $ & $   0.00077 $ & $  10.96630 $ & $ i$\\
$ 55555.88622 $ & $   0.02107 $ & $   0.00076 $ & $  10.96930 $ & $ i$\\
$ 55555.88777 $ & $   0.01809 $ & $   0.00078 $ & $  10.96820 $ & $ i$\\
$ 55555.88933 $ & $   0.01804 $ & $   0.00077 $ & $  10.96850 $ & $ i$\\
$ 55555.89087 $ & $   0.01943 $ & $   0.00077 $ & $  10.97050 $ & $ i$\\
$ 55555.89242 $ & $   0.01700 $ & $   0.00076 $ & $  10.96610 $ & $ i$\\
$ 55555.89396 $ & $   0.02272 $ & $   0.00077 $ & $  10.97160 $ & $ i$\\
$ 55555.89551 $ & $   0.02126 $ & $   0.00077 $ & $  10.97210 $ & $ i$\\
$ 55555.89868 $ & $   0.02099 $ & $   0.00077 $ & $  10.97000 $ & $ i$\\
$ 55555.90023 $ & $   0.01693 $ & $   0.00076 $ & $  10.96540 $ & $ i$\\
$ 55555.90178 $ & $   0.01921 $ & $   0.00077 $ & $  10.96760 $ & $ i$\\
$ 55555.90332 $ & $   0.02018 $ & $   0.00077 $ & $  10.96970 $ & $ i$\\
$ 55555.90488 $ & $   0.01847 $ & $   0.00076 $ & $  10.96590 $ & $ i$\\
$ 55555.90643 $ & $   0.01890 $ & $   0.00076 $ & $  10.96720 $ & $ i$\\
$ 55555.90800 $ & $   0.01945 $ & $   0.00077 $ & $  10.96610 $ & $ i$\\
$ 55555.90955 $ & $   0.01938 $ & $   0.00076 $ & $  10.96670 $ & $ i$\\
$ 55555.91109 $ & $   0.01661 $ & $   0.00076 $ & $  10.96230 $ & $ i$\\
$ 55555.91265 $ & $   0.01666 $ & $   0.00075 $ & $  10.96400 $ & $ i$\\
$ 55555.91420 $ & $   0.01602 $ & $   0.00076 $ & $  10.96310 $ & $ i$\\
$ 55555.91575 $ & $   0.01953 $ & $   0.00076 $ & $  10.96530 $ & $ i$\\
$ 55555.91728 $ & $   0.01629 $ & $   0.00076 $ & $  10.96390 $ & $ i$\\
$ 55555.91885 $ & $   0.01638 $ & $   0.00077 $ & $  10.96230 $ & $ i$\\
$ 55555.92048 $ & $   0.01540 $ & $   0.00076 $ & $  10.96210 $ & $ i$\\
$ 55555.92205 $ & $   0.01549 $ & $   0.00076 $ & $  10.96130 $ & $ i$\\
$ 55555.92358 $ & $   0.01430 $ & $   0.00077 $ & $  10.96110 $ & $ i$\\
$ 55555.92514 $ & $   0.01152 $ & $   0.00075 $ & $  10.95700 $ & $ i$\\
$ 55555.92667 $ & $   0.01202 $ & $   0.00076 $ & $  10.95740 $ & $ i$\\
$ 55555.92827 $ & $   0.01017 $ & $   0.00075 $ & $  10.95620 $ & $ i$\\
$ 55555.92983 $ & $   0.00612 $ & $   0.00076 $ & $  10.95080 $ & $ i$\\
$ 55555.93138 $ & $   0.00527 $ & $   0.00076 $ & $  10.95160 $ & $ i$\\
$ 55555.93291 $ & $   0.00405 $ & $   0.00075 $ & $  10.95020 $ & $ i$\\
$ 55555.93447 $ & $   0.00149 $ & $   0.00075 $ & $  10.94800 $ & $ i$\\
$ 55555.93603 $ & $   0.00122 $ & $   0.00075 $ & $  10.94660 $ & $ i$\\
$ 55555.93757 $ & $   0.00043 $ & $   0.00074 $ & $  10.94550 $ & $ i$\\
$ 55555.93912 $ & $   0.00017 $ & $   0.00075 $ & $  10.94670 $ & $ i$\\
$ 55555.94069 $ & $  -0.00012 $ & $   0.00075 $ & $  10.94410 $ & $ i$\\
$ 55555.94223 $ & $  -0.00257 $ & $   0.00074 $ & $  10.94380 $ & $ i$\\
$ 55555.94386 $ & $  -0.00091 $ & $   0.00074 $ & $  10.94540 $ & $ i$\\
$ 55555.94542 $ & $  -0.00067 $ & $   0.00074 $ & $  10.94550 $ & $ i$\\
$ 55555.94697 $ & $  -0.00283 $ & $   0.00076 $ & $  10.94350 $ & $ i$\\
$ 55555.94852 $ & $  -0.00111 $ & $   0.00075 $ & $  10.94490 $ & $ i$\\
$ 55555.95009 $ & $  -0.00282 $ & $   0.00074 $ & $  10.94340 $ & $ i$\\
$ 55555.95164 $ & $  -0.00168 $ & $   0.00075 $ & $  10.94410 $ & $ i$\\
$ 55555.95320 $ & $   0.00228 $ & $   0.00076 $ & $  10.94880 $ & $ i$\\
$ 55555.95474 $ & $   0.00019 $ & $   0.00077 $ & $  10.94510 $ & $ i$\\
$ 55555.95628 $ & $  -0.00011 $ & $   0.00077 $ & $  10.94450 $ & $ i$\\
$ 55555.95782 $ & $   0.00339 $ & $   0.00077 $ & $  10.94770 $ & $ i$\\
$ 55555.95937 $ & $   0.00359 $ & $   0.00078 $ & $  10.94860 $ & $ i$\\
$ 55555.96091 $ & $   0.00106 $ & $   0.00078 $ & $  10.94640 $ & $ i$\\
$ 55555.96246 $ & $   0.00029 $ & $   0.00080 $ & $  10.94670 $ & $ i$\\
$ 55555.96401 $ & $  -0.00190 $ & $   0.00080 $ & $  10.94220 $ & $ i$\\
$ 55555.96554 $ & $   0.00064 $ & $   0.00080 $ & $  10.94570 $ & $ i$\\
$ 55555.96949 $ & $  -0.00321 $ & $   0.00079 $ & $  10.94070 $ & $ i$\\
$ 55555.97104 $ & $  -0.00063 $ & $   0.00077 $ & $  10.94590 $ & $ i$\\
$ 55555.97258 $ & $   0.00255 $ & $   0.00076 $ & $  10.94760 $ & $ i$\\
$ 55555.97412 $ & $   0.00159 $ & $   0.00076 $ & $  10.94680 $ & $ i$\\
$ 55555.97567 $ & $   0.00037 $ & $   0.00074 $ & $  10.94670 $ & $ i$\\
$ 55555.97723 $ & $   0.00085 $ & $   0.00073 $ & $  10.94600 $ & $ i$\\
$ 55555.98030 $ & $   0.00164 $ & $   0.00074 $ & $  10.94790 $ & $ i$\\
$ 55555.98185 $ & $   0.00125 $ & $   0.00073 $ & $  10.94790 $ & $ i$\\
$ 55555.98342 $ & $   0.00042 $ & $   0.00073 $ & $  10.94670 $ & $ i$\\
$ 55555.98497 $ & $  -0.00062 $ & $   0.00074 $ & $  10.94560 $ & $ i$\\
$ 55555.98652 $ & $   0.00202 $ & $   0.00074 $ & $  10.94750 $ & $ i$\\
$ 55555.98807 $ & $   0.00098 $ & $   0.00074 $ & $  10.94850 $ & $ i$\\
$ 55555.98964 $ & $   0.00181 $ & $   0.00074 $ & $  10.94820 $ & $ i$\\
$ 55555.99117 $ & $  -0.00066 $ & $   0.00074 $ & $  10.94550 $ & $ i$\\
$ 55555.99279 $ & $  -0.00008 $ & $   0.00073 $ & $  10.94580 $ & $ i$\\
$ 55555.99435 $ & $  -0.00206 $ & $   0.00074 $ & $  10.94570 $ & $ i$\\
$ 55555.99590 $ & $  -0.00223 $ & $   0.00074 $ & $  10.94400 $ & $ i$\\
$ 55555.99745 $ & $  -0.00469 $ & $   0.00072 $ & $  10.94190 $ & $ i$\\
$ 55555.99899 $ & $   0.00004 $ & $   0.00073 $ & $  10.94410 $ & $ i$\\
$ 55556.00055 $ & $  -0.00219 $ & $   0.00074 $ & $  10.94320 $ & $ i$\\
$ 55556.00213 $ & $  -0.00291 $ & $   0.00073 $ & $  10.94350 $ & $ i$\\
$ 55556.00368 $ & $  -0.00081 $ & $   0.00072 $ & $  10.94590 $ & $ i$\\
$ 55556.00523 $ & $  -0.00234 $ & $   0.00073 $ & $  10.94390 $ & $ i$\\
$ 55556.00678 $ & $  -0.00134 $ & $   0.00073 $ & $  10.94340 $ & $ i$\\
$ 55556.00833 $ & $   0.00102 $ & $   0.00072 $ & $  10.94690 $ & $ i$\\
$ 55556.00996 $ & $  -0.00447 $ & $   0.00073 $ & $  10.94120 $ & $ i$\\
$ 55556.01150 $ & $  -0.00135 $ & $   0.00072 $ & $  10.94420 $ & $ i$\\
$ 55556.01307 $ & $  -0.00329 $ & $   0.00072 $ & $  10.94340 $ & $ i$\\
$ 55556.01463 $ & $  -0.00170 $ & $   0.00072 $ & $  10.94460 $ & $ i$\\
$ 55556.01621 $ & $  -0.00093 $ & $   0.00072 $ & $  10.94590 $ & $ i$\\
$ 55556.01776 $ & $   0.00350 $ & $   0.00074 $ & $  10.94920 $ & $ i$\\
$ 55556.01929 $ & $  -0.00271 $ & $   0.00073 $ & $  10.94450 $ & $ i$\\
$ 55556.02086 $ & $  -0.00108 $ & $   0.00073 $ & $  10.94480 $ & $ i$\\
$ 55556.02242 $ & $   0.00030 $ & $   0.00072 $ & $  10.94630 $ & $ i$\\
$ 55556.02397 $ & $  -0.00044 $ & $   0.00072 $ & $  10.94630 $ & $ i$\\
$ 55556.02553 $ & $  -0.00265 $ & $   0.00073 $ & $  10.94380 $ & $ i$\\
$ 55556.02708 $ & $  -0.00031 $ & $   0.00073 $ & $  10.94640 $ & $ i$\\
$ 55556.02864 $ & $   0.00063 $ & $   0.00073 $ & $  10.94730 $ & $ i$\\
$ 55556.03018 $ & $   0.00011 $ & $   0.00072 $ & $  10.94760 $ & $ i$\\
$ 55556.03174 $ & $   0.00085 $ & $   0.00072 $ & $  10.94780 $ & $ i$\\
$ 55556.03329 $ & $  -0.00165 $ & $   0.00073 $ & $  10.94560 $ & $ i$\\
$ 55556.03484 $ & $   0.00193 $ & $   0.00073 $ & $  10.94870 $ & $ i$\\
$ 55556.03640 $ & $   0.00055 $ & $   0.00072 $ & $  10.94810 $ & $ i$\\
$ 55556.03794 $ & $  -0.00023 $ & $   0.00072 $ & $  10.94630 $ & $ i$\\
$ 55556.03955 $ & $   0.00094 $ & $   0.00073 $ & $  10.94830 $ & $ i$\\
$ 55556.04106 $ & $   0.00040 $ & $   0.00073 $ & $  10.94710 $ & $ i$\\
$ 55556.04262 $ & $   0.00017 $ & $   0.00072 $ & $  10.94670 $ & $ i$\\
$ 55556.04419 $ & $   0.00162 $ & $   0.00072 $ & $  10.94940 $ & $ i$\\
$ 55556.04572 $ & $  -0.00040 $ & $   0.00072 $ & $  10.94650 $ & $ i$\\
$ 55556.04728 $ & $   0.00208 $ & $   0.00073 $ & $  10.94960 $ & $ i$\\
$ 55556.04882 $ & $   0.00164 $ & $   0.00073 $ & $  10.94950 $ & $ i$\\
$ 55556.05035 $ & $   0.00080 $ & $   0.00074 $ & $  10.94910 $ & $ i$\\
$ 55556.05191 $ & $   0.00529 $ & $   0.00075 $ & $  10.95350 $ & $ i$\\
$ 55556.05347 $ & $   0.00101 $ & $   0.00074 $ & $  10.94770 $ & $ i$\\
$ 55596.91755 $ & $   0.00274 $ & $   0.00079 $ & $  11.01080 $ & $ i$\\
$ 55596.91887 $ & $  -0.00042 $ & $   0.00079 $ & $  11.00820 $ & $ i$\\
$ 55596.92007 $ & $   0.00032 $ & $   0.00078 $ & $  11.00810 $ & $ i$\\
$ 55596.92128 $ & $   0.00218 $ & $   0.00079 $ & $  11.01040 $ & $ i$\\
$ 55596.92248 $ & $  -0.00087 $ & $   0.00078 $ & $  11.00710 $ & $ i$\\
$ 55596.92369 $ & $   0.00086 $ & $   0.00078 $ & $  11.00830 $ & $ i$\\
$ 55596.92489 $ & $   0.00035 $ & $   0.00078 $ & $  11.00790 $ & $ i$\\
$ 55596.92610 $ & $  -0.00050 $ & $   0.00078 $ & $  11.00660 $ & $ i$\\
$ 55596.92731 $ & $   0.00001 $ & $   0.00078 $ & $  11.00840 $ & $ i$\\
$ 55596.92851 $ & $  -0.00221 $ & $   0.00078 $ & $  11.00520 $ & $ i$\\
$ 55596.92991 $ & $   0.00095 $ & $   0.00078 $ & $  11.00870 $ & $ i$\\
$ 55596.93110 $ & $   0.00084 $ & $   0.00078 $ & $  11.00900 $ & $ i$\\
$ 55596.93228 $ & $   0.00196 $ & $   0.00078 $ & $  11.00980 $ & $ i$\\
$ 55596.93347 $ & $   0.00027 $ & $   0.00078 $ & $  11.00810 $ & $ i$\\
$ 55596.93468 $ & $  -0.00155 $ & $   0.00078 $ & $  11.00610 $ & $ i$\\
$ 55596.93608 $ & $  -0.00050 $ & $   0.00078 $ & $  11.00760 $ & $ i$\\
$ 55596.93726 $ & $  -0.00076 $ & $   0.00078 $ & $  11.00730 $ & $ i$\\
$ 55596.93846 $ & $  -0.00213 $ & $   0.00078 $ & $  11.00570 $ & $ i$\\
$ 55596.93966 $ & $  -0.00181 $ & $   0.00078 $ & $  11.00570 $ & $ i$\\
$ 55596.94086 $ & $  -0.00264 $ & $   0.00078 $ & $  11.00520 $ & $ i$\\
$ 55596.94228 $ & $  -0.00008 $ & $   0.00078 $ & $  11.00790 $ & $ i$\\
$ 55596.94349 $ & $   0.00074 $ & $   0.00078 $ & $  11.00820 $ & $ i$\\
$ 55596.94470 $ & $   0.00185 $ & $   0.00078 $ & $  11.00990 $ & $ i$\\
$ 55596.94591 $ & $   0.00195 $ & $   0.00078 $ & $  11.00950 $ & $ i$\\
$ 55596.94711 $ & $   0.00196 $ & $   0.00078 $ & $  11.00950 $ & $ i$\\
$ 55596.94848 $ & $   0.00063 $ & $   0.00078 $ & $  11.00840 $ & $ i$\\
$ 55596.94966 $ & $  -0.00030 $ & $   0.00078 $ & $  11.00770 $ & $ i$\\
$ 55596.95085 $ & $  -0.00136 $ & $   0.00078 $ & $  11.00670 $ & $ i$\\
$ 55596.95206 $ & $  -0.00135 $ & $   0.00078 $ & $  11.00660 $ & $ i$\\
$ 55596.95326 $ & $   0.00099 $ & $   0.00078 $ & $  11.00900 $ & $ i$\\
$ 55596.95496 $ & $   0.00138 $ & $   0.00078 $ & $  11.00930 $ & $ i$\\
$ 55596.95616 $ & $  -0.00107 $ & $   0.00078 $ & $  11.00680 $ & $ i$\\
$ 55596.95735 $ & $   0.00079 $ & $   0.00078 $ & $  11.00840 $ & $ i$\\
$ 55596.95853 $ & $  -0.00108 $ & $   0.00078 $ & $  11.00730 $ & $ i$\\
$ 55596.95974 $ & $   0.00021 $ & $   0.00078 $ & $  11.00780 $ & $ i$\\
$ 55596.96111 $ & $  -0.00019 $ & $   0.00078 $ & $  11.00710 $ & $ i$\\
$ 55596.96231 $ & $  -0.00077 $ & $   0.00078 $ & $  11.00720 $ & $ i$\\
$ 55596.96350 $ & $   0.00002 $ & $   0.00078 $ & $  11.00800 $ & $ i$\\
$ 55596.96470 $ & $  -0.00130 $ & $   0.00078 $ & $  11.00680 $ & $ i$\\
$ 55596.96591 $ & $  -0.00202 $ & $   0.00078 $ & $  11.00600 $ & $ i$\\
$ 55596.96712 $ & $  -0.00106 $ & $   0.00078 $ & $  11.00750 $ & $ i$\\
$ 55596.96831 $ & $  -0.00011 $ & $   0.00078 $ & $  11.00830 $ & $ i$\\
$ 55596.96949 $ & $  -0.00095 $ & $   0.00078 $ & $  11.00730 $ & $ i$\\
$ 55596.97068 $ & $  -0.00303 $ & $   0.00078 $ & $  11.00550 $ & $ i$\\
$ 55596.97188 $ & $  -0.00385 $ & $   0.00078 $ & $  11.00430 $ & $ i$\\
$ 55596.97327 $ & $   0.00103 $ & $   0.00078 $ & $  11.01020 $ & $ i$\\
$ 55596.97447 $ & $  -0.00036 $ & $   0.00078 $ & $  11.00810 $ & $ i$\\
$ 55596.97568 $ & $  -0.00172 $ & $   0.00078 $ & $  11.00750 $ & $ i$\\
$ 55596.97689 $ & $  -0.00097 $ & $   0.00078 $ & $  11.00760 $ & $ i$\\
$ 55596.97808 $ & $   0.00218 $ & $   0.00078 $ & $  11.01020 $ & $ i$\\
$ 55596.97948 $ & $  -0.00084 $ & $   0.00079 $ & $  11.00800 $ & $ i$\\
$ 55596.98069 $ & $   0.00090 $ & $   0.00079 $ & $  11.00980 $ & $ i$\\
$ 55596.98187 $ & $  -0.00019 $ & $   0.00078 $ & $  11.00930 $ & $ i$\\
$ 55596.98307 $ & $   0.00062 $ & $   0.00079 $ & $  11.00990 $ & $ i$\\
$ 55596.98426 $ & $  -0.00065 $ & $   0.00079 $ & $  11.00800 $ & $ i$\\
$ 55596.98565 $ & $   0.00160 $ & $   0.00078 $ & $  11.00990 $ & $ i$\\
$ 55596.98686 $ & $   0.00134 $ & $   0.00078 $ & $  11.01010 $ & $ i$\\
$ 55596.98806 $ & $  -0.00148 $ & $   0.00079 $ & $  11.00780 $ & $ i$\\
$ 55596.98926 $ & $  -0.00009 $ & $   0.00079 $ & $  11.00950 $ & $ i$\\
$ 55596.99048 $ & $   0.00102 $ & $   0.00078 $ & $  11.00980 $ & $ i$\\
$ 55596.99235 $ & $   0.00092 $ & $   0.00078 $ & $  11.01040 $ & $ i$\\
$ 55596.99381 $ & $   0.00327 $ & $   0.00078 $ & $  11.01190 $ & $ i$\\
$ 55596.99502 $ & $   0.00511 $ & $   0.00078 $ & $  11.01380 $ & $ i$\\
$ 55596.99623 $ & $   0.00632 $ & $   0.00079 $ & $  11.01430 $ & $ i$\\
$ 55596.99742 $ & $   0.00765 $ & $   0.00079 $ & $  11.01620 $ & $ i$\\
$ 55596.99879 $ & $   0.01016 $ & $   0.00079 $ & $  11.01930 $ & $ i$\\
$ 55596.99998 $ & $   0.01136 $ & $   0.00079 $ & $  11.02080 $ & $ i$\\
$ 55597.00117 $ & $   0.01298 $ & $   0.00079 $ & $  11.02230 $ & $ i$\\
$ 55597.00238 $ & $   0.01225 $ & $   0.00079 $ & $  11.02140 $ & $ i$\\
$ 55597.00357 $ & $   0.01559 $ & $   0.00079 $ & $  11.02550 $ & $ i$\\
$ 55597.00616 $ & $   0.01518 $ & $   0.00079 $ & $  11.02440 $ & $ i$\\
$ 55597.00738 $ & $   0.01611 $ & $   0.00080 $ & $  11.02610 $ & $ i$\\
$ 55597.00857 $ & $   0.01557 $ & $   0.00080 $ & $  11.02600 $ & $ i$\\
$ 55597.00979 $ & $   0.01832 $ & $   0.00080 $ & $  11.02800 $ & $ i$\\
$ 55597.01115 $ & $   0.01659 $ & $   0.00080 $ & $  11.02690 $ & $ i$\\
$ 55597.01233 $ & $   0.01876 $ & $   0.00079 $ & $  11.02930 $ & $ i$\\
$ 55597.01352 $ & $   0.01655 $ & $   0.00080 $ & $  11.02610 $ & $ i$\\
$ 55597.01470 $ & $   0.01661 $ & $   0.00080 $ & $  11.02710 $ & $ i$\\
$ 55597.01594 $ & $   0.01586 $ & $   0.00080 $ & $  11.02600 $ & $ i$\\
$ 55597.01759 $ & $   0.01746 $ & $   0.00082 $ & $  11.02720 $ & $ i$\\
$ 55597.01878 $ & $   0.01737 $ & $   0.00081 $ & $  11.02810 $ & $ i$\\
$ 55597.02002 $ & $   0.01763 $ & $   0.00080 $ & $  11.02850 $ & $ i$\\
$ 55597.02122 $ & $   0.01607 $ & $   0.00081 $ & $  11.02750 $ & $ i$\\
$ 55597.02241 $ & $   0.01648 $ & $   0.00081 $ & $  11.02720 $ & $ i$\\
$ 55597.02381 $ & $   0.01725 $ & $   0.00082 $ & $  11.02830 $ & $ i$\\
$ 55597.02502 $ & $   0.01781 $ & $   0.00081 $ & $  11.02890 $ & $ i$\\
$ 55597.02621 $ & $   0.01737 $ & $   0.00081 $ & $  11.02900 $ & $ i$\\
$ 55597.02740 $ & $   0.01710 $ & $   0.00083 $ & $  11.02820 $ & $ i$\\
$ 55597.02861 $ & $   0.01831 $ & $   0.00082 $ & $  11.02970 $ & $ i$\\
$ 55597.03303 $ & $   0.01674 $ & $   0.00082 $ & $  11.02830 $ & $ i$\\
$ 55597.03422 $ & $   0.01468 $ & $   0.00081 $ & $  11.02560 $ & $ i$\\
$ 55597.03541 $ & $   0.01899 $ & $   0.00082 $ & $  11.03080 $ & $ i$\\
$ 55597.03781 $ & $   0.01853 $ & $   0.00083 $ & $  11.02980 $ & $ i$\\
$ 55597.03917 $ & $   0.01732 $ & $   0.00082 $ & $  11.02910 $ & $ i$\\
$ 55597.04156 $ & $   0.01616 $ & $   0.00083 $ & $  11.02770 $ & $ i$\\
$ 55597.04274 $ & $   0.01739 $ & $   0.00082 $ & $  11.02950 $ & $ i$\\
$ 55597.04394 $ & $   0.01720 $ & $   0.00083 $ & $  11.02920 $ & $ i$\\
$ 55597.04776 $ & $   0.01803 $ & $   0.00084 $ & $  11.03060 $ & $ i$\\
$ 55597.05013 $ & $   0.01944 $ & $   0.00084 $ & $  11.03120 $ & $ i$\\
$ 55597.05393 $ & $   0.01633 $ & $   0.00087 $ & $  11.02880 $ & $ i$\\
$ 55600.92457 $ & $  -0.00013 $ & $   0.00078 $ & $  11.00160 $ & $ i$\\
$ 55600.92578 $ & $  -0.00061 $ & $   0.00078 $ & $  11.00150 $ & $ i$\\
$ 55600.92698 $ & $  -0.00197 $ & $   0.00078 $ & $  11.00090 $ & $ i$\\
$ 55600.92819 $ & $   0.00030 $ & $   0.00078 $ & $  11.00230 $ & $ i$\\
$ 55600.92940 $ & $   0.00044 $ & $   0.00078 $ & $  11.00320 $ & $ i$\\
$ 55600.93059 $ & $   0.00013 $ & $   0.00078 $ & $  11.00260 $ & $ i$\\
$ 55600.93176 $ & $   0.00119 $ & $   0.00078 $ & $  11.00360 $ & $ i$\\
$ 55600.93295 $ & $   0.00122 $ & $   0.00078 $ & $  11.00450 $ & $ i$\\
$ 55600.93416 $ & $  -0.00160 $ & $   0.00078 $ & $  11.00190 $ & $ i$\\
$ 55600.93535 $ & $  -0.00077 $ & $   0.00078 $ & $  11.00240 $ & $ i$\\
$ 55600.93656 $ & $  -0.00112 $ & $   0.00078 $ & $  11.00200 $ & $ i$\\
$ 55600.93777 $ & $  -0.00241 $ & $   0.00078 $ & $  11.00120 $ & $ i$\\
$ 55600.93896 $ & $   0.00122 $ & $   0.00078 $ & $  11.00470 $ & $ i$\\
$ 55600.94018 $ & $   0.00043 $ & $   0.00078 $ & $  11.00390 $ & $ i$\\
$ 55600.94138 $ & $   0.00225 $ & $   0.00078 $ & $  11.00610 $ & $ i$\\
$ 55600.94258 $ & $   0.00174 $ & $   0.00078 $ & $  11.00580 $ & $ i$\\
$ 55600.94379 $ & $   0.00065 $ & $   0.00078 $ & $  11.00460 $ & $ i$\\
$ 55600.94499 $ & $   0.00110 $ & $   0.00078 $ & $  11.00490 $ & $ i$\\
$ 55600.94621 $ & $   0.00144 $ & $   0.00078 $ & $  11.00570 $ & $ i$\\
$ 55600.94741 $ & $   0.00013 $ & $   0.00078 $ & $  11.00490 $ & $ i$\\
$ 55600.94860 $ & $   0.00095 $ & $   0.00078 $ & $  11.00520 $ & $ i$\\
$ 55600.94981 $ & $   0.00099 $ & $   0.00078 $ & $  11.00470 $ & $ i$\\
$ 55600.95100 $ & $   0.00178 $ & $   0.00078 $ & $  11.00590 $ & $ i$\\
$ 55600.95220 $ & $  -0.00025 $ & $   0.00078 $ & $  11.00320 $ & $ i$\\
$ 55600.95342 $ & $   0.00039 $ & $   0.00078 $ & $  11.00470 $ & $ i$\\
$ 55600.95470 $ & $  -0.00111 $ & $   0.00078 $ & $  11.00320 $ & $ i$\\
$ 55600.95589 $ & $  -0.00015 $ & $   0.00078 $ & $  11.00420 $ & $ i$\\
$ 55600.95710 $ & $   0.00045 $ & $   0.00078 $ & $  11.00440 $ & $ i$\\
$ 55600.95830 $ & $   0.00024 $ & $   0.00078 $ & $  11.00440 $ & $ i$\\
$ 55600.95951 $ & $  -0.00136 $ & $   0.00078 $ & $  11.00300 $ & $ i$\\
$ 55600.96070 $ & $   0.00060 $ & $   0.00078 $ & $  11.00450 $ & $ i$\\
$ 55600.96190 $ & $   0.00001 $ & $   0.00078 $ & $  11.00370 $ & $ i$\\
$ 55600.96312 $ & $  -0.00047 $ & $   0.00078 $ & $  11.00320 $ & $ i$\\
$ 55600.96431 $ & $  -0.00068 $ & $   0.00078 $ & $  11.00310 $ & $ i$\\
$ 55600.96550 $ & $  -0.00064 $ & $   0.00078 $ & $  11.00440 $ & $ i$\\
$ 55600.96672 $ & $   0.00119 $ & $   0.00078 $ & $  11.00550 $ & $ i$\\
$ 55600.96793 $ & $  -0.00145 $ & $   0.00078 $ & $  11.00370 $ & $ i$\\
$ 55600.96915 $ & $  -0.00035 $ & $   0.00078 $ & $  11.00430 $ & $ i$\\
$ 55600.97036 $ & $  -0.00094 $ & $   0.00078 $ & $  11.00340 $ & $ i$\\
$ 55600.97157 $ & $  -0.00088 $ & $   0.00078 $ & $  11.00380 $ & $ i$\\
$ 55600.97278 $ & $  -0.00121 $ & $   0.00078 $ & $  11.00330 $ & $ i$\\
$ 55600.97400 $ & $  -0.00155 $ & $   0.00078 $ & $  11.00320 $ & $ i$\\
$ 55600.97520 $ & $  -0.00015 $ & $   0.00078 $ & $  11.00410 $ & $ i$\\
$ 55600.97642 $ & $   0.00256 $ & $   0.00078 $ & $  11.00780 $ & $ i$\\
$ 55600.97763 $ & $   0.00433 $ & $   0.00078 $ & $  11.00880 $ & $ i$\\
$ 55600.97883 $ & $   0.00453 $ & $   0.00078 $ & $  11.00850 $ & $ i$\\
$ 55600.98006 $ & $   0.00763 $ & $   0.00078 $ & $  11.01230 $ & $ i$\\
$ 55600.98126 $ & $   0.00878 $ & $   0.00078 $ & $  11.01330 $ & $ i$\\
$ 55600.98248 $ & $   0.01047 $ & $   0.00079 $ & $  11.01530 $ & $ i$\\
$ 55600.98368 $ & $   0.01247 $ & $   0.00078 $ & $  11.01720 $ & $ i$\\
$ 55600.98496 $ & $   0.01361 $ & $   0.00079 $ & $  11.01800 $ & $ i$\\
$ 55600.98617 $ & $   0.01530 $ & $   0.00079 $ & $  11.02050 $ & $ i$\\
$ 55600.98738 $ & $   0.01409 $ & $   0.00078 $ & $  11.01850 $ & $ i$\\
$ 55600.98857 $ & $   0.01292 $ & $   0.00079 $ & $  11.01760 $ & $ i$\\
$ 55600.98977 $ & $   0.01460 $ & $   0.00079 $ & $  11.01860 $ & $ i$\\
$ 55600.99098 $ & $   0.01504 $ & $   0.00079 $ & $  11.01880 $ & $ i$\\
$ 55600.99219 $ & $   0.01611 $ & $   0.00079 $ & $  11.02100 $ & $ i$\\
$ 55600.99341 $ & $   0.01662 $ & $   0.00079 $ & $  11.02180 $ & $ i$\\
$ 55600.99462 $ & $   0.01660 $ & $   0.00079 $ & $  11.02190 $ & $ i$\\
$ 55600.99584 $ & $   0.01585 $ & $   0.00079 $ & $  11.02200 $ & $ i$\\
$ 55600.99704 $ & $   0.01537 $ & $   0.00079 $ & $  11.02100 $ & $ i$\\
$ 55600.99826 $ & $   0.01648 $ & $   0.00079 $ & $  11.02240 $ & $ i$\\
$ 55600.99946 $ & $   0.01686 $ & $   0.00079 $ & $  11.02250 $ & $ i$\\
$ 55601.00065 $ & $   0.01876 $ & $   0.00079 $ & $  11.02420 $ & $ i$\\
$ 55601.00186 $ & $   0.01807 $ & $   0.00079 $ & $  11.02360 $ & $ i$\\
$ 55601.00305 $ & $   0.02016 $ & $   0.00079 $ & $  11.02610 $ & $ i$\\
$ 55601.00425 $ & $   0.01889 $ & $   0.00079 $ & $  11.02500 $ & $ i$\\
$ 55601.00546 $ & $   0.01788 $ & $   0.00079 $ & $  11.02410 $ & $ i$\\
$ 55601.00665 $ & $   0.01957 $ & $   0.00079 $ & $  11.02540 $ & $ i$\\
$ 55601.00786 $ & $   0.01793 $ & $   0.00079 $ & $  11.02320 $ & $ i$\\
$ 55601.00906 $ & $   0.01526 $ & $   0.00079 $ & $  11.02170 $ & $ i$\\
$ 55601.01025 $ & $   0.01880 $ & $   0.00079 $ & $  11.02440 $ & $ i$\\
$ 55601.01145 $ & $   0.01990 $ & $   0.00079 $ & $  11.02580 $ & $ i$\\
$ 55601.01265 $ & $   0.01856 $ & $   0.00079 $ & $  11.02510 $ & $ i$\\
$ 55601.01386 $ & $   0.01770 $ & $   0.00079 $ & $  11.02340 $ & $ i$\\
$ 55601.01631 $ & $   0.01966 $ & $   0.00079 $ & $  11.02580 $ & $ i$\\
$ 55601.01753 $ & $   0.01524 $ & $   0.00079 $ & $  11.02210 $ & $ i$\\
$ 55601.01872 $ & $   0.01558 $ & $   0.00079 $ & $  11.02250 $ & $ i$\\
$ 55601.01992 $ & $   0.01837 $ & $   0.00079 $ & $  11.02420 $ & $ i$\\
$ 55601.02113 $ & $   0.01915 $ & $   0.00079 $ & $  11.02510 $ & $ i$\\
$ 55601.02233 $ & $   0.01748 $ & $   0.00079 $ & $  11.02290 $ & $ i$\\
$ 55601.02354 $ & $   0.01937 $ & $   0.00079 $ & $  11.02540 $ & $ i$\\
$ 55601.02474 $ & $   0.01826 $ & $   0.00079 $ & $  11.02320 $ & $ i$\\
$ 55601.02597 $ & $   0.01720 $ & $   0.00079 $ & $  11.02320 $ & $ i$\\
$ 55601.02718 $ & $   0.01911 $ & $   0.00079 $ & $  11.02390 $ & $ i$\\
$ 55601.02838 $ & $   0.01843 $ & $   0.00079 $ & $  11.02390 $ & $ i$\\
$ 55601.02960 $ & $   0.01786 $ & $   0.00079 $ & $  11.02400 $ & $ i$\\
$ 55601.03082 $ & $   0.01774 $ & $   0.00079 $ & $  11.02340 $ & $ i$\\
$ 55601.03203 $ & $   0.01890 $ & $   0.00080 $ & $  11.02480 $ & $ i$\\
$ 55601.03322 $ & $   0.01669 $ & $   0.00079 $ & $  11.02280 $ & $ i$\\
$ 55601.03444 $ & $   0.01826 $ & $   0.00079 $ & $  11.02500 $ & $ i$\\
$ 55601.03565 $ & $   0.01710 $ & $   0.00079 $ & $  11.02370 $ & $ i$\\
$ 55601.03687 $ & $   0.01675 $ & $   0.00079 $ & $  11.02300 $ & $ i$\\
$ 55601.03807 $ & $   0.01785 $ & $   0.00079 $ & $  11.02430 $ & $ i$\\
$ 55601.03929 $ & $   0.01697 $ & $   0.00079 $ & $  11.02270 $ & $ i$\\
$ 55601.04050 $ & $   0.01667 $ & $   0.00079 $ & $  11.02210 $ & $ i$\\
$ 55601.04171 $ & $   0.01708 $ & $   0.00079 $ & $  11.02250 $ & $ i$\\
$ 55601.04291 $ & $   0.01762 $ & $   0.00079 $ & $  11.02420 $ & $ i$\\
$ 55601.04413 $ & $   0.01598 $ & $   0.00080 $ & $  11.02280 $ & $ i$\\
$ 55601.04536 $ & $   0.01542 $ & $   0.00079 $ & $  11.02050 $ & $ i$\\
$ 55601.04658 $ & $   0.01582 $ & $   0.00079 $ & $  11.02140 $ & $ i$\\
$ 55601.04777 $ & $   0.01344 $ & $   0.00080 $ & $  11.01950 $ & $ i$\\
$ 55601.04898 $ & $   0.01455 $ & $   0.00080 $ & $  11.02210 $ & $ i$\\
$ 55601.05017 $ & $   0.01581 $ & $   0.00080 $ & $  11.02150 $ & $ i$\\
$ 55608.89527 $ & $   0.00004 $ & $   0.00112 $ & $  11.17330 $ & $ i$\\
$ 55608.89600 $ & $  -0.00023 $ & $   0.00113 $ & $  11.17360 $ & $ i$\\
$ 55608.89693 $ & $   0.00276 $ & $   0.00112 $ & $  11.17600 $ & $ i$\\
$ 55608.89765 $ & $   0.00023 $ & $   0.00113 $ & $  11.17350 $ & $ i$\\
$ 55608.89857 $ & $   0.00022 $ & $   0.00113 $ & $  11.17400 $ & $ i$\\
$ 55608.89930 $ & $   0.00105 $ & $   0.00112 $ & $  11.17440 $ & $ i$\\
$ 55608.90021 $ & $  -0.00167 $ & $   0.00113 $ & $  11.17210 $ & $ i$\\
$ 55608.90094 $ & $  -0.00450 $ & $   0.00112 $ & $  11.16840 $ & $ i$\\
$ 55608.90188 $ & $   0.00023 $ & $   0.00113 $ & $  11.17370 $ & $ i$\\
$ 55608.90262 $ & $  -0.00001 $ & $   0.00112 $ & $  11.17330 $ & $ i$\\
$ 55608.90357 $ & $  -0.00025 $ & $   0.00112 $ & $  11.17310 $ & $ i$\\
$ 55608.90430 $ & $   0.00101 $ & $   0.00112 $ & $  11.17450 $ & $ i$\\
$ 55608.90521 $ & $   0.00040 $ & $   0.00113 $ & $  11.17380 $ & $ i$\\
$ 55608.90595 $ & $   0.00099 $ & $   0.00113 $ & $  11.17390 $ & $ i$\\
$ 55608.90684 $ & $  -0.00060 $ & $   0.00112 $ & $  11.17280 $ & $ i$\\
$ 55608.90757 $ & $  -0.00191 $ & $   0.00112 $ & $  11.17190 $ & $ i$\\
$ 55608.90849 $ & $  -0.00131 $ & $   0.00113 $ & $  11.17110 $ & $ i$\\
$ 55608.90920 $ & $  -0.00086 $ & $   0.00112 $ & $  11.17190 $ & $ i$\\
$ 55608.91013 $ & $  -0.00035 $ & $   0.00112 $ & $  11.17350 $ & $ i$\\
$ 55608.91086 $ & $   0.00321 $ & $   0.00113 $ & $  11.17620 $ & $ i$\\
$ 55608.91180 $ & $  -0.00066 $ & $   0.00112 $ & $  11.17230 $ & $ i$\\
$ 55608.91254 $ & $  -0.00407 $ & $   0.00112 $ & $  11.16880 $ & $ i$\\
$ 55608.91345 $ & $   0.00066 $ & $   0.00113 $ & $  11.17340 $ & $ i$\\
$ 55608.91421 $ & $  -0.00160 $ & $   0.00113 $ & $  11.17160 $ & $ i$\\
$ 55608.91513 $ & $   0.00214 $ & $   0.00113 $ & $  11.17440 $ & $ i$\\
$ 55608.91586 $ & $  -0.00004 $ & $   0.00112 $ & $  11.17300 $ & $ i$\\
$ 55608.91661 $ & $  -0.00123 $ & $   0.00113 $ & $  11.17220 $ & $ i$\\
$ 55608.91736 $ & $  -0.00007 $ & $   0.00112 $ & $  11.17250 $ & $ i$\\
$ 55608.91828 $ & $  -0.00028 $ & $   0.00112 $ & $  11.17320 $ & $ i$\\
$ 55608.91901 $ & $  -0.00206 $ & $   0.00112 $ & $  11.17130 $ & $ i$\\
$ 55608.91994 $ & $   0.00232 $ & $   0.00113 $ & $  11.17590 $ & $ i$\\
$ 55608.92066 $ & $   0.00190 $ & $   0.00113 $ & $  11.17570 $ & $ i$\\
$ 55608.92158 $ & $   0.00074 $ & $   0.00113 $ & $  11.17320 $ & $ i$\\
$ 55608.92232 $ & $   0.00196 $ & $   0.00113 $ & $  11.17600 $ & $ i$\\
$ 55608.92323 $ & $  -0.00008 $ & $   0.00112 $ & $  11.17390 $ & $ i$\\
$ 55608.92396 $ & $  -0.00109 $ & $   0.00113 $ & $  11.17220 $ & $ i$\\
$ 55608.92488 $ & $   0.00124 $ & $   0.00112 $ & $  11.17550 $ & $ i$\\
$ 55608.92560 $ & $   0.00006 $ & $   0.00112 $ & $  11.17310 $ & $ i$\\
$ 55608.92654 $ & $  -0.00112 $ & $   0.00113 $ & $  11.17220 $ & $ i$\\
$ 55608.92727 $ & $   0.00111 $ & $   0.00114 $ & $  11.17470 $ & $ i$\\
$ 55608.92805 $ & $   0.00173 $ & $   0.00113 $ & $  11.17610 $ & $ i$\\
$ 55608.92878 $ & $  -0.00189 $ & $   0.00112 $ & $  11.17220 $ & $ i$\\
$ 55608.92953 $ & $   0.00065 $ & $   0.00112 $ & $  11.17420 $ & $ i$\\
$ 55608.93027 $ & $   0.00110 $ & $   0.00112 $ & $  11.17460 $ & $ i$\\
$ 55608.93119 $ & $  -0.00028 $ & $   0.00112 $ & $  11.17370 $ & $ i$\\
$ 55608.93192 $ & $   0.00122 $ & $   0.00112 $ & $  11.17500 $ & $ i$\\
$ 55608.93285 $ & $  -0.00148 $ & $   0.00112 $ & $  11.17280 $ & $ i$\\
$ 55608.93358 $ & $   0.00099 $ & $   0.00112 $ & $  11.17520 $ & $ i$\\
$ 55608.93451 $ & $   0.00039 $ & $   0.00112 $ & $  11.17470 $ & $ i$\\
$ 55608.93523 $ & $  -0.00092 $ & $   0.00112 $ & $  11.17280 $ & $ i$\\
$ 55608.93602 $ & $  -0.00098 $ & $   0.00112 $ & $  11.17280 $ & $ i$\\
$ 55608.93676 $ & $   0.00046 $ & $   0.00112 $ & $  11.17470 $ & $ i$\\
$ 55608.93768 $ & $   0.00117 $ & $   0.00112 $ & $  11.17500 $ & $ i$\\
$ 55608.93842 $ & $   0.00081 $ & $   0.00112 $ & $  11.17410 $ & $ i$\\
$ 55608.93935 $ & $   0.00083 $ & $   0.00112 $ & $  11.17520 $ & $ i$\\
$ 55608.94007 $ & $   0.00379 $ & $   0.00112 $ & $  11.17750 $ & $ i$\\
$ 55608.94098 $ & $   0.00201 $ & $   0.00112 $ & $  11.17620 $ & $ i$\\
$ 55608.94170 $ & $   0.00219 $ & $   0.00112 $ & $  11.17590 $ & $ i$\\
$ 55608.94264 $ & $   0.00832 $ & $   0.00113 $ & $  11.18220 $ & $ i$\\
$ 55608.94337 $ & $   0.00910 $ & $   0.00112 $ & $  11.18240 $ & $ i$\\
$ 55608.94432 $ & $   0.00675 $ & $   0.00112 $ & $  11.17980 $ & $ i$\\
$ 55608.94506 $ & $   0.00682 $ & $   0.00112 $ & $  11.18010 $ & $ i$\\
$ 55608.94599 $ & $   0.01222 $ & $   0.00112 $ & $  11.18530 $ & $ i$\\
$ 55608.94673 $ & $   0.01385 $ & $   0.00113 $ & $  11.18710 $ & $ i$\\
$ 55608.94765 $ & $   0.01130 $ & $   0.00112 $ & $  11.18470 $ & $ i$\\
$ 55608.94838 $ & $   0.01382 $ & $   0.00113 $ & $  11.18730 $ & $ i$\\
$ 55608.94931 $ & $   0.01430 $ & $   0.00113 $ & $  11.18800 $ & $ i$\\
$ 55608.95004 $ & $   0.01413 $ & $   0.00113 $ & $  11.18750 $ & $ i$\\
$ 55608.95098 $ & $   0.01380 $ & $   0.00113 $ & $  11.18720 $ & $ i$\\
$ 55608.95172 $ & $   0.01749 $ & $   0.00113 $ & $  11.19080 $ & $ i$\\
$ 55608.95266 $ & $   0.01416 $ & $   0.00113 $ & $  11.18790 $ & $ i$\\
$ 55608.95341 $ & $   0.01183 $ & $   0.00112 $ & $  11.18540 $ & $ i$\\
$ 55608.95433 $ & $   0.01760 $ & $   0.00113 $ & $  11.19160 $ & $ i$\\
$ 55608.95506 $ & $   0.01559 $ & $   0.00113 $ & $  11.18900 $ & $ i$\\
$ 55608.95595 $ & $   0.01544 $ & $   0.00113 $ & $  11.18870 $ & $ i$\\
$ 55608.95669 $ & $   0.01567 $ & $   0.00113 $ & $  11.18950 $ & $ i$\\
$ 55608.95763 $ & $   0.01304 $ & $   0.00113 $ & $  11.18670 $ & $ i$\\
$ 55608.95836 $ & $   0.01862 $ & $   0.00113 $ & $  11.19200 $ & $ i$\\
$ 55608.95927 $ & $   0.01698 $ & $   0.00113 $ & $  11.19070 $ & $ i$\\
$ 55608.96002 $ & $   0.01551 $ & $   0.00113 $ & $  11.18930 $ & $ i$\\
$ 55608.96096 $ & $   0.01684 $ & $   0.00113 $ & $  11.19000 $ & $ i$\\
$ 55608.96171 $ & $   0.01798 $ & $   0.00113 $ & $  11.19210 $ & $ i$\\
$ 55608.96261 $ & $   0.01895 $ & $   0.00114 $ & $  11.19340 $ & $ i$\\
$ 55608.96334 $ & $   0.01703 $ & $   0.00113 $ & $  11.19130 $ & $ i$\\
$ 55608.96424 $ & $   0.01587 $ & $   0.00113 $ & $  11.18960 $ & $ i$\\
$ 55608.96498 $ & $   0.01541 $ & $   0.00114 $ & $  11.18940 $ & $ i$\\
$ 55608.96590 $ & $   0.01876 $ & $   0.00113 $ & $  11.19250 $ & $ i$\\
$ 55608.96664 $ & $   0.01489 $ & $   0.00113 $ & $  11.18880 $ & $ i$\\
$ 55608.96739 $ & $   0.01637 $ & $   0.00113 $ & $  11.19000 $ & $ i$\\
$ 55608.96811 $ & $   0.01261 $ & $   0.00114 $ & $  11.18650 $ & $ i$\\
$ 55608.96904 $ & $   0.01727 $ & $   0.00114 $ & $  11.19160 $ & $ i$\\
$ 55608.96977 $ & $   0.01725 $ & $   0.00115 $ & $  11.19020 $ & $ i$\\
$ 55608.97071 $ & $   0.01507 $ & $   0.00114 $ & $  11.18930 $ & $ i$\\
$ 55608.97144 $ & $   0.01670 $ & $   0.00113 $ & $  11.18950 $ & $ i$\\
$ 55608.97235 $ & $   0.01866 $ & $   0.00113 $ & $  11.19290 $ & $ i$\\
$ 55608.97309 $ & $   0.01967 $ & $   0.00114 $ & $  11.19390 $ & $ i$\\
$ 55608.97402 $ & $   0.01989 $ & $   0.00113 $ & $  11.19450 $ & $ i$\\
$ 55608.97476 $ & $   0.01585 $ & $   0.00114 $ & $  11.18960 $ & $ i$\\
$ 55608.97568 $ & $   0.02000 $ & $   0.00114 $ & $  11.19460 $ & $ i$\\
$ 55608.97640 $ & $   0.01874 $ & $   0.00113 $ & $  11.19260 $ & $ i$\\
$ 55608.97734 $ & $   0.02214 $ & $   0.00113 $ & $  11.19620 $ & $ i$\\
$ 55608.97807 $ & $   0.02105 $ & $   0.00113 $ & $  11.19570 $ & $ i$\\
$ 55608.97900 $ & $   0.01750 $ & $   0.00113 $ & $  11.19210 $ & $ i$\\
$ 55608.97976 $ & $   0.01781 $ & $   0.00113 $ & $  11.19240 $ & $ i$\\
$ 55608.98069 $ & $   0.01964 $ & $   0.00113 $ & $  11.19360 $ & $ i$\\
$ 55608.98143 $ & $   0.01847 $ & $   0.00113 $ & $  11.19290 $ & $ i$\\
$ 55608.98217 $ & $   0.02045 $ & $   0.00113 $ & $  11.19530 $ & $ i$\\
$ 55608.98291 $ & $   0.01716 $ & $   0.00113 $ & $  11.19130 $ & $ i$\\
$ 55608.98381 $ & $   0.01654 $ & $   0.00114 $ & $  11.19120 $ & $ i$\\
$ 55608.98454 $ & $   0.01644 $ & $   0.00114 $ & $  11.19110 $ & $ i$\\
$ 55608.98550 $ & $   0.01967 $ & $   0.00113 $ & $  11.19470 $ & $ i$\\
$ 55608.98623 $ & $   0.01943 $ & $   0.00114 $ & $  11.19430 $ & $ i$\\
$ 55608.98715 $ & $   0.01772 $ & $   0.00114 $ & $  11.19150 $ & $ i$\\
$ 55608.98787 $ & $   0.01643 $ & $   0.00114 $ & $  11.19070 $ & $ i$\\
$ 55608.98881 $ & $   0.01648 $ & $   0.00113 $ & $  11.19050 $ & $ i$\\
$ 55608.98955 $ & $   0.01506 $ & $   0.00113 $ & $  11.18920 $ & $ i$\\
$ 55608.99047 $ & $   0.01900 $ & $   0.00114 $ & $  11.19290 $ & $ i$\\
$ 55608.99120 $ & $   0.01820 $ & $   0.00114 $ & $  11.19240 $ & $ i$\\
$ 55608.99213 $ & $   0.01739 $ & $   0.00113 $ & $  11.19140 $ & $ i$\\
$ 55608.99287 $ & $   0.01666 $ & $   0.00113 $ & $  11.19100 $ & $ i$\\
$ 55608.99382 $ & $   0.01332 $ & $   0.00113 $ & $  11.18780 $ & $ i$\\
$ 55608.99455 $ & $   0.01575 $ & $   0.00114 $ & $  11.19030 $ & $ i$\\
$ 55608.99546 $ & $   0.01895 $ & $   0.00113 $ & $  11.19290 $ & $ i$\\
$ 55608.99618 $ & $   0.01713 $ & $   0.00113 $ & $  11.19100 $ & $ i$\\
$ 55608.99712 $ & $   0.02030 $ & $   0.00113 $ & $  11.19440 $ & $ i$\\
$ 55608.99785 $ & $   0.01902 $ & $   0.00113 $ & $  11.19320 $ & $ i$\\
$ 55608.99875 $ & $   0.01713 $ & $   0.00113 $ & $  11.19120 $ & $ i$\\
$ 55608.99949 $ & $   0.01947 $ & $   0.00113 $ & $  11.19380 $ & $ i$\\
$ 55609.00024 $ & $   0.01462 $ & $   0.00113 $ & $  11.18880 $ & $ i$\\
$ 55609.00096 $ & $   0.01820 $ & $   0.00113 $ & $  11.19210 $ & $ i$\\
$ 55609.00190 $ & $   0.01733 $ & $   0.00113 $ & $  11.19180 $ & $ i$\\
$ 55609.00263 $ & $   0.01589 $ & $   0.00113 $ & $  11.19000 $ & $ i$\\
$ 55609.00356 $ & $   0.01881 $ & $   0.00113 $ & $  11.19310 $ & $ i$\\
$ 55609.00429 $ & $   0.01424 $ & $   0.00113 $ & $  11.18860 $ & $ i$\\
$ 55609.00522 $ & $   0.01394 $ & $   0.00114 $ & $  11.18860 $ & $ i$\\
$ 55609.00597 $ & $   0.01395 $ & $   0.00113 $ & $  11.18890 $ & $ i$\\
$ 55609.00688 $ & $   0.01638 $ & $   0.00113 $ & $  11.19070 $ & $ i$\\
$ 55609.00761 $ & $   0.01780 $ & $   0.00113 $ & $  11.19230 $ & $ i$\\
$ 55609.00851 $ & $   0.01636 $ & $   0.00113 $ & $  11.19030 $ & $ i$\\
$ 55609.00924 $ & $   0.01558 $ & $   0.00113 $ & $  11.18920 $ & $ i$\\
$ 55609.01018 $ & $   0.01640 $ & $   0.00113 $ & $  11.19030 $ & $ i$\\
$ 55609.01094 $ & $   0.01319 $ & $   0.00113 $ & $  11.18750 $ & $ i$\\
$ 55609.01187 $ & $   0.01458 $ & $   0.00114 $ & $  11.18900 $ & $ i$\\
$ 55609.01260 $ & $   0.01362 $ & $   0.00113 $ & $  11.18790 $ & $ i$\\
$ 55609.01351 $ & $   0.01686 $ & $   0.00114 $ & $  11.19100 $ & $ i$\\
$ 55609.01424 $ & $   0.01541 $ & $   0.00113 $ & $  11.18920 $ & $ i$\\
$ 55609.01517 $ & $   0.01404 $ & $   0.00113 $ & $  11.18870 $ & $ i$\\
$ 55609.01590 $ & $   0.01242 $ & $   0.00113 $ & $  11.18670 $ & $ i$\\
$ 55609.01682 $ & $   0.01371 $ & $   0.00114 $ & $  11.18800 $ & $ i$\\
$ 55609.01756 $ & $   0.01689 $ & $   0.00115 $ & $  11.19070 $ & $ i$\\
$ 55609.01850 $ & $   0.01841 $ & $   0.00114 $ & $  11.19310 $ & $ i$\\
$ 55609.01923 $ & $   0.01336 $ & $   0.00114 $ & $  11.18750 $ & $ i$\\
$ 55609.02017 $ & $   0.01466 $ & $   0.00114 $ & $  11.18930 $ & $ i$\\
$ 55609.02091 $ & $   0.01138 $ & $   0.00114 $ & $  11.18660 $ & $ i$\\
$ 55609.02180 $ & $   0.01250 $ & $   0.00114 $ & $  11.18620 $ & $ i$\\
$ 55609.02253 $ & $   0.01148 $ & $   0.00114 $ & $  11.18510 $ & $ i$\\
$ 55609.02344 $ & $   0.00820 $ & $   0.00114 $ & $  11.18230 $ & $ i$\\
$ 55609.02418 $ & $   0.00372 $ & $   0.00113 $ & $  11.17850 $ & $ i$\\
$ 55609.02507 $ & $   0.00599 $ & $   0.00113 $ & $  11.17970 $ & $ i$\\
$ 55609.02581 $ & $   0.00611 $ & $   0.00113 $ & $  11.17910 $ & $ i$\\
$ 55609.02659 $ & $   0.00615 $ & $   0.00113 $ & $  11.18030 $ & $ i$\\
$ 55609.02732 $ & $   0.00155 $ & $   0.00113 $ & $  11.17590 $ & $ i$\\
$ 55609.02826 $ & $   0.00114 $ & $   0.00112 $ & $  11.17540 $ & $ i$\\
$ 55609.02899 $ & $   0.00105 $ & $   0.00112 $ & $  11.17520 $ & $ i$\\
$ 55609.02974 $ & $  -0.00295 $ & $   0.00112 $ & $  11.17180 $ & $ i$\\
$ 55609.03047 $ & $  -0.00297 $ & $   0.00112 $ & $  11.17160 $ & $ i$\\
$ 55609.03141 $ & $  -0.00039 $ & $   0.00112 $ & $  11.17370 $ & $ i$\\
$ 55609.03213 $ & $   0.00020 $ & $   0.00112 $ & $  11.17410 $ & $ i$\\
$ 55609.03305 $ & $   0.00272 $ & $   0.00112 $ & $  11.17690 $ & $ i$\\
$ 55609.03380 $ & $  -0.00123 $ & $   0.00112 $ & $  11.17290 $ & $ i$\\
$ 55609.03475 $ & $   0.00110 $ & $   0.00112 $ & $  11.17620 $ & $ i$\\
$ 55609.03639 $ & $   0.00335 $ & $   0.00112 $ & $  11.17770 $ & $ i$\\
$ 55609.03713 $ & $  -0.00012 $ & $   0.00111 $ & $  11.17430 $ & $ i$\\
$ 55609.03805 $ & $   0.00251 $ & $   0.00112 $ & $  11.17730 $ & $ i$\\
$ 55609.03878 $ & $  -0.00133 $ & $   0.00111 $ & $  11.17350 $ & $ i$\\
$ 55609.03972 $ & $   0.00030 $ & $   0.00111 $ & $  11.17450 $ & $ i$\\
$ 55609.04044 $ & $  -0.00078 $ & $   0.00112 $ & $  11.17320 $ & $ i$\\
$ 55609.04137 $ & $   0.00150 $ & $   0.00111 $ & $  11.17490 $ & $ i$\\
$ 55609.04210 $ & $   0.00118 $ & $   0.00112 $ & $  11.17570 $ & $ i$\\
$ 55609.04305 $ & $  -0.00073 $ & $   0.00112 $ & $  11.17350 $ & $ i$\\
$ 55609.04378 $ & $   0.00141 $ & $   0.00112 $ & $  11.17600 $ & $ i$\\
$ 55609.04468 $ & $  -0.00076 $ & $   0.00112 $ & $  11.17370 $ & $ i$\\
$ 55609.04542 $ & $  -0.00152 $ & $   0.00112 $ & $  11.17240 $ & $ i$\\
$ 55609.04635 $ & $   0.00055 $ & $   0.00113 $ & $  11.17450 $ & $ i$\\
$ 55609.04709 $ & $  -0.00204 $ & $   0.00113 $ & $  11.17210 $ & $ i$\\
$ 55609.04800 $ & $  -0.00009 $ & $   0.00113 $ & $  11.17410 $ & $ i$\\


==> data/HTR143-001_phfu_tab_short.tex <==
$ 55555.84870 $ & $   0.00292 $ & $   0.00081 $ & $  10.95490 $ & $ i$\\
$ 55555.85050 $ & $   0.00957 $ & $   0.00083 $ & $  10.96050 $ & $ i$\\
$ 55555.85205 $ & $   0.00817 $ & $   0.00078 $ & $  10.96100 $ & $ i$\\
$ 55555.85362 $ & $   0.01416 $ & $   0.00079 $ & $  10.96370 $ & $ i$\\
$ 55555.85516 $ & $   0.01203 $ & $   0.00079 $ & $  10.96260 $ & $ i$\\
$ 55555.85671 $ & $   0.01521 $ & $   0.00079 $ & $  10.96600 $ & $ i$\\
$ 55555.85826 $ & $   0.01690 $ & $   0.00078 $ & $  10.96760 $ & $ i$\\
$ 55555.85981 $ & $   0.01833 $ & $   0.00079 $ & $  10.96870 $ & $ i$\\
$ 55555.86135 $ & $   0.01590 $ & $   0.00078 $ & $  10.96410 $ & $ i$\\
$ 55555.86292 $ & $   0.01733 $ & $   0.00078 $ & $  10.96540 $ & $ i$\\


==> data/HTR143-001_rvtable.tex <==
$ 1547.02139 $ & $  -206.37 $ & $    22.40 $ & $    20.50 $ & $    15.80 $ & $   0.319 $\\
$ 1550.04236 $ & $   200.83 $ & $    22.80 $ & $   -11.40 $ & $    21.60 $ & $   0.594 $\\
$ 1554.99394 $ & $  -293.87 $ & $    11.40 $ & $    -7.50 $ & $     7.50 $ & $   0.325 $\\
$ 1556.05388 $ & $  -237.67 $ & $     7.40 $ & $     3.20 $ & $     7.70 $ & $   0.123 $\\
$ 1557.05533 $ & $   240.83 $ & $    24.60 $ & $     5.10 $ & $    18.40 $ & $   0.878 $\\
$ 1558.95741 $ & $  -355.47 $ & $    10.50 $ & $     4.30 $ & $     8.70 $ & $   0.311 $\\
$ 1559.99613 $ & $  -199.97 $ & $    17.70 $ & $   -14.10 $ & $    17.40 $ & $   0.093 $\\
$ 1576.04204 $ & $  -326.97 $ & $    16.70 $ & \nodata      & \nodata      & $   0.182 $\\
$ 1576.91790 $ & $   331.53 $ & $    14.40 $ & \nodata      & \nodata      & $   0.842 $\\
$ 1578.04243 $ & $   265.83 $ & $     7.40 $ & \nodata      & \nodata      & $   0.689 $\\
$ 1579.96119 $ & $  -277.57 $ & $     9.00 $ & \nodata      & \nodata      & $   0.135 $\\
$ 1580.92488 $ & $   257.33 $ & $    12.40 $ & \nodata      & \nodata      & $   0.861 $\\


==> data/HTR340-006_phfu_tab.old.tex <==
$ 55338.79359 $ & $  -0.00005 $ & $   0.00080 $ & $  10.12720 $ & $ i$\\
$ 55338.79427 $ & $  -0.00125 $ & $   0.00080 $ & $  10.12640 $ & $ i$\\
$ 55338.79494 $ & $   0.00250 $ & $   0.00080 $ & $  10.12910 $ & $ i$\\
$ 55338.79563 $ & $  -0.00056 $ & $   0.00080 $ & $  10.12660 $ & $ i$\\
$ 55338.79633 $ & $   0.00149 $ & $   0.00080 $ & $  10.12850 $ & $ i$\\
$ 55338.79701 $ & $   0.00026 $ & $   0.00079 $ & $  10.12720 $ & $ i$\\
$ 55338.79769 $ & $  -0.00254 $ & $   0.00079 $ & $  10.12440 $ & $ i$\\
$ 55338.79837 $ & $  -0.00311 $ & $   0.00079 $ & $  10.12340 $ & $ i$\\
$ 55338.79905 $ & $   0.00175 $ & $   0.00079 $ & $  10.12940 $ & $ i$\\
$ 55338.79969 $ & $   0.00178 $ & $   0.00079 $ & $  10.12900 $ & $ i$\\
$ 55338.80036 $ & $  -0.00107 $ & $   0.00078 $ & $  10.12570 $ & $ i$\\
$ 55338.80103 $ & $  -0.00235 $ & $   0.00078 $ & $  10.12470 $ & $ i$\\
$ 55338.80170 $ & $  -0.00156 $ & $   0.00078 $ & $  10.12600 $ & $ i$\\
$ 55338.80239 $ & $  -0.00229 $ & $   0.00078 $ & $  10.12530 $ & $ i$\\
$ 55338.80307 $ & $   0.00137 $ & $   0.00078 $ & $  10.12940 $ & $ i$\\
$ 55338.80377 $ & $   0.00060 $ & $   0.00078 $ & $  10.12790 $ & $ i$\\
$ 55338.80445 $ & $  -0.00029 $ & $   0.00078 $ & $  10.12690 $ & $ i$\\
$ 55338.80514 $ & $  -0.00008 $ & $   0.00078 $ & $  10.12670 $ & $ i$\\
$ 55338.80581 $ & $   0.00185 $ & $   0.00078 $ & $  10.12890 $ & $ i$\\
$ 55338.80649 $ & $   0.00171 $ & $   0.00078 $ & $  10.12920 $ & $ i$\\
$ 55338.80719 $ & $  -0.00026 $ & $   0.00078 $ & $  10.12710 $ & $ i$\\
$ 55338.80787 $ & $   0.00247 $ & $   0.00078 $ & $  10.13010 $ & $ i$\\
$ 55338.80854 $ & $   0.00224 $ & $   0.00078 $ & $  10.13020 $ & $ i$\\
$ 55338.80991 $ & $  -0.00355 $ & $   0.00077 $ & $  10.12390 $ & $ i$\\
$ 55338.81059 $ & $  -0.00142 $ & $   0.00077 $ & $  10.12570 $ & $ i$\\
$ 55338.81126 $ & $  -0.00001 $ & $   0.00077 $ & $  10.12720 $ & $ i$\\
$ 55338.81194 $ & $   0.00072 $ & $   0.00077 $ & $  10.12800 $ & $ i$\\
$ 55338.81263 $ & $   0.00221 $ & $   0.00077 $ & $  10.12890 $ & $ i$\\
$ 55338.81327 $ & $  -0.00169 $ & $   0.00077 $ & $  10.12530 $ & $ i$\\
$ 55338.81397 $ & $  -0.00101 $ & $   0.00077 $ & $  10.12650 $ & $ i$\\
$ 55338.81468 $ & $   0.00079 $ & $   0.00077 $ & $  10.12800 $ & $ i$\\
$ 55338.81537 $ & $  -0.00163 $ & $   0.00077 $ & $  10.12540 $ & $ i$\\
$ 55338.81605 $ & $   0.00329 $ & $   0.00077 $ & $  10.13030 $ & $ i$\\
$ 55338.81672 $ & $   0.00379 $ & $   0.00077 $ & $  10.13070 $ & $ i$\\
$ 55338.81740 $ & $  -0.00061 $ & $   0.00076 $ & $  10.12590 $ & $ i$\\
$ 55338.81808 $ & $  -0.00293 $ & $   0.00076 $ & $  10.12380 $ & $ i$\\
$ 55338.81876 $ & $  -0.00305 $ & $   0.00076 $ & $  10.12340 $ & $ i$\\
$ 55338.81944 $ & $  -0.00032 $ & $   0.00076 $ & $  10.12640 $ & $ i$\\
$ 55338.82013 $ & $   0.00199 $ & $   0.00076 $ & $  10.12860 $ & $ i$\\
$ 55338.82079 $ & $   0.00294 $ & $   0.00076 $ & $  10.13020 $ & $ i$\\
$ 55338.82146 $ & $  -0.00020 $ & $   0.00076 $ & $  10.12700 $ & $ i$\\
$ 55338.82214 $ & $  -0.00202 $ & $   0.00076 $ & $  10.12500 $ & $ i$\\
$ 55338.82281 $ & $   0.00104 $ & $   0.00076 $ & $  10.12790 $ & $ i$\\
$ 55338.82348 $ & $   0.00044 $ & $   0.00076 $ & $  10.12790 $ & $ i$\\
$ 55338.82415 $ & $  -0.00020 $ & $   0.00076 $ & $  10.12660 $ & $ i$\\
$ 55338.82485 $ & $  -0.00336 $ & $   0.00076 $ & $  10.12300 $ & $ i$\\
$ 55338.82553 $ & $  -0.00240 $ & $   0.00076 $ & $  10.12470 $ & $ i$\\
$ 55338.82624 $ & $  -0.00163 $ & $   0.00076 $ & $  10.12570 $ & $ i$\\
$ 55338.82692 $ & $   0.00107 $ & $   0.00076 $ & $  10.12790 $ & $ i$\\
$ 55338.82760 $ & $   0.00211 $ & $   0.00076 $ & $  10.12830 $ & $ i$\\
$ 55338.82830 $ & $   0.00089 $ & $   0.00076 $ & $  10.12790 $ & $ i$\\
$ 55338.82898 $ & $  -0.00134 $ & $   0.00075 $ & $  10.12540 $ & $ i$\\
$ 55338.82965 $ & $  -0.00183 $ & $   0.00076 $ & $  10.12540 $ & $ i$\\
$ 55338.83034 $ & $   0.00235 $ & $   0.00076 $ & $  10.12930 $ & $ i$\\
$ 55338.83100 $ & $   0.00301 $ & $   0.00076 $ & $  10.13040 $ & $ i$\\
$ 55338.83169 $ & $  -0.00206 $ & $   0.00075 $ & $  10.12490 $ & $ i$\\
$ 55338.83238 $ & $   0.00361 $ & $   0.00075 $ & $  10.12990 $ & $ i$\\
$ 55338.83306 $ & $   0.00399 $ & $   0.00075 $ & $  10.13080 $ & $ i$\\
$ 55338.83373 $ & $   0.00090 $ & $   0.00075 $ & $  10.12790 $ & $ i$\\
$ 55338.83440 $ & $   0.00095 $ & $   0.00075 $ & $  10.12710 $ & $ i$\\
$ 55338.83507 $ & $   0.00299 $ & $   0.00076 $ & $  10.13000 $ & $ i$\\
$ 55338.83582 $ & $   0.00415 $ & $   0.00076 $ & $  10.13140 $ & $ i$\\
$ 55338.83652 $ & $   0.00590 $ & $   0.00076 $ & $  10.13300 $ & $ i$\\
$ 55338.83719 $ & $   0.00471 $ & $   0.00076 $ & $  10.13200 $ & $ i$\\
$ 55338.83786 $ & $   0.00418 $ & $   0.00075 $ & $  10.13080 $ & $ i$\\
$ 55338.83853 $ & $   0.00356 $ & $   0.00075 $ & $  10.13030 $ & $ i$\\
$ 55338.83921 $ & $   0.00605 $ & $   0.00075 $ & $  10.13190 $ & $ i$\\
$ 55338.83991 $ & $   0.00761 $ & $   0.00075 $ & $  10.13420 $ & $ i$\\
$ 55338.84059 $ & $   0.00766 $ & $   0.00075 $ & $  10.13410 $ & $ i$\\
$ 55338.84126 $ & $   0.00614 $ & $   0.00075 $ & $  10.13270 $ & $ i$\\
$ 55338.84195 $ & $   0.00842 $ & $   0.00075 $ & $  10.13420 $ & $ i$\\
$ 55338.84264 $ & $   0.00783 $ & $   0.00075 $ & $  10.13390 $ & $ i$\\
$ 55338.84331 $ & $   0.00958 $ & $   0.00075 $ & $  10.13560 $ & $ i$\\
$ 55338.84399 $ & $   0.00929 $ & $   0.00075 $ & $  10.13490 $ & $ i$\\
$ 55338.84467 $ & $   0.00816 $ & $   0.00075 $ & $  10.13370 $ & $ i$\\
$ 55338.84535 $ & $   0.00718 $ & $   0.00075 $ & $  10.13260 $ & $ i$\\
$ 55338.84603 $ & $   0.00869 $ & $   0.00075 $ & $  10.13420 $ & $ i$\\
$ 55338.84671 $ & $   0.00803 $ & $   0.00075 $ & $  10.13370 $ & $ i$\\
$ 55338.84739 $ & $   0.00811 $ & $   0.00075 $ & $  10.13350 $ & $ i$\\
$ 55338.84807 $ & $   0.00872 $ & $   0.00074 $ & $  10.13390 $ & $ i$\\
$ 55338.84876 $ & $   0.00875 $ & $   0.00074 $ & $  10.13410 $ & $ i$\\
$ 55338.84943 $ & $   0.00600 $ & $   0.00074 $ & $  10.13140 $ & $ i$\\
$ 55338.85013 $ & $   0.00644 $ & $   0.00074 $ & $  10.13200 $ & $ i$\\
$ 55338.85080 $ & $   0.00785 $ & $   0.00075 $ & $  10.13440 $ & $ i$\\
$ 55338.85151 $ & $   0.00909 $ & $   0.00074 $ & $  10.13530 $ & $ i$\\
$ 55338.85215 $ & $   0.00688 $ & $   0.00074 $ & $  10.13210 $ & $ i$\\
$ 55338.85284 $ & $   0.00725 $ & $   0.00074 $ & $  10.13210 $ & $ i$\\
$ 55338.85352 $ & $   0.00700 $ & $   0.00074 $ & $  10.13260 $ & $ i$\\
$ 55338.85419 $ & $   0.00751 $ & $   0.00074 $ & $  10.13330 $ & $ i$\\
$ 55338.85486 $ & $   0.00654 $ & $   0.00074 $ & $  10.13200 $ & $ i$\\
$ 55338.85555 $ & $   0.00721 $ & $   0.00074 $ & $  10.13260 $ & $ i$\\
$ 55338.85628 $ & $   0.00711 $ & $   0.00074 $ & $  10.13230 $ & $ i$\\
$ 55338.85697 $ & $   0.00706 $ & $   0.00074 $ & $  10.13270 $ & $ i$\\
$ 55338.85764 $ & $   0.00817 $ & $   0.00074 $ & $  10.13320 $ & $ i$\\
$ 55338.85831 $ & $   0.00658 $ & $   0.00074 $ & $  10.13210 $ & $ i$\\
$ 55338.85900 $ & $   0.00644 $ & $   0.00074 $ & $  10.13210 $ & $ i$\\
$ 55338.85967 $ & $   0.00561 $ & $   0.00074 $ & $  10.13180 $ & $ i$\\
$ 55338.86035 $ & $   0.00830 $ & $   0.00074 $ & $  10.13420 $ & $ i$\\
$ 55338.86103 $ & $   0.00666 $ & $   0.00074 $ & $  10.13230 $ & $ i$\\
$ 55338.86172 $ & $   0.00536 $ & $   0.00074 $ & $  10.13070 $ & $ i$\\
$ 55338.86239 $ & $   0.00697 $ & $   0.00074 $ & $  10.13240 $ & $ i$\\
$ 55338.86307 $ & $   0.00737 $ & $   0.00074 $ & $  10.13250 $ & $ i$\\
$ 55338.86374 $ & $   0.00602 $ & $   0.00074 $ & $  10.13100 $ & $ i$\\
$ 55338.86442 $ & $   0.00547 $ & $   0.00074 $ & $  10.13080 $ & $ i$\\
$ 55338.86512 $ & $   0.00708 $ & $   0.00074 $ & $  10.13290 $ & $ i$\\
$ 55338.86581 $ & $   0.00573 $ & $   0.00074 $ & $  10.13160 $ & $ i$\\
$ 55338.86650 $ & $   0.00530 $ & $   0.00074 $ & $  10.13070 $ & $ i$\\
$ 55338.86716 $ & $   0.00712 $ & $   0.00073 $ & $  10.13270 $ & $ i$\\
$ 55338.86784 $ & $   0.00602 $ & $   0.00073 $ & $  10.13150 $ & $ i$\\
$ 55338.86851 $ & $   0.00902 $ & $   0.00074 $ & $  10.13400 $ & $ i$\\
$ 55338.86918 $ & $   0.00737 $ & $   0.00074 $ & $  10.13290 $ & $ i$\\
$ 55338.86985 $ & $   0.00808 $ & $   0.00074 $ & $  10.13350 $ & $ i$\\
$ 55338.87054 $ & $   0.00769 $ & $   0.00074 $ & $  10.13320 $ & $ i$\\
$ 55338.87121 $ & $   0.00873 $ & $   0.00074 $ & $  10.13460 $ & $ i$\\
$ 55338.87188 $ & $   0.00891 $ & $   0.00073 $ & $  10.13390 $ & $ i$\\
$ 55338.87257 $ & $   0.00712 $ & $   0.00073 $ & $  10.13240 $ & $ i$\\
$ 55338.87326 $ & $   0.00691 $ & $   0.00074 $ & $  10.13240 $ & $ i$\\
$ 55338.87392 $ & $   0.00609 $ & $   0.00074 $ & $  10.13250 $ & $ i$\\
$ 55338.87459 $ & $   0.00795 $ & $   0.00074 $ & $  10.13440 $ & $ i$\\
$ 55338.87527 $ & $   0.00703 $ & $   0.00074 $ & $  10.13330 $ & $ i$\\
$ 55338.87594 $ & $   0.00659 $ & $   0.00074 $ & $  10.13300 $ & $ i$\\
$ 55338.87668 $ & $   0.00790 $ & $   0.00074 $ & $  10.13430 $ & $ i$\\
$ 55338.87736 $ & $   0.00720 $ & $   0.00074 $ & $  10.13330 $ & $ i$\\
$ 55338.87804 $ & $   0.00631 $ & $   0.00074 $ & $  10.13260 $ & $ i$\\
$ 55338.87871 $ & $   0.00816 $ & $   0.00074 $ & $  10.13450 $ & $ i$\\
$ 55338.87937 $ & $   0.00895 $ & $   0.00074 $ & $  10.13500 $ & $ i$\\
$ 55338.88004 $ & $   0.00833 $ & $   0.00074 $ & $  10.13520 $ & $ i$\\
$ 55338.88073 $ & $   0.00801 $ & $   0.00074 $ & $  10.13390 $ & $ i$\\
$ 55338.88143 $ & $   0.00756 $ & $   0.00074 $ & $  10.13440 $ & $ i$\\
$ 55338.88210 $ & $   0.00603 $ & $   0.00074 $ & $  10.13270 $ & $ i$\\
$ 55338.88278 $ & $   0.00779 $ & $   0.00074 $ & $  10.13430 $ & $ i$\\
$ 55338.88344 $ & $   0.00421 $ & $   0.00074 $ & $  10.13100 $ & $ i$\\
$ 55338.88410 $ & $   0.00873 $ & $   0.00073 $ & $  10.13430 $ & $ i$\\
$ 55338.88474 $ & $   0.00830 $ & $   0.00073 $ & $  10.13420 $ & $ i$\\
$ 55338.88543 $ & $   0.00726 $ & $   0.00073 $ & $  10.13340 $ & $ i$\\
$ 55338.88608 $ & $   0.00817 $ & $   0.00073 $ & $  10.13430 $ & $ i$\\
$ 55338.88676 $ & $   0.01045 $ & $   0.00074 $ & $  10.13690 $ & $ i$\\
$ 55338.88745 $ & $   0.00868 $ & $   0.00074 $ & $  10.13480 $ & $ i$\\
$ 55338.88813 $ & $   0.00819 $ & $   0.00073 $ & $  10.13430 $ & $ i$\\
$ 55338.88881 $ & $   0.00912 $ & $   0.00074 $ & $  10.13520 $ & $ i$\\
$ 55338.88947 $ & $   0.00799 $ & $   0.00074 $ & $  10.13450 $ & $ i$\\
$ 55338.89014 $ & $   0.00711 $ & $   0.00074 $ & $  10.13340 $ & $ i$\\
$ 55338.89083 $ & $   0.00768 $ & $   0.00074 $ & $  10.13410 $ & $ i$\\
$ 55338.89152 $ & $   0.00753 $ & $   0.00074 $ & $  10.13410 $ & $ i$\\
$ 55338.89220 $ & $   0.00751 $ & $   0.00073 $ & $  10.13350 $ & $ i$\\
$ 55338.89289 $ & $   0.00765 $ & $   0.00073 $ & $  10.13350 $ & $ i$\\
$ 55338.89353 $ & $   0.00794 $ & $   0.00073 $ & $  10.13410 $ & $ i$\\
$ 55338.89422 $ & $   0.00570 $ & $   0.00074 $ & $  10.13280 $ & $ i$\\
$ 55338.89490 $ & $   0.00749 $ & $   0.00074 $ & $  10.13460 $ & $ i$\\
$ 55338.89556 $ & $   0.00698 $ & $   0.00073 $ & $  10.13370 $ & $ i$\\
$ 55338.89626 $ & $   0.00743 $ & $   0.00073 $ & $  10.13330 $ & $ i$\\
$ 55338.89700 $ & $   0.00767 $ & $   0.00073 $ & $  10.13380 $ & $ i$\\
$ 55338.89768 $ & $   0.00624 $ & $   0.00073 $ & $  10.13170 $ & $ i$\\
$ 55338.89837 $ & $   0.00912 $ & $   0.00073 $ & $  10.13520 $ & $ i$\\
$ 55338.89906 $ & $   0.00747 $ & $   0.00074 $ & $  10.13460 $ & $ i$\\
$ 55338.89973 $ & $   0.00924 $ & $   0.00074 $ & $  10.13600 $ & $ i$\\
$ 55338.90041 $ & $   0.00845 $ & $   0.00073 $ & $  10.13440 $ & $ i$\\
$ 55338.90107 $ & $   0.00795 $ & $   0.00073 $ & $  10.13380 $ & $ i$\\
$ 55338.90176 $ & $   0.00871 $ & $   0.00073 $ & $  10.13430 $ & $ i$\\
$ 55338.90245 $ & $   0.00857 $ & $   0.00073 $ & $  10.13410 $ & $ i$\\
$ 55338.90312 $ & $   0.00825 $ & $   0.00073 $ & $  10.13380 $ & $ i$\\
$ 55338.90379 $ & $   0.00817 $ & $   0.00073 $ & $  10.13390 $ & $ i$\\
$ 55338.90447 $ & $   0.00740 $ & $   0.00073 $ & $  10.13320 $ & $ i$\\
$ 55338.90513 $ & $   0.00572 $ & $   0.00073 $ & $  10.13200 $ & $ i$\\
$ 55338.90582 $ & $   0.00716 $ & $   0.00073 $ & $  10.13280 $ & $ i$\\
$ 55338.90650 $ & $   0.00785 $ & $   0.00072 $ & $  10.13290 $ & $ i$\\
$ 55338.90718 $ & $   0.00707 $ & $   0.00073 $ & $  10.13240 $ & $ i$\\
$ 55338.90784 $ & $   0.00776 $ & $   0.00073 $ & $  10.13340 $ & $ i$\\
$ 55338.90851 $ & $   0.00735 $ & $   0.00073 $ & $  10.13320 $ & $ i$\\
$ 55338.90920 $ & $   0.00852 $ & $   0.00073 $ & $  10.13390 $ & $ i$\\
$ 55338.90988 $ & $   0.00746 $ & $   0.00073 $ & $  10.13300 $ & $ i$\\
$ 55338.91056 $ & $   0.00877 $ & $   0.00073 $ & $  10.13370 $ & $ i$\\
$ 55338.91123 $ & $   0.00790 $ & $   0.00073 $ & $  10.13360 $ & $ i$\\
$ 55338.91190 $ & $   0.00876 $ & $   0.00073 $ & $  10.13470 $ & $ i$\\
$ 55338.91259 $ & $   0.00824 $ & $   0.00074 $ & $  10.13500 $ & $ i$\\
$ 55338.91326 $ & $   0.00772 $ & $   0.00073 $ & $  10.13400 $ & $ i$\\
$ 55338.91393 $ & $   0.00949 $ & $   0.00076 $ & $  10.13790 $ & $ i$\\
$ 55338.91459 $ & $   0.00832 $ & $   0.00075 $ & $  10.13530 $ & $ i$\\
$ 55338.91526 $ & $   0.00764 $ & $   0.00073 $ & $  10.13370 $ & $ i$\\
$ 55338.91594 $ & $   0.00826 $ & $   0.00073 $ & $  10.13420 $ & $ i$\\
$ 55338.91663 $ & $   0.00670 $ & $   0.00074 $ & $  10.13330 $ & $ i$\\
$ 55338.91734 $ & $   0.00859 $ & $   0.00074 $ & $  10.13540 $ & $ i$\\
$ 55338.91800 $ & $   0.00798 $ & $   0.00073 $ & $  10.13400 $ & $ i$\\
$ 55338.91868 $ & $   0.00894 $ & $   0.00073 $ & $  10.13420 $ & $ i$\\
$ 55338.91936 $ & $   0.00792 $ & $   0.00074 $ & $  10.13430 $ & $ i$\\
$ 55338.92003 $ & $   0.00904 $ & $   0.00074 $ & $  10.13520 $ & $ i$\\
$ 55338.92071 $ & $   0.00776 $ & $   0.00073 $ & $  10.13370 $ & $ i$\\
$ 55338.92142 $ & $   0.00678 $ & $   0.00073 $ & $  10.13280 $ & $ i$\\
$ 55338.92209 $ & $   0.00869 $ & $   0.00073 $ & $  10.13490 $ & $ i$\\
$ 55338.92277 $ & $   0.00884 $ & $   0.00073 $ & $  10.13430 $ & $ i$\\
$ 55338.92346 $ & $   0.00859 $ & $   0.00073 $ & $  10.13380 $ & $ i$\\
$ 55338.92414 $ & $   0.00909 $ & $   0.00073 $ & $  10.13460 $ & $ i$\\
$ 55338.92483 $ & $   0.00776 $ & $   0.00074 $ & $  10.13420 $ & $ i$\\
$ 55338.92552 $ & $   0.00661 $ & $   0.00073 $ & $  10.13260 $ & $ i$\\
$ 55338.92618 $ & $   0.00831 $ & $   0.00073 $ & $  10.13400 $ & $ i$\\
$ 55338.92686 $ & $   0.00715 $ & $   0.00073 $ & $  10.13200 $ & $ i$\\
$ 55338.92753 $ & $   0.00895 $ & $   0.00073 $ & $  10.13430 $ & $ i$\\
$ 55338.92820 $ & $   0.00801 $ & $   0.00073 $ & $  10.13360 $ & $ i$\\
$ 55338.92887 $ & $   0.00985 $ & $   0.00073 $ & $  10.13520 $ & $ i$\\
$ 55338.92957 $ & $   0.00773 $ & $   0.00073 $ & $  10.13330 $ & $ i$\\
$ 55338.93025 $ & $   0.00875 $ & $   0.00073 $ & $  10.13400 $ & $ i$\\
$ 55338.93093 $ & $   0.00789 $ & $   0.00073 $ & $  10.13380 $ & $ i$\\
$ 55338.93159 $ & $   0.00790 $ & $   0.00073 $ & $  10.13270 $ & $ i$\\
$ 55338.93228 $ & $   0.00747 $ & $   0.00073 $ & $  10.13250 $ & $ i$\\
$ 55338.93296 $ & $   0.00772 $ & $   0.00073 $ & $  10.13310 $ & $ i$\\
$ 55338.93364 $ & $   0.00930 $ & $   0.00073 $ & $  10.13470 $ & $ i$\\
$ 55338.93431 $ & $   0.00797 $ & $   0.00073 $ & $  10.13290 $ & $ i$\\
$ 55338.93502 $ & $   0.00823 $ & $   0.00073 $ & $  10.13290 $ & $ i$\\
$ 55338.93569 $ & $   0.00693 $ & $   0.00073 $ & $  10.13260 $ & $ i$\\
$ 55338.93635 $ & $   0.00827 $ & $   0.00073 $ & $  10.13340 $ & $ i$\\
$ 55338.93703 $ & $   0.00889 $ & $   0.00073 $ & $  10.13400 $ & $ i$\\
$ 55338.93777 $ & $   0.00697 $ & $   0.00073 $ & $  10.13210 $ & $ i$\\
$ 55338.93845 $ & $   0.00691 $ & $   0.00073 $ & $  10.13200 $ & $ i$\\
$ 55338.93912 $ & $   0.00722 $ & $   0.00073 $ & $  10.13230 $ & $ i$\\
$ 55338.93979 $ & $   0.00767 $ & $   0.00073 $ & $  10.13280 $ & $ i$\\
$ 55338.94048 $ & $   0.00839 $ & $   0.00073 $ & $  10.13300 $ & $ i$\\
$ 55338.94117 $ & $   0.00636 $ & $   0.00072 $ & $  10.13130 $ & $ i$\\
$ 55338.94187 $ & $   0.00743 $ & $   0.00072 $ & $  10.13250 $ & $ i$\\
$ 55338.94254 $ & $   0.00703 $ & $   0.00073 $ & $  10.13190 $ & $ i$\\
$ 55338.94323 $ & $   0.00840 $ & $   0.00072 $ & $  10.13270 $ & $ i$\\
$ 55338.94392 $ & $   0.00641 $ & $   0.00073 $ & $  10.13190 $ & $ i$\\
$ 55338.94458 $ & $   0.00713 $ & $   0.00073 $ & $  10.13230 $ & $ i$\\
$ 55338.94525 $ & $   0.00733 $ & $   0.00073 $ & $  10.13200 $ & $ i$\\
$ 55338.94593 $ & $   0.00796 $ & $   0.00072 $ & $  10.13270 $ & $ i$\\
$ 55338.94663 $ & $   0.00766 $ & $   0.00072 $ & $  10.13200 $ & $ i$\\
$ 55338.94730 $ & $   0.00456 $ & $   0.00073 $ & $  10.13000 $ & $ i$\\
$ 55338.94798 $ & $   0.00796 $ & $   0.00072 $ & $  10.13250 $ & $ i$\\
$ 55338.94867 $ & $   0.00810 $ & $   0.00072 $ & $  10.13270 $ & $ i$\\
$ 55338.94935 $ & $   0.00567 $ & $   0.00072 $ & $  10.13060 $ & $ i$\\
$ 55338.95001 $ & $   0.00484 $ & $   0.00072 $ & $  10.12960 $ & $ i$\\
$ 55338.95069 $ & $   0.00551 $ & $   0.00072 $ & $  10.13040 $ & $ i$\\
$ 55338.95139 $ & $   0.00725 $ & $   0.00072 $ & $  10.13230 $ & $ i$\\
$ 55338.95207 $ & $   0.00619 $ & $   0.00073 $ & $  10.13110 $ & $ i$\\
$ 55338.95275 $ & $   0.00690 $ & $   0.00073 $ & $  10.13160 $ & $ i$\\
$ 55338.95341 $ & $   0.00607 $ & $   0.00073 $ & $  10.13110 $ & $ i$\\
$ 55338.95411 $ & $   0.00808 $ & $   0.00073 $ & $  10.13270 $ & $ i$\\
$ 55338.95480 $ & $   0.00920 $ & $   0.00073 $ & $  10.13430 $ & $ i$\\
$ 55338.95547 $ & $   0.00818 $ & $   0.00073 $ & $  10.13300 $ & $ i$\\
$ 55338.95613 $ & $   0.00448 $ & $   0.00072 $ & $  10.12910 $ & $ i$\\
$ 55338.95682 $ & $   0.00687 $ & $   0.00072 $ & $  10.13160 $ & $ i$\\
$ 55338.95750 $ & $   0.00651 $ & $   0.00073 $ & $  10.13180 $ & $ i$\\
$ 55338.95823 $ & $   0.00571 $ & $   0.00073 $ & $  10.13080 $ & $ i$\\
$ 55338.95890 $ & $   0.00543 $ & $   0.00072 $ & $  10.13010 $ & $ i$\\
$ 55338.95959 $ & $   0.00457 $ & $   0.00072 $ & $  10.12950 $ & $ i$\\
$ 55338.96025 $ & $   0.00642 $ & $   0.00072 $ & $  10.13160 $ & $ i$\\
$ 55338.96094 $ & $   0.00529 $ & $   0.00072 $ & $  10.13090 $ & $ i$\\
$ 55338.96162 $ & $   0.00547 $ & $   0.00072 $ & $  10.13040 $ & $ i$\\
$ 55338.96231 $ & $   0.00597 $ & $   0.00073 $ & $  10.13150 $ & $ i$\\
$ 55338.96298 $ & $   0.00664 $ & $   0.00073 $ & $  10.13240 $ & $ i$\\
$ 55338.96366 $ & $   0.00566 $ & $   0.00074 $ & $  10.13220 $ & $ i$\\
$ 55338.96433 $ & $   0.00372 $ & $   0.00073 $ & $  10.13070 $ & $ i$\\
$ 55338.96501 $ & $   0.00547 $ & $   0.00072 $ & $  10.13090 $ & $ i$\\
$ 55338.96568 $ & $   0.00233 $ & $   0.00073 $ & $  10.12780 $ & $ i$\\
$ 55338.96635 $ & $   0.00520 $ & $   0.00072 $ & $  10.12990 $ & $ i$\\
$ 55338.96705 $ & $   0.00263 $ & $   0.00073 $ & $  10.12900 $ & $ i$\\
$ 55338.96773 $ & $   0.00154 $ & $   0.00073 $ & $  10.12760 $ & $ i$\\
$ 55338.96842 $ & $   0.00335 $ & $   0.00073 $ & $  10.12960 $ & $ i$\\
$ 55338.96907 $ & $   0.00092 $ & $   0.00072 $ & $  10.12630 $ & $ i$\\
$ 55338.96973 $ & $   0.00397 $ & $   0.00073 $ & $  10.12930 $ & $ i$\\
$ 55338.97042 $ & $   0.00073 $ & $   0.00072 $ & $  10.12620 $ & $ i$\\
$ 55338.97110 $ & $   0.00247 $ & $   0.00072 $ & $  10.12760 $ & $ i$\\
$ 55338.97178 $ & $   0.00010 $ & $   0.00072 $ & $  10.12520 $ & $ i$\\
$ 55480.59376 $ & $   0.00133 $ & $   0.00080 $ & $   9.13948 $ & $  $\\
$ 55480.59409 $ & $   0.00303 $ & $   0.00080 $ & $   9.14170 $ & $  $\\
$ 55480.59441 $ & $  -0.00152 $ & $   0.00080 $ & $   9.13698 $ & $  $\\
$ 55480.59475 $ & $  -0.00043 $ & $   0.00079 $ & $   9.13803 $ & $  $\\
$ 55480.59510 $ & $   0.00095 $ & $   0.00080 $ & $   9.13926 $ & $  $\\
$ 55480.59542 $ & $  -0.00251 $ & $   0.00080 $ & $   9.13627 $ & $  $\\
$ 55480.59575 $ & $  -0.00161 $ & $   0.00080 $ & $   9.13636 $ & $  $\\
$ 55480.59609 $ & $  -0.00018 $ & $   0.00080 $ & $   9.13811 $ & $  $\\
$ 55480.59643 $ & $  -0.00134 $ & $   0.00080 $ & $   9.13751 $ & $  $\\
$ 55480.59679 $ & $   0.00044 $ & $   0.00080 $ & $   9.13874 $ & $  $\\
$ 55480.59711 $ & $   0.00225 $ & $   0.00080 $ & $   9.14054 $ & $  $\\
$ 55480.59744 $ & $   0.00059 $ & $   0.00080 $ & $   9.13862 $ & $  $\\
$ 55480.59777 $ & $  -0.00029 $ & $   0.00080 $ & $   9.13862 $ & $  $\\
$ 55480.59811 $ & $  -0.00087 $ & $   0.00080 $ & $   9.13798 $ & $  $\\
$ 55480.59843 $ & $  -0.00022 $ & $   0.00079 $ & $   9.13825 $ & $  $\\
$ 55480.59876 $ & $   0.00080 $ & $   0.00080 $ & $   9.13951 $ & $  $\\
$ 55480.59909 $ & $  -0.00078 $ & $   0.00080 $ & $   9.13769 $ & $  $\\
$ 55480.59943 $ & $  -0.00113 $ & $   0.00080 $ & $   9.13738 $ & $  $\\
$ 55480.59976 $ & $   0.00311 $ & $   0.00080 $ & $   9.14210 $ & $  $\\
$ 55480.60010 $ & $   0.00262 $ & $   0.00080 $ & $   9.14148 $ & $  $\\
$ 55480.60041 $ & $  -0.00062 $ & $   0.00080 $ & $   9.13780 $ & $  $\\
$ 55480.60076 $ & $   0.00280 $ & $   0.00080 $ & $   9.14128 $ & $  $\\
$ 55480.60108 $ & $   0.00105 $ & $   0.00080 $ & $   9.13999 $ & $  $\\
$ 55480.60142 $ & $   0.00221 $ & $   0.00080 $ & $   9.14099 $ & $  $\\
$ 55480.60174 $ & $   0.00159 $ & $   0.00080 $ & $   9.14092 $ & $  $\\
$ 55480.60209 $ & $   0.00203 $ & $   0.00080 $ & $   9.14026 $ & $  $\\
$ 55480.60242 $ & $   0.00159 $ & $   0.00080 $ & $   9.14004 $ & $  $\\
$ 55480.60275 $ & $   0.00210 $ & $   0.00080 $ & $   9.14086 $ & $  $\\
$ 55480.60308 $ & $   0.00359 $ & $   0.00080 $ & $   9.14178 $ & $  $\\
$ 55480.60342 $ & $   0.00164 $ & $   0.00080 $ & $   9.14054 $ & $  $\\
$ 55480.60374 $ & $   0.00561 $ & $   0.00080 $ & $   9.14462 $ & $  $\\
$ 55480.60408 $ & $   0.00314 $ & $   0.00080 $ & $   9.14156 $ & $  $\\
$ 55480.60440 $ & $   0.00574 $ & $   0.00080 $ & $   9.14452 $ & $  $\\
$ 55480.60475 $ & $   0.00522 $ & $   0.00080 $ & $   9.14383 $ & $  $\\
$ 55480.60507 $ & $   0.00378 $ & $   0.00080 $ & $   9.14193 $ & $  $\\
$ 55480.60540 $ & $   0.00410 $ & $   0.00080 $ & $   9.14236 $ & $  $\\
$ 55480.60575 $ & $   0.00330 $ & $   0.00080 $ & $   9.14224 $ & $  $\\
$ 55480.60608 $ & $   0.00434 $ & $   0.00080 $ & $   9.14317 $ & $  $\\
$ 55480.60639 $ & $   0.00670 $ & $   0.00080 $ & $   9.14515 $ & $  $\\
$ 55480.60673 $ & $   0.00531 $ & $   0.00080 $ & $   9.14405 $ & $  $\\
$ 55480.60705 $ & $   0.00660 $ & $   0.00080 $ & $   9.14494 $ & $  $\\
$ 55480.60739 $ & $   0.00287 $ & $   0.00080 $ & $   9.14176 $ & $  $\\
$ 55480.60771 $ & $   0.00448 $ & $   0.00080 $ & $   9.14303 $ & $  $\\
$ 55480.60805 $ & $   0.00535 $ & $   0.00080 $ & $   9.14429 $ & $  $\\
$ 55480.60836 $ & $   0.00417 $ & $   0.00080 $ & $   9.14309 $ & $  $\\
$ 55480.60870 $ & $   0.00557 $ & $   0.00080 $ & $   9.14427 $ & $  $\\
$ 55480.60903 $ & $   0.00850 $ & $   0.00080 $ & $   9.14737 $ & $  $\\
$ 55480.60936 $ & $   0.00722 $ & $   0.00080 $ & $   9.14607 $ & $  $\\
$ 55480.60970 $ & $   0.00908 $ & $   0.00080 $ & $   9.14818 $ & $  $\\
$ 55480.61004 $ & $   0.00769 $ & $   0.00080 $ & $   9.14656 $ & $  $\\
$ 55480.61037 $ & $   0.00597 $ & $   0.00080 $ & $   9.14453 $ & $  $\\
$ 55480.61070 $ & $   0.00659 $ & $   0.00080 $ & $   9.14551 $ & $  $\\
$ 55480.61102 $ & $   0.00679 $ & $   0.00080 $ & $   9.14581 $ & $  $\\
$ 55480.61136 $ & $   0.00697 $ & $   0.00080 $ & $   9.14554 $ & $  $\\
$ 55480.61169 $ & $   0.01018 $ & $   0.00080 $ & $   9.14917 $ & $  $\\
$ 55480.61204 $ & $   0.00591 $ & $   0.00080 $ & $   9.14435 $ & $  $\\
$ 55480.61235 $ & $   0.00686 $ & $   0.00080 $ & $   9.14593 $ & $  $\\
$ 55480.61270 $ & $   0.00555 $ & $   0.00080 $ & $   9.14497 $ & $  $\\
$ 55480.61302 $ & $   0.00791 $ & $   0.00080 $ & $   9.14701 $ & $  $\\
$ 55480.61336 $ & $   0.00872 $ & $   0.00080 $ & $   9.14775 $ & $  $\\
$ 55480.61370 $ & $   0.00447 $ & $   0.00080 $ & $   9.14372 $ & $  $\\
$ 55480.61404 $ & $   0.00450 $ & $   0.00080 $ & $   9.14388 $ & $  $\\
$ 55480.61438 $ & $   0.00759 $ & $   0.00080 $ & $   9.14704 $ & $  $\\
$ 55480.61469 $ & $   0.00693 $ & $   0.00080 $ & $   9.14641 $ & $  $\\
$ 55480.61504 $ & $   0.00564 $ & $   0.00081 $ & $   9.14555 $ & $  $\\
$ 55480.61535 $ & $   0.00691 $ & $   0.00080 $ & $   9.14606 $ & $  $\\
$ 55480.61569 $ & $   0.00645 $ & $   0.00080 $ & $   9.14618 $ & $  $\\
$ 55480.61603 $ & $   0.00701 $ & $   0.00080 $ & $   9.14637 $ & $  $\\
$ 55480.61637 $ & $   0.00792 $ & $   0.00080 $ & $   9.14655 $ & $  $\\
$ 55480.61671 $ & $   0.00708 $ & $   0.00080 $ & $   9.14600 $ & $  $\\
$ 55480.61703 $ & $   0.00900 $ & $   0.00080 $ & $   9.14869 $ & $  $\\
$ 55480.61733 $ & $   0.00891 $ & $   0.00080 $ & $   9.14802 $ & $  $\\
$ 55480.61765 $ & $   0.00779 $ & $   0.00080 $ & $   9.14693 $ & $  $\\
$ 55480.61794 $ & $   0.00893 $ & $   0.00080 $ & $   9.14784 $ & $  $\\
$ 55480.61829 $ & $   0.00670 $ & $   0.00080 $ & $   9.14592 $ & $  $\\
$ 55480.61863 $ & $   0.00903 $ & $   0.00080 $ & $   9.14852 $ & $  $\\
$ 55480.61895 $ & $   0.00704 $ & $   0.00080 $ & $   9.14641 $ & $  $\\
$ 55480.61927 $ & $   0.00705 $ & $   0.00080 $ & $   9.14624 $ & $  $\\
$ 55480.61959 $ & $   0.00736 $ & $   0.00080 $ & $   9.14625 $ & $  $\\
$ 55480.61993 $ & $   0.00633 $ & $   0.00080 $ & $   9.14542 $ & $  $\\
$ 55480.62027 $ & $   0.00536 $ & $   0.00080 $ & $   9.14436 $ & $  $\\
$ 55480.62062 $ & $   0.00788 $ & $   0.00080 $ & $   9.14724 $ & $  $\\
$ 55480.62095 $ & $   0.00872 $ & $   0.00080 $ & $   9.14801 $ & $  $\\
$ 55480.62128 $ & $   0.00577 $ & $   0.00080 $ & $   9.14435 $ & $  $\\
$ 55480.62161 $ & $   0.00715 $ & $   0.00080 $ & $   9.14588 $ & $  $\\
$ 55480.62196 $ & $   0.00734 $ & $   0.00080 $ & $   9.14655 $ & $  $\\
$ 55480.62228 $ & $   0.00557 $ & $   0.00080 $ & $   9.14518 $ & $  $\\
$ 55480.62262 $ & $   0.00550 $ & $   0.00080 $ & $   9.14527 $ & $  $\\
$ 55480.62297 $ & $   0.00678 $ & $   0.00080 $ & $   9.14570 $ & $  $\\
$ 55480.62327 $ & $   0.00463 $ & $   0.00080 $ & $   9.14342 $ & $  $\\
$ 55480.62359 $ & $   0.00516 $ & $   0.00080 $ & $   9.14442 $ & $  $\\
$ 55480.62392 $ & $   0.00775 $ & $   0.00080 $ & $   9.14689 $ & $  $\\
$ 55480.62425 $ & $   0.00659 $ & $   0.00080 $ & $   9.14537 $ & $  $\\
$ 55480.62460 $ & $   0.00735 $ & $   0.00080 $ & $   9.14642 $ & $  $\\
$ 55480.62493 $ & $   0.00377 $ & $   0.00080 $ & $   9.14306 $ & $  $\\
$ 55480.62525 $ & $   0.00841 $ & $   0.00080 $ & $   9.14805 $ & $  $\\
$ 55480.62559 $ & $   0.00704 $ & $   0.00080 $ & $   9.14660 $ & $  $\\
$ 55480.62592 $ & $   0.00800 $ & $   0.00080 $ & $   9.14731 $ & $  $\\
$ 55480.62624 $ & $   0.00843 $ & $   0.00080 $ & $   9.14775 $ & $  $\\
$ 55480.62659 $ & $   0.00750 $ & $   0.00080 $ & $   9.14684 $ & $  $\\
$ 55480.62694 $ & $   0.00695 $ & $   0.00080 $ & $   9.14530 $ & $  $\\
$ 55480.62727 $ & $   0.00784 $ & $   0.00080 $ & $   9.14687 $ & $  $\\
$ 55480.62762 $ & $   0.00409 $ & $   0.00080 $ & $   9.14268 $ & $  $\\
$ 55480.62794 $ & $   0.00543 $ & $   0.00080 $ & $   9.14483 $ & $  $\\
$ 55480.62828 $ & $   0.00881 $ & $   0.00080 $ & $   9.14790 $ & $  $\\
$ 55480.62863 $ & $   0.00777 $ & $   0.00080 $ & $   9.14667 $ & $  $\\
$ 55480.62896 $ & $   0.00900 $ & $   0.00080 $ & $   9.14780 $ & $  $\\
$ 55480.62929 $ & $   0.00785 $ & $   0.00080 $ & $   9.14658 $ & $  $\\
$ 55480.62962 $ & $   0.00632 $ & $   0.00080 $ & $   9.14536 $ & $  $\\
$ 55480.62996 $ & $   0.00866 $ & $   0.00080 $ & $   9.14724 $ & $  $\\
$ 55480.63028 $ & $   0.00592 $ & $   0.00080 $ & $   9.14452 $ & $  $\\
$ 55480.63060 $ & $   0.00872 $ & $   0.00080 $ & $   9.14752 $ & $  $\\
$ 55480.63095 $ & $   0.00945 $ & $   0.00080 $ & $   9.14849 $ & $  $\\
$ 55480.63126 $ & $   0.00757 $ & $   0.00080 $ & $   9.14718 $ & $  $\\
$ 55480.63162 $ & $   0.00720 $ & $   0.00080 $ & $   9.14656 $ & $  $\\
$ 55480.63194 $ & $   0.00659 $ & $   0.00080 $ & $   9.14576 $ & $  $\\
$ 55480.63228 $ & $   0.00555 $ & $   0.00080 $ & $   9.14476 $ & $  $\\
$ 55480.63261 $ & $   0.00648 $ & $   0.00080 $ & $   9.14515 $ & $  $\\
$ 55480.63295 $ & $   0.00476 $ & $   0.00080 $ & $   9.14353 $ & $  $\\
$ 55480.63328 $ & $   0.00641 $ & $   0.00080 $ & $   9.14577 $ & $  $\\
$ 55480.63360 $ & $   0.00710 $ & $   0.00080 $ & $   9.14640 $ & $  $\\
$ 55480.63395 $ & $   0.01101 $ & $   0.00080 $ & $   9.15005 $ & $  $\\
$ 55480.63427 $ & $   0.00737 $ & $   0.00080 $ & $   9.14622 $ & $  $\\
$ 55480.63460 $ & $   0.00845 $ & $   0.00080 $ & $   9.14767 $ & $  $\\
$ 55480.63494 $ & $   0.00725 $ & $   0.00080 $ & $   9.14642 $ & $  $\\
$ 55480.63527 $ & $   0.00733 $ & $   0.00080 $ & $   9.14593 $ & $  $\\
$ 55480.63560 $ & $   0.00498 $ & $   0.00080 $ & $   9.14429 $ & $  $\\
$ 55480.63593 $ & $   0.00751 $ & $   0.00080 $ & $   9.14629 $ & $  $\\
$ 55480.63626 $ & $   0.00917 $ & $   0.00080 $ & $   9.14812 $ & $  $\\
$ 55480.63661 $ & $   0.00595 $ & $   0.00080 $ & $   9.14540 $ & $  $\\
$ 55480.63692 $ & $   0.00860 $ & $   0.00080 $ & $   9.14781 $ & $  $\\
$ 55480.63724 $ & $   0.00447 $ & $   0.00080 $ & $   9.14399 $ & $  $\\
$ 55480.63755 $ & $   0.00585 $ & $   0.00080 $ & $   9.14569 $ & $  $\\
$ 55480.63788 $ & $   0.00701 $ & $   0.00081 $ & $   9.14683 $ & $  $\\
$ 55480.63821 $ & $   0.00768 $ & $   0.00080 $ & $   9.14659 $ & $  $\\
$ 55480.63853 $ & $   0.00722 $ & $   0.00080 $ & $   9.14636 $ & $  $\\
$ 55480.63886 $ & $   0.01029 $ & $   0.00080 $ & $   9.14964 $ & $  $\\
$ 55480.63920 $ & $   0.00912 $ & $   0.00080 $ & $   9.14865 $ & $  $\\
$ 55480.63953 $ & $   0.00846 $ & $   0.00080 $ & $   9.14783 $ & $  $\\
$ 55480.63983 $ & $   0.00596 $ & $   0.00080 $ & $   9.14515 $ & $  $\\
$ 55480.64018 $ & $   0.00712 $ & $   0.00080 $ & $   9.14624 $ & $  $\\
$ 55480.64050 $ & $   0.00880 $ & $   0.00080 $ & $   9.14763 $ & $  $\\
$ 55480.64085 $ & $   0.00457 $ & $   0.00080 $ & $   9.14372 $ & $  $\\
$ 55480.64117 $ & $   0.00649 $ & $   0.00080 $ & $   9.14504 $ & $  $\\
$ 55480.64152 $ & $   0.00794 $ & $   0.00080 $ & $   9.14661 $ & $  $\\
$ 55480.64184 $ & $   0.00916 $ & $   0.00080 $ & $   9.14846 $ & $  $\\
$ 55480.64219 $ & $   0.00765 $ & $   0.00080 $ & $   9.14697 $ & $  $\\
$ 55480.64249 $ & $   0.00808 $ & $   0.00080 $ & $   9.14714 $ & $  $\\
$ 55480.64284 $ & $   0.00524 $ & $   0.00080 $ & $   9.14432 $ & $  $\\
$ 55480.64317 $ & $   0.00824 $ & $   0.00080 $ & $   9.14706 $ & $  $\\
$ 55480.64351 $ & $   0.00817 $ & $   0.00080 $ & $   9.14745 $ & $  $\\
$ 55480.64383 $ & $   0.00884 $ & $   0.00080 $ & $   9.14814 $ & $  $\\
$ 55480.64417 $ & $   0.00918 $ & $   0.00080 $ & $   9.14904 $ & $  $\\
$ 55480.64449 $ & $   0.00609 $ & $   0.00081 $ & $   9.14570 $ & $  $\\
$ 55480.64485 $ & $   0.00621 $ & $   0.00080 $ & $   9.14554 $ & $  $\\
$ 55480.64514 $ & $   0.00379 $ & $   0.00080 $ & $   9.14268 $ & $  $\\
$ 55480.64549 $ & $   0.01012 $ & $   0.00080 $ & $   9.14933 $ & $  $\\
$ 55480.64581 $ & $   0.00783 $ & $   0.00080 $ & $   9.14715 $ & $  $\\
$ 55480.64615 $ & $   0.00591 $ & $   0.00080 $ & $   9.14545 $ & $  $\\
$ 55480.64650 $ & $   0.01014 $ & $   0.00080 $ & $   9.14831 $ & $  $\\
$ 55480.64681 $ & $   0.00599 $ & $   0.00080 $ & $   9.14550 $ & $  $\\
$ 55480.64714 $ & $   0.00646 $ & $   0.00080 $ & $   9.14622 $ & $  $\\
$ 55480.64748 $ & $   0.00893 $ & $   0.00080 $ & $   9.14817 $ & $  $\\
$ 55480.64781 $ & $   0.00788 $ & $   0.00081 $ & $   9.14791 $ & $  $\\
$ 55480.64814 $ & $   0.00955 $ & $   0.00081 $ & $   9.15008 $ & $  $\\
$ 55480.64847 $ & $   0.00879 $ & $   0.00080 $ & $   9.14820 $ & $  $\\
$ 55480.64881 $ & $   0.00801 $ & $   0.00080 $ & $   9.14730 $ & $  $\\
$ 55480.64914 $ & $   0.00666 $ & $   0.00080 $ & $   9.14541 $ & $  $\\
$ 55480.64948 $ & $   0.01067 $ & $   0.00080 $ & $   9.15027 $ & $  $\\
$ 55480.64982 $ & $   0.00820 $ & $   0.00080 $ & $   9.14753 $ & $  $\\
$ 55480.65015 $ & $   0.00514 $ & $   0.00080 $ & $   9.14397 $ & $  $\\
$ 55480.65049 $ & $   0.01295 $ & $   0.00080 $ & $   9.15185 $ & $  $\\
$ 55480.65081 $ & $   0.00797 $ & $   0.00080 $ & $   9.14673 $ & $  $\\
$ 55480.65115 $ & $   0.00882 $ & $   0.00080 $ & $   9.14749 $ & $  $\\
$ 55480.65144 $ & $   0.00764 $ & $   0.00080 $ & $   9.14608 $ & $  $\\
$ 55480.65178 $ & $   0.00497 $ & $   0.00080 $ & $   9.14304 $ & $  $\\
$ 55480.65211 $ & $   0.00782 $ & $   0.00080 $ & $   9.14656 $ & $  $\\
$ 55480.65245 $ & $   0.00837 $ & $   0.00080 $ & $   9.14725 $ & $  $\\
$ 55480.65278 $ & $   0.00746 $ & $   0.00080 $ & $   9.14627 $ & $  $\\
$ 55480.65310 $ & $   0.00629 $ & $   0.00080 $ & $   9.14550 $ & $  $\\
$ 55480.65345 $ & $   0.00701 $ & $   0.00080 $ & $   9.14580 $ & $  $\\
$ 55480.65379 $ & $   0.00884 $ & $   0.00080 $ & $   9.14823 $ & $  $\\
$ 55480.65411 $ & $   0.00983 $ & $   0.00080 $ & $   9.14924 $ & $  $\\
$ 55480.65443 $ & $   0.00905 $ & $   0.00080 $ & $   9.14829 $ & $  $\\
$ 55480.65478 $ & $   0.00813 $ & $   0.00080 $ & $   9.14722 $ & $  $\\
$ 55480.65511 $ & $   0.00583 $ & $   0.00080 $ & $   9.14407 $ & $  $\\
$ 55480.65545 $ & $   0.00673 $ & $   0.00080 $ & $   9.14558 $ & $  $\\
$ 55480.65578 $ & $   0.00473 $ & $   0.00080 $ & $   9.14332 $ & $  $\\
$ 55480.65610 $ & $   0.01022 $ & $   0.00080 $ & $   9.14882 $ & $  $\\
$ 55480.65645 $ & $   0.00941 $ & $   0.00080 $ & $   9.14805 $ & $  $\\
$ 55480.65677 $ & $   0.00623 $ & $   0.00080 $ & $   9.14534 $ & $  $\\
$ 55480.65708 $ & $   0.00459 $ & $   0.00080 $ & $   9.14363 $ & $  $\\
$ 55480.65741 $ & $   0.00810 $ & $   0.00080 $ & $   9.14732 $ & $  $\\
$ 55480.65776 $ & $   0.00973 $ & $   0.00080 $ & $   9.14902 $ & $  $\\
$ 55480.65808 $ & $   0.00841 $ & $   0.00080 $ & $   9.14747 $ & $  $\\
$ 55480.65843 $ & $   0.00934 $ & $   0.00080 $ & $   9.14861 $ & $  $\\
$ 55480.65875 $ & $   0.00777 $ & $   0.00080 $ & $   9.14664 $ & $  $\\
$ 55480.65909 $ & $   0.00900 $ & $   0.00080 $ & $   9.14763 $ & $  $\\
$ 55480.65942 $ & $   0.00549 $ & $   0.00080 $ & $   9.14522 $ & $  $\\
$ 55480.65976 $ & $   0.00794 $ & $   0.00080 $ & $   9.14679 $ & $  $\\
$ 55480.66011 $ & $   0.00874 $ & $   0.00080 $ & $   9.14787 $ & $  $\\
$ 55480.66045 $ & $   0.00597 $ & $   0.00080 $ & $   9.14496 $ & $  $\\
$ 55480.66078 $ & $   0.00933 $ & $   0.00080 $ & $   9.14792 $ & $  $\\
$ 55480.66110 $ & $   0.00685 $ & $   0.00080 $ & $   9.14506 $ & $  $\\
$ 55480.66142 $ & $   0.00820 $ & $   0.00080 $ & $   9.14686 $ & $  $\\
$ 55480.66176 $ & $   0.00865 $ & $   0.00080 $ & $   9.14812 $ & $  $\\
$ 55480.66208 $ & $   0.00786 $ & $   0.00080 $ & $   9.14711 $ & $  $\\
$ 55480.66242 $ & $   0.00682 $ & $   0.00080 $ & $   9.14573 $ & $  $\\
$ 55480.66274 $ & $   0.00697 $ & $   0.00080 $ & $   9.14518 $ & $  $\\
$ 55480.66309 $ & $   0.00759 $ & $   0.00080 $ & $   9.14633 $ & $  $\\
$ 55480.66340 $ & $   0.00718 $ & $   0.00080 $ & $   9.14601 $ & $  $\\
$ 55480.66375 $ & $   0.00667 $ & $   0.00080 $ & $   9.14531 $ & $  $\\
$ 55480.66409 $ & $   0.01001 $ & $   0.00080 $ & $   9.14878 $ & $  $\\
$ 55480.66442 $ & $   0.00645 $ & $   0.00080 $ & $   9.14490 $ & $  $\\
$ 55480.66475 $ & $   0.00486 $ & $   0.00080 $ & $   9.14286 $ & $  $\\
$ 55480.66509 $ & $   0.00756 $ & $   0.00080 $ & $   9.14598 $ & $  $\\
$ 55480.66542 $ & $   0.00885 $ & $   0.00080 $ & $   9.14746 $ & $  $\\
$ 55480.66574 $ & $   0.00704 $ & $   0.00080 $ & $   9.14576 $ & $  $\\
$ 55480.66605 $ & $   0.00787 $ & $   0.00080 $ & $   9.14678 $ & $  $\\
$ 55480.66640 $ & $   0.00786 $ & $   0.00080 $ & $   9.14726 $ & $  $\\
$ 55480.66672 $ & $   0.00792 $ & $   0.00080 $ & $   9.14671 $ & $  $\\
$ 55480.66706 $ & $   0.00814 $ & $   0.00080 $ & $   9.14667 $ & $  $\\
$ 55480.66736 $ & $   0.00764 $ & $   0.00081 $ & $   9.14745 $ & $  $\\
$ 55480.66770 $ & $   0.00694 $ & $   0.00081 $ & $   9.14655 $ & $  $\\
$ 55480.66803 $ & $   0.00842 $ & $   0.00080 $ & $   9.14736 $ & $  $\\
$ 55480.66836 $ & $   0.00781 $ & $   0.00080 $ & $   9.14656 $ & $  $\\
$ 55480.66870 $ & $   0.00888 $ & $   0.00080 $ & $   9.14848 $ & $  $\\
$ 55480.66903 $ & $   0.01054 $ & $   0.00081 $ & $   9.14998 $ & $  $\\
$ 55480.66933 $ & $   0.00728 $ & $   0.00080 $ & $   9.14642 $ & $  $\\
$ 55480.66966 $ & $   0.01070 $ & $   0.00080 $ & $   9.14972 $ & $  $\\
$ 55480.67001 $ & $   0.00845 $ & $   0.00080 $ & $   9.14688 $ & $  $\\
$ 55480.67035 $ & $   0.00568 $ & $   0.00080 $ & $   9.14451 $ & $  $\\
$ 55480.67068 $ & $   0.00884 $ & $   0.00080 $ & $   9.14688 $ & $  $\\
$ 55480.67100 $ & $   0.00872 $ & $   0.00080 $ & $   9.14689 $ & $  $\\
$ 55480.67134 $ & $   0.00650 $ & $   0.00080 $ & $   9.14567 $ & $  $\\
$ 55480.67168 $ & $   0.01078 $ & $   0.00080 $ & $   9.14948 $ & $  $\\
$ 55480.67197 $ & $   0.00775 $ & $   0.00080 $ & $   9.14606 $ & $  $\\
$ 55480.67231 $ & $   0.00872 $ & $   0.00080 $ & $   9.14669 $ & $  $\\
$ 55480.67265 $ & $   0.00870 $ & $   0.00080 $ & $   9.14683 $ & $  $\\
$ 55480.67297 $ & $   0.00953 $ & $   0.00080 $ & $   9.14766 $ & $  $\\
$ 55480.67331 $ & $   0.00805 $ & $   0.00080 $ & $   9.14622 $ & $  $\\
$ 55480.67365 $ & $   0.00643 $ & $   0.00080 $ & $   9.14429 $ & $  $\\
$ 55480.67397 $ & $   0.00823 $ & $   0.00080 $ & $   9.14651 $ & $  $\\
$ 55480.67430 $ & $   0.00835 $ & $   0.00080 $ & $   9.14613 $ & $  $\\
$ 55480.67470 $ & $   0.00830 $ & $   0.00080 $ & $   9.14712 $ & $  $\\
$ 55480.67510 $ & $   0.00618 $ & $   0.00080 $ & $   9.14483 $ & $  $\\
$ 55480.67549 $ & $   0.00917 $ & $   0.00080 $ & $   9.14701 $ & $  $\\
$ 55480.67587 $ & $   0.00931 $ & $   0.00080 $ & $   9.14740 $ & $  $\\
$ 55480.67624 $ & $   0.00835 $ & $   0.00080 $ & $   9.14669 $ & $  $\\
$ 55480.67656 $ & $   0.00984 $ & $   0.00080 $ & $   9.14844 $ & $  $\\
$ 55480.67691 $ & $   0.00784 $ & $   0.00080 $ & $   9.14599 $ & $  $\\
$ 55480.67722 $ & $   0.01087 $ & $   0.00080 $ & $   9.14879 $ & $  $\\
$ 55480.67756 $ & $   0.00859 $ & $   0.00080 $ & $   9.14700 $ & $  $\\
$ 55480.67789 $ & $   0.00987 $ & $   0.00080 $ & $   9.14718 $ & $  $\\
$ 55480.67824 $ & $   0.00660 $ & $   0.00080 $ & $   9.14483 $ & $  $\\
$ 55480.67856 $ & $   0.00812 $ & $   0.00080 $ & $   9.14620 $ & $  $\\
$ 55480.67889 $ & $   0.00661 $ & $   0.00080 $ & $   9.14434 $ & $  $\\
$ 55480.67924 $ & $   0.00652 $ & $   0.00080 $ & $   9.14469 $ & $  $\\
$ 55480.67956 $ & $   0.00703 $ & $   0.00080 $ & $   9.14482 $ & $  $\\
$ 55480.67988 $ & $   0.00935 $ & $   0.00080 $ & $   9.14681 $ & $  $\\
$ 55480.68023 $ & $   0.00749 $ & $   0.00080 $ & $   9.14440 $ & $  $\\
$ 55480.68055 $ & $   0.00610 $ & $   0.00080 $ & $   9.14390 $ & $  $\\
$ 55480.68090 $ & $   0.00686 $ & $   0.00080 $ & $   9.14461 $ & $  $\\
$ 55480.68121 $ & $   0.00939 $ & $   0.00080 $ & $   9.14735 $ & $  $\\
$ 55480.68156 $ & $   0.00904 $ & $   0.00080 $ & $   9.14640 $ & $  $\\
$ 55480.68190 $ & $   0.00703 $ & $   0.00080 $ & $   9.14513 $ & $  $\\
$ 55480.68222 $ & $   0.00965 $ & $   0.00080 $ & $   9.14736 $ & $  $\\
$ 55480.68256 $ & $   0.00683 $ & $   0.00080 $ & $   9.14507 $ & $  $\\
$ 55480.68288 $ & $   0.00623 $ & $   0.00080 $ & $   9.14408 $ & $  $\\
$ 55480.68323 $ & $   0.00959 $ & $   0.00080 $ & $   9.14748 $ & $  $\\
$ 55480.68355 $ & $   0.00580 $ & $   0.00080 $ & $   9.14312 $ & $  $\\
$ 55480.68390 $ & $   0.00809 $ & $   0.00080 $ & $   9.14620 $ & $  $\\
$ 55480.68424 $ & $   0.00782 $ & $   0.00080 $ & $   9.14556 $ & $  $\\
$ 55480.68455 $ & $   0.00774 $ & $   0.00080 $ & $   9.14568 $ & $  $\\
$ 55480.68487 $ & $   0.00744 $ & $   0.00080 $ & $   9.14518 $ & $  $\\
$ 55480.68521 $ & $   0.00811 $ & $   0.00080 $ & $   9.14574 $ & $  $\\
$ 55480.68551 $ & $   0.00626 $ & $   0.00080 $ & $   9.14453 $ & $  $\\
$ 55480.68583 $ & $   0.01078 $ & $   0.00080 $ & $   9.14916 $ & $  $\\
$ 55480.68618 $ & $   0.00810 $ & $   0.00080 $ & $   9.14614 $ & $  $\\
$ 55480.68652 $ & $   0.00855 $ & $   0.00080 $ & $   9.14639 $ & $  $\\
$ 55480.68683 $ & $   0.00578 $ & $   0.00080 $ & $   9.14426 $ & $  $\\
$ 55480.68716 $ & $   0.00806 $ & $   0.00080 $ & $   9.14652 $ & $  $\\
$ 55480.68750 $ & $   0.00664 $ & $   0.00080 $ & $   9.14438 $ & $  $\\
$ 55480.68783 $ & $   0.00705 $ & $   0.00080 $ & $   9.14462 $ & $  $\\
$ 55480.68815 $ & $   0.00726 $ & $   0.00080 $ & $   9.14456 $ & $  $\\
$ 55480.68849 $ & $   0.01025 $ & $   0.00080 $ & $   9.14818 $ & $  $\\
$ 55480.68882 $ & $   0.00764 $ & $   0.00080 $ & $   9.14547 $ & $  $\\
$ 55480.68916 $ & $   0.00848 $ & $   0.00080 $ & $   9.14621 $ & $  $\\
$ 55480.68950 $ & $   0.00687 $ & $   0.00080 $ & $   9.14468 $ & $  $\\
$ 55480.68981 $ & $   0.00863 $ & $   0.00080 $ & $   9.14624 $ & $  $\\
$ 55480.69015 $ & $   0.01047 $ & $   0.00080 $ & $   9.14826 $ & $  $\\
$ 55480.69048 $ & $   0.00570 $ & $   0.00080 $ & $   9.14390 $ & $  $\\
$ 55480.69087 $ & $   0.00736 $ & $   0.00080 $ & $   9.14550 $ & $  $\\
$ 55480.69125 $ & $   0.00674 $ & $   0.00080 $ & $   9.14472 $ & $  $\\
$ 55480.69163 $ & $   0.00558 $ & $   0.00080 $ & $   9.14324 $ & $  $\\
$ 55480.69200 $ & $   0.00727 $ & $   0.00080 $ & $   9.14463 $ & $  $\\
$ 55480.69238 $ & $   0.00533 $ & $   0.00080 $ & $   9.14330 $ & $  $\\
$ 55480.69272 $ & $   0.00928 $ & $   0.00080 $ & $   9.14732 $ & $  $\\
$ 55480.69304 $ & $   0.00623 $ & $   0.00080 $ & $   9.14380 $ & $  $\\
$ 55480.69338 $ & $   0.00744 $ & $   0.00080 $ & $   9.14498 $ & $  $\\
$ 55480.69372 $ & $   0.00705 $ & $   0.00080 $ & $   9.14522 $ & $  $\\
$ 55480.69406 $ & $   0.00760 $ & $   0.00080 $ & $   9.14566 $ & $  $\\
$ 55480.69438 $ & $   0.00964 $ & $   0.00080 $ & $   9.14763 $ & $  $\\
$ 55480.69473 $ & $   0.00597 $ & $   0.00080 $ & $   9.14423 $ & $  $\\
$ 55480.69511 $ & $   0.00506 $ & $   0.00080 $ & $   9.14292 $ & $  $\\
$ 55480.69550 $ & $   0.00933 $ & $   0.00080 $ & $   9.14723 $ & $  $\\
$ 55480.69588 $ & $   0.01035 $ & $   0.00080 $ & $   9.14828 $ & $  $\\
$ 55480.69625 $ & $   0.00533 $ & $   0.00080 $ & $   9.14322 $ & $  $\\
$ 55480.69660 $ & $   0.00959 $ & $   0.00080 $ & $   9.14736 $ & $  $\\
$ 55480.69694 $ & $   0.00747 $ & $   0.00080 $ & $   9.14544 $ & $  $\\
$ 55480.69724 $ & $   0.00689 $ & $   0.00080 $ & $   9.14515 $ & $  $\\
$ 55480.69758 $ & $   0.00580 $ & $   0.00081 $ & $   9.14474 $ & $  $\\
$ 55480.69791 $ & $   0.00896 $ & $   0.00081 $ & $   9.14828 $ & $  $\\
$ 55480.69825 $ & $   0.01064 $ & $   0.00081 $ & $   9.15006 $ & $  $\\
$ 55480.69859 $ & $   0.00838 $ & $   0.00081 $ & $   9.14788 $ & $  $\\
$ 55480.69890 $ & $   0.00829 $ & $   0.00081 $ & $   9.14667 $ & $  $\\
$ 55480.69925 $ & $   0.00656 $ & $   0.00080 $ & $   9.14454 $ & $  $\\
$ 55480.69957 $ & $   0.00578 $ & $   0.00080 $ & $   9.14360 $ & $  $\\
$ 55480.69989 $ & $   0.00806 $ & $   0.00080 $ & $   9.14607 $ & $  $\\
$ 55480.70022 $ & $   0.00772 $ & $   0.00080 $ & $   9.14567 $ & $  $\\
$ 55480.70054 $ & $   0.00962 $ & $   0.00080 $ & $   9.14714 $ & $  $\\
$ 55480.70089 $ & $   0.00816 $ & $   0.00080 $ & $   9.14668 $ & $  $\\
$ 55480.70122 $ & $   0.00794 $ & $   0.00080 $ & $   9.14607 $ & $  $\\
$ 55480.70154 $ & $   0.00603 $ & $   0.00080 $ & $   9.14395 $ & $  $\\
$ 55480.70187 $ & $   0.00861 $ & $   0.00081 $ & $   9.14714 $ & $  $\\
$ 55480.70220 $ & $   0.00865 $ & $   0.00081 $ & $   9.14695 $ & $  $\\
$ 55480.70253 $ & $   0.00812 $ & $   0.00081 $ & $   9.14645 $ & $  $\\
$ 55480.70286 $ & $   0.00754 $ & $   0.00080 $ & $   9.14574 $ & $  $\\
$ 55480.70319 $ & $   0.00634 $ & $   0.00081 $ & $   9.14528 $ & $  $\\
$ 55480.70352 $ & $   0.00586 $ & $   0.00081 $ & $   9.14456 $ & $  $\\
$ 55480.70385 $ & $   0.00964 $ & $   0.00081 $ & $   9.14756 $ & $  $\\
$ 55480.70419 $ & $   0.00537 $ & $   0.00080 $ & $   9.14334 $ & $  $\\
$ 55480.70452 $ & $   0.00822 $ & $   0.00080 $ & $   9.14588 $ & $  $\\
$ 55480.70485 $ & $   0.00783 $ & $   0.00080 $ & $   9.14572 $ & $  $\\
$ 55480.70518 $ & $   0.00622 $ & $   0.00080 $ & $   9.14406 $ & $  $\\
$ 55480.70552 $ & $   0.00636 $ & $   0.00080 $ & $   9.14471 $ & $  $\\
$ 55480.70584 $ & $   0.00838 $ & $   0.00081 $ & $   9.14637 $ & $  $\\
$ 55480.70619 $ & $   0.00736 $ & $   0.00080 $ & $   9.14572 $ & $  $\\
$ 55480.70651 $ & $   0.00888 $ & $   0.00080 $ & $   9.14688 $ & $  $\\
$ 55480.70685 $ & $   0.00700 $ & $   0.00080 $ & $   9.14541 $ & $  $\\
$ 55480.70717 $ & $   0.00573 $ & $   0.00080 $ & $   9.14401 $ & $  $\\
$ 55480.70752 $ & $   0.00786 $ & $   0.00080 $ & $   9.14567 $ & $  $\\
$ 55480.70784 $ & $   0.00912 $ & $   0.00080 $ & $   9.14690 $ & $  $\\
$ 55480.70817 $ & $   0.00937 $ & $   0.00081 $ & $   9.14786 $ & $  $\\
$ 55480.70852 $ & $   0.00423 $ & $   0.00080 $ & $   9.14307 $ & $  $\\
$ 55480.70884 $ & $   0.01057 $ & $   0.00081 $ & $   9.14837 $ & $  $\\
$ 55480.70916 $ & $   0.00725 $ & $   0.00080 $ & $   9.14553 $ & $  $\\
$ 55480.70950 $ & $   0.00988 $ & $   0.00080 $ & $   9.14821 $ & $  $\\
$ 55480.70982 $ & $   0.00724 $ & $   0.00081 $ & $   9.14581 $ & $  $\\
$ 55480.71016 $ & $   0.00758 $ & $   0.00081 $ & $   9.14536 $ & $  $\\
$ 55480.71047 $ & $   0.00666 $ & $   0.00081 $ & $   9.14483 $ & $  $\\
$ 55480.71081 $ & $   0.00534 $ & $   0.00080 $ & $   9.14333 $ & $  $\\
$ 55480.71115 $ & $   0.00642 $ & $   0.00080 $ & $   9.14492 $ & $  $\\
$ 55480.71148 $ & $   0.00879 $ & $   0.00081 $ & $   9.14680 $ & $  $\\
$ 55480.71181 $ & $   0.00611 $ & $   0.00080 $ & $   9.14443 $ & $  $\\
$ 55480.71215 $ & $   0.00686 $ & $   0.00080 $ & $   9.14531 $ & $  $\\
$ 55480.71247 $ & $   0.00836 $ & $   0.00081 $ & $   9.14643 $ & $  $\\
$ 55480.71280 $ & $   0.00821 $ & $   0.00081 $ & $   9.14649 $ & $  $\\
$ 55480.71312 $ & $   0.00758 $ & $   0.00080 $ & $   9.14590 $ & $  $\\
$ 55480.71346 $ & $   0.00758 $ & $   0.00080 $ & $   9.14558 $ & $  $\\
$ 55480.71379 $ & $   0.00924 $ & $   0.00080 $ & $   9.14702 $ & $  $\\
$ 55480.71413 $ & $   0.00628 $ & $   0.00080 $ & $   9.14466 $ & $  $\\
$ 55480.71446 $ & $   0.01030 $ & $   0.00081 $ & $   9.14887 $ & $  $\\
$ 55480.71479 $ & $   0.01057 $ & $   0.00081 $ & $   9.14911 $ & $  $\\
$ 55480.71511 $ & $   0.00523 $ & $   0.00081 $ & $   9.14366 $ & $  $\\
$ 55480.71544 $ & $   0.00419 $ & $   0.00081 $ & $   9.14217 $ & $  $\\
$ 55480.71578 $ & $   0.00857 $ & $   0.00081 $ & $   9.14657 $ & $  $\\
$ 55480.71611 $ & $   0.00640 $ & $   0.00081 $ & $   9.14470 $ & $  $\\
$ 55480.71644 $ & $   0.00596 $ & $   0.00081 $ & $   9.14449 $ & $  $\\
$ 55480.71678 $ & $   0.00675 $ & $   0.00081 $ & $   9.14500 $ & $  $\\
$ 55480.71709 $ & $   0.00558 $ & $   0.00080 $ & $   9.14335 $ & $  $\\
$ 55480.71744 $ & $   0.00245 $ & $   0.00080 $ & $   9.14133 $ & $  $\\
$ 55480.71776 $ & $   0.00785 $ & $   0.00081 $ & $   9.14558 $ & $  $\\
$ 55480.71811 $ & $   0.01022 $ & $   0.00081 $ & $   9.14859 $ & $  $\\
$ 55480.71845 $ & $   0.00548 $ & $   0.00081 $ & $   9.14315 $ & $  $\\
$ 55480.71878 $ & $   0.00884 $ & $   0.00081 $ & $   9.14800 $ & $  $\\
$ 55480.71909 $ & $   0.00594 $ & $   0.00081 $ & $   9.14424 $ & $  $\\
$ 55480.71943 $ & $   0.00784 $ & $   0.00081 $ & $   9.14618 $ & $  $\\
$ 55480.71976 $ & $   0.00695 $ & $   0.00081 $ & $   9.14588 $ & $  $\\
$ 55480.72009 $ & $   0.00945 $ & $   0.00081 $ & $   9.14815 $ & $  $\\
$ 55480.72044 $ & $   0.00789 $ & $   0.00080 $ & $   9.14591 $ & $  $\\
$ 55480.72076 $ & $   0.00879 $ & $   0.00081 $ & $   9.14726 $ & $  $\\
$ 55480.72111 $ & $   0.00780 $ & $   0.00081 $ & $   9.14699 $ & $  $\\
$ 55480.72143 $ & $   0.00617 $ & $   0.00081 $ & $   9.14481 $ & $  $\\
$ 55480.72177 $ & $   0.00547 $ & $   0.00081 $ & $   9.14402 $ & $  $\\
$ 55480.72209 $ & $   0.00557 $ & $   0.00081 $ & $   9.14418 $ & $  $\\
$ 55480.72243 $ & $   0.00638 $ & $   0.00081 $ & $   9.14476 $ & $  $\\
$ 55480.72274 $ & $   0.00629 $ & $   0.00081 $ & $   9.14497 $ & $  $\\
$ 55480.72309 $ & $   0.01047 $ & $   0.00081 $ & $   9.14844 $ & $  $\\
$ 55480.72341 $ & $   0.00511 $ & $   0.00081 $ & $   9.14441 $ & $  $\\
$ 55480.72375 $ & $   0.00889 $ & $   0.00081 $ & $   9.14670 $ & $  $\\
$ 55480.72405 $ & $   0.00680 $ & $   0.00081 $ & $   9.14497 $ & $  $\\
$ 55480.72438 $ & $   0.00646 $ & $   0.00081 $ & $   9.14531 $ & $  $\\
$ 55480.72473 $ & $   0.00667 $ & $   0.00081 $ & $   9.14521 $ & $  $\\
$ 55480.72504 $ & $   0.00637 $ & $   0.00081 $ & $   9.14495 $ & $  $\\
$ 55480.72540 $ & $   0.00617 $ & $   0.00081 $ & $   9.14433 $ & $  $\\
$ 55480.72571 $ & $   0.00525 $ & $   0.00081 $ & $   9.14419 $ & $  $\\
$ 55480.72604 $ & $   0.00347 $ & $   0.00081 $ & $   9.14172 $ & $  $\\
$ 55480.72638 $ & $   0.00590 $ & $   0.00081 $ & $   9.14463 $ & $  $\\
$ 55480.72679 $ & $   0.00632 $ & $   0.00081 $ & $   9.14520 $ & $  $\\
$ 55480.72720 $ & $   0.00995 $ & $   0.00081 $ & $   9.14797 $ & $  $\\
$ 55480.72759 $ & $   0.00966 $ & $   0.00081 $ & $   9.14911 $ & $  $\\
$ 55480.72796 $ & $   0.00611 $ & $   0.00081 $ & $   9.14481 $ & $  $\\
$ 55480.72831 $ & $   0.00726 $ & $   0.00081 $ & $   9.14578 $ & $  $\\
$ 55480.72864 $ & $   0.00821 $ & $   0.00081 $ & $   9.14730 $ & $  $\\
$ 55480.72895 $ & $   0.00689 $ & $   0.00081 $ & $   9.14577 $ & $  $\\
$ 55480.72934 $ & $   0.00445 $ & $   0.00081 $ & $   9.14344 $ & $  $\\
$ 55480.72972 $ & $   0.00386 $ & $   0.00081 $ & $   9.14234 $ & $  $\\
$ 55480.73008 $ & $   0.00443 $ & $   0.00081 $ & $   9.14424 $ & $  $\\
$ 55480.73045 $ & $   0.01035 $ & $   0.00081 $ & $   9.14917 $ & $  $\\
$ 55480.73082 $ & $   0.00698 $ & $   0.00081 $ & $   9.14503 $ & $  $\\
$ 55480.73121 $ & $   0.00726 $ & $   0.00081 $ & $   9.14600 $ & $  $\\
$ 55480.73158 $ & $   0.00402 $ & $   0.00081 $ & $   9.14255 $ & $  $\\
$ 55480.73196 $ & $   0.00906 $ & $   0.00081 $ & $   9.14796 $ & $  $\\
$ 55480.73233 $ & $   0.00676 $ & $   0.00081 $ & $   9.14561 $ & $  $\\
$ 55480.73273 $ & $   0.00690 $ & $   0.00081 $ & $   9.14503 $ & $  $\\
$ 55480.73311 $ & $   0.00327 $ & $   0.00081 $ & $   9.14144 $ & $  $\\
$ 55480.73349 $ & $   0.00167 $ & $   0.00081 $ & $   9.14092 $ & $  $\\
$ 55480.73387 $ & $   0.00543 $ & $   0.00081 $ & $   9.14379 $ & $  $\\
$ 55480.73425 $ & $   0.00827 $ & $   0.00081 $ & $   9.14728 $ & $  $\\
$ 55480.73462 $ & $   0.00342 $ & $   0.00081 $ & $   9.14226 $ & $  $\\
$ 55480.73502 $ & $   0.00042 $ & $   0.00080 $ & $   9.13906 $ & $  $\\
$ 55480.73539 $ & $   0.00106 $ & $   0.00081 $ & $   9.13981 $ & $  $\\
$ 55480.73578 $ & $   0.00532 $ & $   0.00081 $ & $   9.14400 $ & $  $\\
$ 55480.73615 $ & $   0.00254 $ & $   0.00081 $ & $   9.14159 $ & $  $\\
$ 55480.73655 $ & $   0.00223 $ & $   0.00081 $ & $   9.14090 $ & $  $\\
$ 55480.73693 $ & $   0.00325 $ & $   0.00081 $ & $   9.14296 $ & $  $\\
$ 55480.73731 $ & $   0.00417 $ & $   0.00081 $ & $   9.14343 $ & $  $\\
$ 55480.73767 $ & $   0.00085 $ & $   0.00081 $ & $   9.13991 $ & $  $\\
$ 55480.73804 $ & $  -0.00081 $ & $   0.00081 $ & $   9.13818 $ & $  $\\
$ 55480.73842 $ & $  -0.00076 $ & $   0.00081 $ & $   9.13745 $ & $  $\\
$ 55480.73881 $ & $  -0.00101 $ & $   0.00081 $ & $   9.13820 $ & $  $\\
$ 55480.73920 $ & $   0.00059 $ & $   0.00081 $ & $   9.13962 $ & $  $\\
$ 55480.73957 $ & $   0.00255 $ & $   0.00081 $ & $   9.14123 $ & $  $\\
$ 55480.73995 $ & $  -0.00065 $ & $   0.00081 $ & $   9.13798 $ & $  $\\
$ 55480.74033 $ & $   0.00396 $ & $   0.00081 $ & $   9.14189 $ & $  $\\
$ 55480.74070 $ & $  -0.00221 $ & $   0.00081 $ & $   9.13673 $ & $  $\\
$ 55480.74107 $ & $   0.00202 $ & $   0.00081 $ & $   9.14077 $ & $  $\\
$ 55480.74141 $ & $   0.00054 $ & $   0.00081 $ & $   9.13952 $ & $  $\\
$ 55480.74208 $ & $   0.00485 $ & $   0.00081 $ & $   9.14422 $ & $  $\\
$ 55480.74241 $ & $   0.00012 $ & $   0.00081 $ & $   9.14055 $ & $  $\\
$ 55480.74276 $ & $  -0.00320 $ & $   0.00081 $ & $   9.13702 $ & $  $\\
$ 55480.74307 $ & $   0.00392 $ & $   0.00081 $ & $   9.14389 $ & $  $\\
$ 55480.74341 $ & $  -0.00126 $ & $   0.00081 $ & $   9.13782 $ & $  $\\
$ 55480.74376 $ & $  -0.00312 $ & $   0.00081 $ & $   9.13583 $ & $  $\\
$ 55480.74414 $ & $  -0.00319 $ & $   0.00081 $ & $   9.13530 $ & $  $\\
$ 55480.74452 $ & $  -0.00338 $ & $   0.00081 $ & $   9.13531 $ & $  $\\
$ 55480.74481 $ & $   0.00316 $ & $   0.00081 $ & $   9.14201 $ & $  $\\
$ 55480.74516 $ & $  -0.00153 $ & $   0.00081 $ & $   9.13742 $ & $  $\\
$ 55480.74548 $ & $  -0.00141 $ & $   0.00081 $ & $   9.13711 $ & $  $\\
$ 55480.74580 $ & $   0.00097 $ & $   0.00081 $ & $   9.13995 $ & $  $\\
$ 55480.74613 $ & $   0.00212 $ & $   0.00081 $ & $   9.14173 $ & $  $\\
$ 55480.74678 $ & $   0.00203 $ & $   0.00081 $ & $   9.14166 $ & $  $\\
$ 55480.74710 $ & $  -0.00122 $ & $   0.00081 $ & $   9.13855 $ & $  $\\
$ 55480.74742 $ & $  -0.00062 $ & $   0.00082 $ & $   9.14022 $ & $  $\\
$ 55480.74777 $ & $   0.00186 $ & $   0.00081 $ & $   9.14104 $ & $  $\\
$ 55480.74812 $ & $   0.00050 $ & $   0.00081 $ & $   9.13981 $ & $  $\\
$ 55480.74845 $ & $   0.00365 $ & $   0.00082 $ & $   9.14420 $ & $  $\\
$ 55480.74878 $ & $   0.00164 $ & $   0.00081 $ & $   9.13967 $ & $  $\\
$ 55480.74911 $ & $   0.00033 $ & $   0.00081 $ & $   9.13889 $ & $  $\\
$ 55480.74943 $ & $   0.00333 $ & $   0.00081 $ & $   9.14218 $ & $  $\\
$ 55480.74975 $ & $   0.00230 $ & $   0.00081 $ & $   9.14090 $ & $  $\\
$ 55480.75009 $ & $   0.00103 $ & $   0.00081 $ & $   9.13916 $ & $  $\\
$ 55480.75042 $ & $   0.00265 $ & $   0.00081 $ & $   9.14153 $ & $  $\\
$ 55480.75111 $ & $  -0.00186 $ & $   0.00081 $ & $   9.13685 $ & $  $\\
$ 55480.75142 $ & $  -0.00072 $ & $   0.00081 $ & $   9.13799 $ & $  $\\
$ 55480.75175 $ & $   0.00305 $ & $   0.00081 $ & $   9.14145 $ & $  $\\
$ 55480.75208 $ & $   0.00216 $ & $   0.00081 $ & $   9.14087 $ & $  $\\
$ 55480.75241 $ & $  -0.00156 $ & $   0.00081 $ & $   9.13737 $ & $  $\\
$ 55480.75275 $ & $   0.00152 $ & $   0.00081 $ & $   9.14067 $ & $  $\\
$ 55480.75310 $ & $  -0.00147 $ & $   0.00081 $ & $   9.13747 $ & $  $\\
$ 55480.75342 $ & $  -0.00103 $ & $   0.00082 $ & $   9.13866 $ & $  $\\
$ 55480.75409 $ & $  -0.00414 $ & $   0.00081 $ & $   9.13510 $ & $  $\\
$ 55480.75442 $ & $  -0.00349 $ & $   0.00081 $ & $   9.13514 $ & $  $\\
$ 55480.75475 $ & $  -0.00505 $ & $   0.00081 $ & $   9.13372 $ & $  $\\
$ 55480.75509 $ & $   0.00287 $ & $   0.00081 $ & $   9.14191 $ & $  $\\
$ 55480.75541 $ & $   0.00135 $ & $   0.00081 $ & $   9.14081 $ & $  $\\
$ 55480.75609 $ & $  -0.00166 $ & $   0.00081 $ & $   9.13689 $ & $  $\\
$ 55480.75643 $ & $  -0.00057 $ & $   0.00081 $ & $   9.13804 $ & $  $\\
$ 55480.75674 $ & $  -0.00046 $ & $   0.00081 $ & $   9.13822 $ & $  $\\
$ 55480.75709 $ & $   0.00286 $ & $   0.00081 $ & $   9.14120 $ & $  $\\
$ 55480.75741 $ & $  -0.00127 $ & $   0.00081 $ & $   9.13756 $ & $  $\\
$ 55480.75774 $ & $   0.00369 $ & $   0.00081 $ & $   9.14244 $ & $  $\\
$ 55480.75808 $ & $  -0.00245 $ & $   0.00081 $ & $   9.13602 $ & $  $\\
$ 55480.75844 $ & $   0.00420 $ & $   0.00081 $ & $   9.14231 $ & $  $\\
$ 55480.75878 $ & $   0.00007 $ & $   0.00081 $ & $   9.13878 $ & $  $\\
$ 55480.75910 $ & $  -0.00144 $ & $   0.00081 $ & $   9.13640 $ & $  $\\
$ 55480.75943 $ & $  -0.00297 $ & $   0.00081 $ & $   9.13524 $ & $  $\\
$ 55480.75977 $ & $  -0.00234 $ & $   0.00081 $ & $   9.13626 $ & $  $\\
$ 55480.76009 $ & $   0.00452 $ & $   0.00081 $ & $   9.14333 $ & $  $\\
$ 55480.76043 $ & $   0.00266 $ & $   0.00081 $ & $   9.14192 $ & $  $\\
$ 55480.76076 $ & $   0.00040 $ & $   0.00081 $ & $   9.13900 $ & $  $\\
$ 55480.76110 $ & $   0.00145 $ & $   0.00081 $ & $   9.14006 $ & $  $\\
$ 55480.76187 $ & $   0.00202 $ & $   0.00081 $ & $   9.14067 $ & $  $\\
$ 55480.76225 $ & $   0.00222 $ & $   0.00081 $ & $   9.14072 $ & $  $\\
$ 55480.76263 $ & $   0.00014 $ & $   0.00081 $ & $   9.13860 $ & $  $\\
$ 55480.76301 $ & $   0.00197 $ & $   0.00081 $ & $   9.14132 $ & $  $\\
$ 55480.76334 $ & $  -0.00397 $ & $   0.00081 $ & $   9.13451 $ & $  $\\
$ 55480.76370 $ & $  -0.00071 $ & $   0.00081 $ & $   9.13855 $ & $  $\\
$ 55480.76408 $ & $  -0.00347 $ & $   0.00081 $ & $   9.13472 $ & $  $\\
$ 55480.76447 $ & $   0.00393 $ & $   0.00081 $ & $   9.14222 $ & $  $\\
$ 55480.76485 $ & $   0.00011 $ & $   0.00081 $ & $   9.13867 $ & $  $\\
$ 55480.76524 $ & $   0.00000 $ & $   0.00081 $ & $   9.13857 $ & $  $\\
$ 55480.76561 $ & $  -0.00157 $ & $   0.00081 $ & $   9.13635 $ & $  $\\
$ 55480.76599 $ & $   0.00011 $ & $   0.00081 $ & $   9.13890 $ & $  $\\
$ 55480.76636 $ & $  -0.00167 $ & $   0.00081 $ & $   9.13725 $ & $  $\\
$ 55480.76669 $ & $   0.00211 $ & $   0.00081 $ & $   9.14047 $ & $  $\\
$ 55480.76703 $ & $   0.00203 $ & $   0.00081 $ & $   9.14055 $ & $  $\\
$ 55480.76738 $ & $   0.00125 $ & $   0.00081 $ & $   9.14027 $ & $  $\\
$ 55480.76771 $ & $  -0.00303 $ & $   0.00081 $ & $   9.13443 $ & $  $\\
$ 55480.76804 $ & $  -0.00223 $ & $   0.00081 $ & $   9.13703 $ & $  $\\
$ 55480.76837 $ & $  -0.00098 $ & $   0.00081 $ & $   9.13812 $ & $  $\\
$ 55480.76904 $ & $   0.00189 $ & $   0.00081 $ & $   9.14114 $ & $  $\\
$ 55480.76938 $ & $   0.00345 $ & $   0.00082 $ & $   9.14259 $ & $  $\\
$ 55480.76969 $ & $  -0.00434 $ & $   0.00081 $ & $   9.13455 $ & $  $\\
$ 55480.77004 $ & $  -0.00004 $ & $   0.00082 $ & $   9.13976 $ & $  $\\
$ 55480.77037 $ & $  -0.00370 $ & $   0.00081 $ & $   9.13572 $ & $  $\\
$ 55480.77070 $ & $  -0.00031 $ & $   0.00082 $ & $   9.13863 $ & $  $\\
$ 55480.77102 $ & $  -0.00070 $ & $   0.00081 $ & $   9.13725 $ & $  $\\
$ 55480.77136 $ & $  -0.00277 $ & $   0.00081 $ & $   9.13586 $ & $  $\\
$ 55480.77169 $ & $  -0.00175 $ & $   0.00082 $ & $   9.13725 $ & $  $\\
$ 55480.77203 $ & $  -0.00175 $ & $   0.00081 $ & $   9.13758 $ & $  $\\
$ 55480.77235 $ & $   0.00242 $ & $   0.00082 $ & $   9.14163 $ & $  $\\


==> data/HTR340-006_phfu_tab.tex <==
$ 55338.79359 $ & $   0.00011 $ & $   0.00080 $ & $  10.12720 $ & $ i$\\
$ 55338.79427 $ & $  -0.00108 $ & $   0.00080 $ & $  10.12640 $ & $ i$\\
$ 55338.79494 $ & $   0.00263 $ & $   0.00080 $ & $  10.12910 $ & $ i$\\
$ 55338.79563 $ & $  -0.00041 $ & $   0.00080 $ & $  10.12660 $ & $ i$\\
$ 55338.79633 $ & $   0.00158 $ & $   0.00080 $ & $  10.12850 $ & $ i$\\
$ 55338.79701 $ & $   0.00036 $ & $   0.00079 $ & $  10.12720 $ & $ i$\\
$ 55338.79769 $ & $  -0.00243 $ & $   0.00079 $ & $  10.12440 $ & $ i$\\
$ 55338.79837 $ & $  -0.00305 $ & $   0.00079 $ & $  10.12340 $ & $ i$\\
$ 55338.79905 $ & $   0.00184 $ & $   0.00079 $ & $  10.12940 $ & $ i$\\
$ 55338.79969 $ & $   0.00187 $ & $   0.00079 $ & $  10.12900 $ & $ i$\\
$ 55338.80036 $ & $  -0.00102 $ & $   0.00078 $ & $  10.12570 $ & $ i$\\
$ 55338.80103 $ & $  -0.00230 $ & $   0.00078 $ & $  10.12470 $ & $ i$\\
$ 55338.80170 $ & $  -0.00152 $ & $   0.00078 $ & $  10.12600 $ & $ i$\\
$ 55338.80239 $ & $  -0.00223 $ & $   0.00078 $ & $  10.12530 $ & $ i$\\
$ 55338.80307 $ & $   0.00141 $ & $   0.00078 $ & $  10.12940 $ & $ i$\\
$ 55338.80377 $ & $   0.00063 $ & $   0.00078 $ & $  10.12790 $ & $ i$\\
$ 55338.80445 $ & $  -0.00023 $ & $   0.00078 $ & $  10.12690 $ & $ i$\\
$ 55338.80514 $ & $  -0.00008 $ & $   0.00078 $ & $  10.12670 $ & $ i$\\
$ 55338.80581 $ & $   0.00189 $ & $   0.00078 $ & $  10.12890 $ & $ i$\\
$ 55338.80649 $ & $   0.00170 $ & $   0.00078 $ & $  10.12920 $ & $ i$\\
$ 55338.80719 $ & $  -0.00021 $ & $   0.00078 $ & $  10.12710 $ & $ i$\\
$ 55338.80787 $ & $   0.00250 $ & $   0.00078 $ & $  10.13010 $ & $ i$\\
$ 55338.80854 $ & $   0.00227 $ & $   0.00078 $ & $  10.13020 $ & $ i$\\
$ 55338.80991 $ & $  -0.00354 $ & $   0.00077 $ & $  10.12390 $ & $ i$\\
$ 55338.81059 $ & $  -0.00141 $ & $   0.00077 $ & $  10.12570 $ & $ i$\\
$ 55338.81126 $ & $  -0.00003 $ & $   0.00077 $ & $  10.12720 $ & $ i$\\
$ 55338.81194 $ & $   0.00072 $ & $   0.00077 $ & $  10.12800 $ & $ i$\\
$ 55338.81263 $ & $   0.00221 $ & $   0.00077 $ & $  10.12890 $ & $ i$\\
$ 55338.81327 $ & $  -0.00171 $ & $   0.00077 $ & $  10.12530 $ & $ i$\\
$ 55338.81397 $ & $  -0.00103 $ & $   0.00077 $ & $  10.12650 $ & $ i$\\
$ 55338.81468 $ & $   0.00075 $ & $   0.00077 $ & $  10.12800 $ & $ i$\\
$ 55338.81537 $ & $  -0.00170 $ & $   0.00077 $ & $  10.12540 $ & $ i$\\
$ 55338.81605 $ & $   0.00326 $ & $   0.00077 $ & $  10.13030 $ & $ i$\\
$ 55338.81672 $ & $   0.00375 $ & $   0.00077 $ & $  10.13070 $ & $ i$\\
$ 55338.81740 $ & $  -0.00066 $ & $   0.00076 $ & $  10.12590 $ & $ i$\\
$ 55338.81808 $ & $  -0.00298 $ & $   0.00076 $ & $  10.12380 $ & $ i$\\
$ 55338.81876 $ & $  -0.00308 $ & $   0.00076 $ & $  10.12340 $ & $ i$\\
$ 55338.81944 $ & $  -0.00037 $ & $   0.00076 $ & $  10.12640 $ & $ i$\\
$ 55338.82013 $ & $   0.00194 $ & $   0.00076 $ & $  10.12860 $ & $ i$\\
$ 55338.82079 $ & $   0.00293 $ & $   0.00076 $ & $  10.13020 $ & $ i$\\
$ 55338.82146 $ & $  -0.00025 $ & $   0.00076 $ & $  10.12700 $ & $ i$\\
$ 55338.82214 $ & $  -0.00207 $ & $   0.00076 $ & $  10.12500 $ & $ i$\\
$ 55338.82281 $ & $   0.00100 $ & $   0.00076 $ & $  10.12790 $ & $ i$\\
$ 55338.82348 $ & $   0.00040 $ & $   0.00076 $ & $  10.12790 $ & $ i$\\
$ 55338.82415 $ & $  -0.00025 $ & $   0.00076 $ & $  10.12660 $ & $ i$\\
$ 55338.82485 $ & $  -0.00341 $ & $   0.00076 $ & $  10.12300 $ & $ i$\\
$ 55338.82553 $ & $  -0.00246 $ & $   0.00076 $ & $  10.12470 $ & $ i$\\
$ 55338.82624 $ & $  -0.00167 $ & $   0.00076 $ & $  10.12570 $ & $ i$\\
$ 55338.82692 $ & $   0.00101 $ & $   0.00076 $ & $  10.12790 $ & $ i$\\
$ 55338.82760 $ & $   0.00203 $ & $   0.00076 $ & $  10.12830 $ & $ i$\\
$ 55338.82830 $ & $   0.00080 $ & $   0.00076 $ & $  10.12790 $ & $ i$\\
$ 55338.82898 $ & $  -0.00142 $ & $   0.00075 $ & $  10.12540 $ & $ i$\\
$ 55338.82965 $ & $  -0.00191 $ & $   0.00076 $ & $  10.12540 $ & $ i$\\
$ 55338.83034 $ & $   0.00226 $ & $   0.00076 $ & $  10.12930 $ & $ i$\\
$ 55338.83100 $ & $   0.00291 $ & $   0.00076 $ & $  10.13040 $ & $ i$\\
$ 55338.83169 $ & $  -0.00217 $ & $   0.00075 $ & $  10.12490 $ & $ i$\\
$ 55338.83238 $ & $   0.00346 $ & $   0.00075 $ & $  10.12990 $ & $ i$\\
$ 55338.83306 $ & $   0.00388 $ & $   0.00075 $ & $  10.13080 $ & $ i$\\
$ 55338.83373 $ & $   0.00079 $ & $   0.00075 $ & $  10.12790 $ & $ i$\\
$ 55338.83440 $ & $   0.00082 $ & $   0.00075 $ & $  10.12710 $ & $ i$\\
$ 55338.83507 $ & $   0.00287 $ & $   0.00076 $ & $  10.13000 $ & $ i$\\
$ 55338.83582 $ & $   0.00407 $ & $   0.00076 $ & $  10.13140 $ & $ i$\\
$ 55338.83652 $ & $   0.00578 $ & $   0.00076 $ & $  10.13300 $ & $ i$\\
$ 55338.83719 $ & $   0.00462 $ & $   0.00076 $ & $  10.13200 $ & $ i$\\
$ 55338.83786 $ & $   0.00406 $ & $   0.00075 $ & $  10.13080 $ & $ i$\\
$ 55338.83853 $ & $   0.00344 $ & $   0.00075 $ & $  10.13030 $ & $ i$\\
$ 55338.83921 $ & $   0.00590 $ & $   0.00075 $ & $  10.13190 $ & $ i$\\
$ 55338.83991 $ & $   0.00745 $ & $   0.00075 $ & $  10.13420 $ & $ i$\\
$ 55338.84059 $ & $   0.00751 $ & $   0.00075 $ & $  10.13410 $ & $ i$\\
$ 55338.84126 $ & $   0.00597 $ & $   0.00075 $ & $  10.13270 $ & $ i$\\
$ 55338.84195 $ & $   0.00828 $ & $   0.00075 $ & $  10.13420 $ & $ i$\\
$ 55338.84264 $ & $   0.00762 $ & $   0.00075 $ & $  10.13390 $ & $ i$\\
$ 55338.84331 $ & $   0.00937 $ & $   0.00075 $ & $  10.13560 $ & $ i$\\
$ 55338.84399 $ & $   0.00911 $ & $   0.00075 $ & $  10.13490 $ & $ i$\\
$ 55338.84467 $ & $   0.00797 $ & $   0.00075 $ & $  10.13370 $ & $ i$\\
$ 55338.84535 $ & $   0.00699 $ & $   0.00075 $ & $  10.13260 $ & $ i$\\
$ 55338.84603 $ & $   0.00850 $ & $   0.00075 $ & $  10.13420 $ & $ i$\\
$ 55338.84671 $ & $   0.00783 $ & $   0.00075 $ & $  10.13370 $ & $ i$\\
$ 55338.84739 $ & $   0.00791 $ & $   0.00075 $ & $  10.13350 $ & $ i$\\
$ 55338.84807 $ & $   0.00853 $ & $   0.00074 $ & $  10.13390 $ & $ i$\\
$ 55338.84876 $ & $   0.00854 $ & $   0.00074 $ & $  10.13410 $ & $ i$\\
$ 55338.84943 $ & $   0.00579 $ & $   0.00074 $ & $  10.13140 $ & $ i$\\
$ 55338.85013 $ & $   0.00624 $ & $   0.00074 $ & $  10.13200 $ & $ i$\\
$ 55338.85080 $ & $   0.00766 $ & $   0.00075 $ & $  10.13440 $ & $ i$\\
$ 55338.85151 $ & $   0.00891 $ & $   0.00074 $ & $  10.13530 $ & $ i$\\
$ 55338.85215 $ & $   0.00667 $ & $   0.00074 $ & $  10.13210 $ & $ i$\\
$ 55338.85284 $ & $   0.00706 $ & $   0.00074 $ & $  10.13210 $ & $ i$\\
$ 55338.85352 $ & $   0.00681 $ & $   0.00074 $ & $  10.13260 $ & $ i$\\
$ 55338.85419 $ & $   0.00732 $ & $   0.00074 $ & $  10.13330 $ & $ i$\\
$ 55338.85486 $ & $   0.00633 $ & $   0.00074 $ & $  10.13200 $ & $ i$\\
$ 55338.85555 $ & $   0.00703 $ & $   0.00074 $ & $  10.13260 $ & $ i$\\
$ 55338.85628 $ & $   0.00687 $ & $   0.00074 $ & $  10.13230 $ & $ i$\\
$ 55338.85697 $ & $   0.00686 $ & $   0.00074 $ & $  10.13270 $ & $ i$\\
$ 55338.85764 $ & $   0.00795 $ & $   0.00074 $ & $  10.13320 $ & $ i$\\
$ 55338.85831 $ & $   0.00634 $ & $   0.00074 $ & $  10.13210 $ & $ i$\\
$ 55338.85900 $ & $   0.00622 $ & $   0.00074 $ & $  10.13210 $ & $ i$\\
$ 55338.85967 $ & $   0.00537 $ & $   0.00074 $ & $  10.13180 $ & $ i$\\
$ 55338.86035 $ & $   0.00807 $ & $   0.00074 $ & $  10.13420 $ & $ i$\\
$ 55338.86103 $ & $   0.00644 $ & $   0.00074 $ & $  10.13230 $ & $ i$\\
$ 55338.86172 $ & $   0.00512 $ & $   0.00074 $ & $  10.13070 $ & $ i$\\
$ 55338.86239 $ & $   0.00673 $ & $   0.00074 $ & $  10.13240 $ & $ i$\\
$ 55338.86307 $ & $   0.00714 $ & $   0.00074 $ & $  10.13250 $ & $ i$\\
$ 55338.86374 $ & $   0.00578 $ & $   0.00074 $ & $  10.13100 $ & $ i$\\
$ 55338.86442 $ & $   0.00520 $ & $   0.00074 $ & $  10.13080 $ & $ i$\\
$ 55338.86512 $ & $   0.00684 $ & $   0.00074 $ & $  10.13290 $ & $ i$\\
$ 55338.86581 $ & $   0.00549 $ & $   0.00074 $ & $  10.13160 $ & $ i$\\
$ 55338.86650 $ & $   0.00505 $ & $   0.00074 $ & $  10.13070 $ & $ i$\\
$ 55338.86716 $ & $   0.00689 $ & $   0.00073 $ & $  10.13270 $ & $ i$\\
$ 55338.86784 $ & $   0.00577 $ & $   0.00073 $ & $  10.13150 $ & $ i$\\
$ 55338.86851 $ & $   0.00875 $ & $   0.00074 $ & $  10.13400 $ & $ i$\\
$ 55338.86918 $ & $   0.00710 $ & $   0.00074 $ & $  10.13290 $ & $ i$\\
$ 55338.86985 $ & $   0.00782 $ & $   0.00074 $ & $  10.13350 $ & $ i$\\
$ 55338.87054 $ & $   0.00742 $ & $   0.00074 $ & $  10.13320 $ & $ i$\\
$ 55338.87121 $ & $   0.00847 $ & $   0.00074 $ & $  10.13460 $ & $ i$\\
$ 55338.87188 $ & $   0.00862 $ & $   0.00073 $ & $  10.13390 $ & $ i$\\
$ 55338.87257 $ & $   0.00684 $ & $   0.00073 $ & $  10.13240 $ & $ i$\\
$ 55338.87326 $ & $   0.00664 $ & $   0.00074 $ & $  10.13240 $ & $ i$\\
$ 55338.87392 $ & $   0.00585 $ & $   0.00074 $ & $  10.13250 $ & $ i$\\
$ 55338.87459 $ & $   0.00771 $ & $   0.00074 $ & $  10.13440 $ & $ i$\\
$ 55338.87527 $ & $   0.00675 $ & $   0.00074 $ & $  10.13330 $ & $ i$\\
$ 55338.87594 $ & $   0.00632 $ & $   0.00074 $ & $  10.13300 $ & $ i$\\
$ 55338.87668 $ & $   0.00762 $ & $   0.00074 $ & $  10.13430 $ & $ i$\\
$ 55338.87736 $ & $   0.00689 $ & $   0.00074 $ & $  10.13330 $ & $ i$\\
$ 55338.87804 $ & $   0.00604 $ & $   0.00074 $ & $  10.13260 $ & $ i$\\
$ 55338.87871 $ & $   0.00787 $ & $   0.00074 $ & $  10.13450 $ & $ i$\\
$ 55338.87937 $ & $   0.00869 $ & $   0.00074 $ & $  10.13500 $ & $ i$\\
$ 55338.88004 $ & $   0.00806 $ & $   0.00074 $ & $  10.13520 $ & $ i$\\
$ 55338.88073 $ & $   0.00774 $ & $   0.00074 $ & $  10.13390 $ & $ i$\\
$ 55338.88143 $ & $   0.00727 $ & $   0.00074 $ & $  10.13440 $ & $ i$\\
$ 55338.88210 $ & $   0.00578 $ & $   0.00074 $ & $  10.13270 $ & $ i$\\
$ 55338.88278 $ & $   0.00752 $ & $   0.00074 $ & $  10.13430 $ & $ i$\\
$ 55338.88344 $ & $   0.00391 $ & $   0.00074 $ & $  10.13100 $ & $ i$\\
$ 55338.88410 $ & $   0.00847 $ & $   0.00073 $ & $  10.13430 $ & $ i$\\
$ 55338.88474 $ & $   0.00801 $ & $   0.00073 $ & $  10.13420 $ & $ i$\\
$ 55338.88543 $ & $   0.00701 $ & $   0.00073 $ & $  10.13340 $ & $ i$\\
$ 55338.88608 $ & $   0.00793 $ & $   0.00073 $ & $  10.13430 $ & $ i$\\
$ 55338.88676 $ & $   0.01015 $ & $   0.00074 $ & $  10.13690 $ & $ i$\\
$ 55338.88745 $ & $   0.00842 $ & $   0.00074 $ & $  10.13480 $ & $ i$\\
$ 55338.88813 $ & $   0.00790 $ & $   0.00073 $ & $  10.13430 $ & $ i$\\
$ 55338.88881 $ & $   0.00884 $ & $   0.00074 $ & $  10.13520 $ & $ i$\\
$ 55338.88947 $ & $   0.00774 $ & $   0.00074 $ & $  10.13450 $ & $ i$\\
$ 55338.89014 $ & $   0.00683 $ & $   0.00074 $ & $  10.13340 $ & $ i$\\
$ 55338.89083 $ & $   0.00744 $ & $   0.00074 $ & $  10.13410 $ & $ i$\\
$ 55338.89152 $ & $   0.00726 $ & $   0.00074 $ & $  10.13410 $ & $ i$\\
$ 55338.89220 $ & $   0.00725 $ & $   0.00073 $ & $  10.13350 $ & $ i$\\
$ 55338.89289 $ & $   0.00738 $ & $   0.00073 $ & $  10.13350 $ & $ i$\\
$ 55338.89353 $ & $   0.00768 $ & $   0.00073 $ & $  10.13410 $ & $ i$\\
$ 55338.89422 $ & $   0.00545 $ & $   0.00074 $ & $  10.13280 $ & $ i$\\
$ 55338.89490 $ & $   0.00720 $ & $   0.00074 $ & $  10.13460 $ & $ i$\\
$ 55338.89556 $ & $   0.00674 $ & $   0.00073 $ & $  10.13370 $ & $ i$\\
$ 55338.89626 $ & $   0.00716 $ & $   0.00073 $ & $  10.13330 $ & $ i$\\
$ 55338.89700 $ & $   0.00741 $ & $   0.00073 $ & $  10.13380 $ & $ i$\\
$ 55338.89768 $ & $   0.00596 $ & $   0.00073 $ & $  10.13170 $ & $ i$\\
$ 55338.89837 $ & $   0.00885 $ & $   0.00073 $ & $  10.13520 $ & $ i$\\
$ 55338.89906 $ & $   0.00721 $ & $   0.00074 $ & $  10.13460 $ & $ i$\\
$ 55338.89973 $ & $   0.00900 $ & $   0.00074 $ & $  10.13600 $ & $ i$\\
$ 55338.90041 $ & $   0.00818 $ & $   0.00073 $ & $  10.13440 $ & $ i$\\
$ 55338.90107 $ & $   0.00770 $ & $   0.00073 $ & $  10.13380 $ & $ i$\\
$ 55338.90176 $ & $   0.00841 $ & $   0.00073 $ & $  10.13430 $ & $ i$\\
$ 55338.90245 $ & $   0.00829 $ & $   0.00073 $ & $  10.13410 $ & $ i$\\
$ 55338.90312 $ & $   0.00798 $ & $   0.00073 $ & $  10.13380 $ & $ i$\\
$ 55338.90379 $ & $   0.00792 $ & $   0.00073 $ & $  10.13390 $ & $ i$\\
$ 55338.90447 $ & $   0.00714 $ & $   0.00073 $ & $  10.13320 $ & $ i$\\
$ 55338.90513 $ & $   0.00545 $ & $   0.00073 $ & $  10.13200 $ & $ i$\\
$ 55338.90582 $ & $   0.00690 $ & $   0.00073 $ & $  10.13280 $ & $ i$\\
$ 55338.90650 $ & $   0.00755 $ & $   0.00072 $ & $  10.13290 $ & $ i$\\
$ 55338.90718 $ & $   0.00677 $ & $   0.00073 $ & $  10.13240 $ & $ i$\\
$ 55338.90784 $ & $   0.00749 $ & $   0.00073 $ & $  10.13340 $ & $ i$\\
$ 55338.90851 $ & $   0.00710 $ & $   0.00073 $ & $  10.13320 $ & $ i$\\
$ 55338.90920 $ & $   0.00823 $ & $   0.00073 $ & $  10.13390 $ & $ i$\\
$ 55338.90988 $ & $   0.00714 $ & $   0.00073 $ & $  10.13300 $ & $ i$\\
$ 55338.91056 $ & $   0.00849 $ & $   0.00073 $ & $  10.13370 $ & $ i$\\
$ 55338.91123 $ & $   0.00764 $ & $   0.00073 $ & $  10.13360 $ & $ i$\\
$ 55338.91190 $ & $   0.00846 $ & $   0.00073 $ & $  10.13470 $ & $ i$\\
$ 55338.91259 $ & $   0.00800 $ & $   0.00074 $ & $  10.13500 $ & $ i$\\
$ 55338.91326 $ & $   0.00743 $ & $   0.00073 $ & $  10.13400 $ & $ i$\\
$ 55338.91393 $ & $   0.00927 $ & $   0.00076 $ & $  10.13790 $ & $ i$\\
$ 55338.91459 $ & $   0.00806 $ & $   0.00075 $ & $  10.13530 $ & $ i$\\
$ 55338.91526 $ & $   0.00738 $ & $   0.00073 $ & $  10.13370 $ & $ i$\\
$ 55338.91594 $ & $   0.00799 $ & $   0.00073 $ & $  10.13420 $ & $ i$\\
$ 55338.91663 $ & $   0.00643 $ & $   0.00074 $ & $  10.13330 $ & $ i$\\
$ 55338.91734 $ & $   0.00834 $ & $   0.00074 $ & $  10.13540 $ & $ i$\\
$ 55338.91800 $ & $   0.00774 $ & $   0.00073 $ & $  10.13400 $ & $ i$\\
$ 55338.91868 $ & $   0.00867 $ & $   0.00073 $ & $  10.13420 $ & $ i$\\
$ 55338.91936 $ & $   0.00767 $ & $   0.00074 $ & $  10.13430 $ & $ i$\\
$ 55338.92003 $ & $   0.00884 $ & $   0.00074 $ & $  10.13520 $ & $ i$\\
$ 55338.92071 $ & $   0.00748 $ & $   0.00073 $ & $  10.13370 $ & $ i$\\
$ 55338.92142 $ & $   0.00657 $ & $   0.00073 $ & $  10.13280 $ & $ i$\\
$ 55338.92209 $ & $   0.00844 $ & $   0.00073 $ & $  10.13490 $ & $ i$\\
$ 55338.92277 $ & $   0.00860 $ & $   0.00073 $ & $  10.13430 $ & $ i$\\
$ 55338.92346 $ & $   0.00833 $ & $   0.00073 $ & $  10.13380 $ & $ i$\\
$ 55338.92414 $ & $   0.00886 $ & $   0.00073 $ & $  10.13460 $ & $ i$\\
$ 55338.92483 $ & $   0.00752 $ & $   0.00074 $ & $  10.13420 $ & $ i$\\
$ 55338.92552 $ & $   0.00638 $ & $   0.00073 $ & $  10.13260 $ & $ i$\\
$ 55338.92618 $ & $   0.00806 $ & $   0.00073 $ & $  10.13400 $ & $ i$\\
$ 55338.92686 $ & $   0.00690 $ & $   0.00073 $ & $  10.13200 $ & $ i$\\
$ 55338.92753 $ & $   0.00871 $ & $   0.00073 $ & $  10.13430 $ & $ i$\\
$ 55338.92820 $ & $   0.00777 $ & $   0.00073 $ & $  10.13360 $ & $ i$\\
$ 55338.92887 $ & $   0.00962 $ & $   0.00073 $ & $  10.13520 $ & $ i$\\
$ 55338.92957 $ & $   0.00750 $ & $   0.00073 $ & $  10.13330 $ & $ i$\\
$ 55338.93025 $ & $   0.00853 $ & $   0.00073 $ & $  10.13400 $ & $ i$\\
$ 55338.93093 $ & $   0.00768 $ & $   0.00073 $ & $  10.13380 $ & $ i$\\
$ 55338.93159 $ & $   0.00768 $ & $   0.00073 $ & $  10.13270 $ & $ i$\\
$ 55338.93228 $ & $   0.00727 $ & $   0.00073 $ & $  10.13250 $ & $ i$\\
$ 55338.93296 $ & $   0.00749 $ & $   0.00073 $ & $  10.13310 $ & $ i$\\
$ 55338.93364 $ & $   0.00908 $ & $   0.00073 $ & $  10.13470 $ & $ i$\\
$ 55338.93431 $ & $   0.00775 $ & $   0.00073 $ & $  10.13290 $ & $ i$\\
$ 55338.93502 $ & $   0.00801 $ & $   0.00073 $ & $  10.13290 $ & $ i$\\
$ 55338.93569 $ & $   0.00671 $ & $   0.00073 $ & $  10.13260 $ & $ i$\\
$ 55338.93635 $ & $   0.00805 $ & $   0.00073 $ & $  10.13340 $ & $ i$\\
$ 55338.93703 $ & $   0.00866 $ & $   0.00073 $ & $  10.13400 $ & $ i$\\
$ 55338.93777 $ & $   0.00675 $ & $   0.00073 $ & $  10.13210 $ & $ i$\\
$ 55338.93845 $ & $   0.00669 $ & $   0.00073 $ & $  10.13200 $ & $ i$\\
$ 55338.93912 $ & $   0.00700 $ & $   0.00073 $ & $  10.13230 $ & $ i$\\
$ 55338.93979 $ & $   0.00745 $ & $   0.00073 $ & $  10.13280 $ & $ i$\\
$ 55338.94048 $ & $   0.00819 $ & $   0.00073 $ & $  10.13300 $ & $ i$\\
$ 55338.94117 $ & $   0.00618 $ & $   0.00072 $ & $  10.13130 $ & $ i$\\
$ 55338.94187 $ & $   0.00723 $ & $   0.00072 $ & $  10.13250 $ & $ i$\\
$ 55338.94254 $ & $   0.00684 $ & $   0.00073 $ & $  10.13190 $ & $ i$\\
$ 55338.94323 $ & $   0.00819 $ & $   0.00072 $ & $  10.13270 $ & $ i$\\
$ 55338.94392 $ & $   0.00624 $ & $   0.00073 $ & $  10.13190 $ & $ i$\\
$ 55338.94458 $ & $   0.00695 $ & $   0.00073 $ & $  10.13230 $ & $ i$\\
$ 55338.94525 $ & $   0.00712 $ & $   0.00073 $ & $  10.13200 $ & $ i$\\
$ 55338.94593 $ & $   0.00773 $ & $   0.00072 $ & $  10.13270 $ & $ i$\\
$ 55338.94663 $ & $   0.00747 $ & $   0.00072 $ & $  10.13200 $ & $ i$\\
$ 55338.94730 $ & $   0.00442 $ & $   0.00073 $ & $  10.13000 $ & $ i$\\
$ 55338.94798 $ & $   0.00775 $ & $   0.00072 $ & $  10.13250 $ & $ i$\\
$ 55338.94867 $ & $   0.00790 $ & $   0.00072 $ & $  10.13270 $ & $ i$\\
$ 55338.94935 $ & $   0.00548 $ & $   0.00072 $ & $  10.13060 $ & $ i$\\
$ 55338.95001 $ & $   0.00465 $ & $   0.00072 $ & $  10.12960 $ & $ i$\\
$ 55338.95069 $ & $   0.00532 $ & $   0.00072 $ & $  10.13040 $ & $ i$\\
$ 55338.95139 $ & $   0.00706 $ & $   0.00072 $ & $  10.13230 $ & $ i$\\
$ 55338.95207 $ & $   0.00598 $ & $   0.00073 $ & $  10.13110 $ & $ i$\\
$ 55338.95275 $ & $   0.00669 $ & $   0.00073 $ & $  10.13160 $ & $ i$\\
$ 55338.95341 $ & $   0.00590 $ & $   0.00073 $ & $  10.13110 $ & $ i$\\
$ 55338.95411 $ & $   0.00789 $ & $   0.00073 $ & $  10.13270 $ & $ i$\\
$ 55338.95480 $ & $   0.00904 $ & $   0.00073 $ & $  10.13430 $ & $ i$\\
$ 55338.95547 $ & $   0.00802 $ & $   0.00073 $ & $  10.13300 $ & $ i$\\
$ 55338.95613 $ & $   0.00430 $ & $   0.00072 $ & $  10.12910 $ & $ i$\\
$ 55338.95682 $ & $   0.00669 $ & $   0.00072 $ & $  10.13160 $ & $ i$\\
$ 55338.95750 $ & $   0.00636 $ & $   0.00073 $ & $  10.13180 $ & $ i$\\
$ 55338.95823 $ & $   0.00554 $ & $   0.00073 $ & $  10.13080 $ & $ i$\\
$ 55338.95890 $ & $   0.00528 $ & $   0.00072 $ & $  10.13010 $ & $ i$\\
$ 55338.95959 $ & $   0.00445 $ & $   0.00072 $ & $  10.12950 $ & $ i$\\
$ 55338.96025 $ & $   0.00629 $ & $   0.00072 $ & $  10.13160 $ & $ i$\\
$ 55338.96094 $ & $   0.00521 $ & $   0.00072 $ & $  10.13090 $ & $ i$\\
$ 55338.96162 $ & $   0.00536 $ & $   0.00072 $ & $  10.13040 $ & $ i$\\
$ 55338.96231 $ & $   0.00588 $ & $   0.00073 $ & $  10.13150 $ & $ i$\\
$ 55338.96298 $ & $   0.00659 $ & $   0.00073 $ & $  10.13240 $ & $ i$\\
$ 55338.96366 $ & $   0.00564 $ & $   0.00074 $ & $  10.13220 $ & $ i$\\
$ 55338.96433 $ & $   0.00370 $ & $   0.00073 $ & $  10.13070 $ & $ i$\\
$ 55338.96501 $ & $   0.00538 $ & $   0.00072 $ & $  10.13090 $ & $ i$\\
$ 55338.96568 $ & $   0.00228 $ & $   0.00073 $ & $  10.12780 $ & $ i$\\
$ 55338.96635 $ & $   0.00514 $ & $   0.00072 $ & $  10.12990 $ & $ i$\\
$ 55338.96705 $ & $   0.00266 $ & $   0.00073 $ & $  10.12900 $ & $ i$\\
$ 55338.96773 $ & $   0.00152 $ & $   0.00073 $ & $  10.12760 $ & $ i$\\
$ 55338.96842 $ & $   0.00333 $ & $   0.00073 $ & $  10.12960 $ & $ i$\\
$ 55338.96907 $ & $   0.00090 $ & $   0.00072 $ & $  10.12630 $ & $ i$\\
$ 55338.96973 $ & $   0.00397 $ & $   0.00073 $ & $  10.12930 $ & $ i$\\
$ 55338.97042 $ & $   0.00071 $ & $   0.00072 $ & $  10.12620 $ & $ i$\\
$ 55338.97110 $ & $   0.00244 $ & $   0.00072 $ & $  10.12760 $ & $ i$\\
$ 55338.97178 $ & $   0.00007 $ & $   0.00072 $ & $  10.12520 $ & $ i$\\
$ 55480.59376 $ & $   0.00144 $ & $   0.00080 $ & $   9.13948 $ & $  $\\
$ 55480.59409 $ & $   0.00313 $ & $   0.00080 $ & $   9.14170 $ & $  $\\
$ 55480.59441 $ & $  -0.00141 $ & $   0.00080 $ & $   9.13698 $ & $  $\\
$ 55480.59475 $ & $  -0.00031 $ & $   0.00079 $ & $   9.13803 $ & $  $\\
$ 55480.59510 $ & $   0.00107 $ & $   0.00080 $ & $   9.13926 $ & $  $\\
$ 55480.59542 $ & $  -0.00243 $ & $   0.00080 $ & $   9.13627 $ & $  $\\
$ 55480.59575 $ & $  -0.00152 $ & $   0.00080 $ & $   9.13636 $ & $  $\\
$ 55480.59609 $ & $  -0.00010 $ & $   0.00080 $ & $   9.13811 $ & $  $\\
$ 55480.59643 $ & $  -0.00125 $ & $   0.00080 $ & $   9.13751 $ & $  $\\
$ 55480.59679 $ & $   0.00050 $ & $   0.00080 $ & $   9.13874 $ & $  $\\
$ 55480.59711 $ & $   0.00233 $ & $   0.00080 $ & $   9.14054 $ & $  $\\
$ 55480.59744 $ & $   0.00067 $ & $   0.00080 $ & $   9.13862 $ & $  $\\
$ 55480.59777 $ & $  -0.00021 $ & $   0.00080 $ & $   9.13862 $ & $  $\\
$ 55480.59811 $ & $  -0.00082 $ & $   0.00080 $ & $   9.13798 $ & $  $\\
$ 55480.59843 $ & $  -0.00016 $ & $   0.00079 $ & $   9.13825 $ & $  $\\
$ 55480.59876 $ & $   0.00089 $ & $   0.00080 $ & $   9.13951 $ & $  $\\
$ 55480.59909 $ & $  -0.00072 $ & $   0.00080 $ & $   9.13769 $ & $  $\\
$ 55480.59943 $ & $  -0.00107 $ & $   0.00080 $ & $   9.13738 $ & $  $\\
$ 55480.59976 $ & $   0.00316 $ & $   0.00080 $ & $   9.14210 $ & $  $\\
$ 55480.60010 $ & $   0.00268 $ & $   0.00080 $ & $   9.14148 $ & $  $\\
$ 55480.60041 $ & $  -0.00057 $ & $   0.00080 $ & $   9.13780 $ & $  $\\
$ 55480.60076 $ & $   0.00284 $ & $   0.00080 $ & $   9.14128 $ & $  $\\
$ 55480.60108 $ & $   0.00111 $ & $   0.00080 $ & $   9.13999 $ & $  $\\
$ 55480.60142 $ & $   0.00221 $ & $   0.00080 $ & $   9.14099 $ & $  $\\
$ 55480.60174 $ & $   0.00159 $ & $   0.00080 $ & $   9.14092 $ & $  $\\
$ 55480.60209 $ & $   0.00207 $ & $   0.00080 $ & $   9.14026 $ & $  $\\
$ 55480.60242 $ & $   0.00161 $ & $   0.00080 $ & $   9.14004 $ & $  $\\
$ 55480.60275 $ & $   0.00211 $ & $   0.00080 $ & $   9.14086 $ & $  $\\
$ 55480.60308 $ & $   0.00364 $ & $   0.00080 $ & $   9.14178 $ & $  $\\
$ 55480.60342 $ & $   0.00167 $ & $   0.00080 $ & $   9.14054 $ & $  $\\
$ 55480.60374 $ & $   0.00563 $ & $   0.00080 $ & $   9.14462 $ & $  $\\
$ 55480.60408 $ & $   0.00314 $ & $   0.00080 $ & $   9.14156 $ & $  $\\
$ 55480.60440 $ & $   0.00573 $ & $   0.00080 $ & $   9.14452 $ & $  $\\
$ 55480.60475 $ & $   0.00522 $ & $   0.00080 $ & $   9.14383 $ & $  $\\
$ 55480.60507 $ & $   0.00380 $ & $   0.00080 $ & $   9.14193 $ & $  $\\
$ 55480.60540 $ & $   0.00410 $ & $   0.00080 $ & $   9.14236 $ & $  $\\
$ 55480.60575 $ & $   0.00332 $ & $   0.00080 $ & $   9.14224 $ & $  $\\
$ 55480.60608 $ & $   0.00435 $ & $   0.00080 $ & $   9.14317 $ & $  $\\
$ 55480.60639 $ & $   0.00671 $ & $   0.00080 $ & $   9.14515 $ & $  $\\
$ 55480.60673 $ & $   0.00532 $ & $   0.00080 $ & $   9.14405 $ & $  $\\
$ 55480.60705 $ & $   0.00662 $ & $   0.00080 $ & $   9.14494 $ & $  $\\
$ 55480.60739 $ & $   0.00287 $ & $   0.00080 $ & $   9.14176 $ & $  $\\
$ 55480.60771 $ & $   0.00447 $ & $   0.00080 $ & $   9.14303 $ & $  $\\
$ 55480.60805 $ & $   0.00533 $ & $   0.00080 $ & $   9.14429 $ & $  $\\
$ 55480.60836 $ & $   0.00413 $ & $   0.00080 $ & $   9.14309 $ & $  $\\
$ 55480.60870 $ & $   0.00556 $ & $   0.00080 $ & $   9.14427 $ & $  $\\
$ 55480.60903 $ & $   0.00843 $ & $   0.00080 $ & $   9.14737 $ & $  $\\
$ 55480.60936 $ & $   0.00718 $ & $   0.00080 $ & $   9.14607 $ & $  $\\
$ 55480.60970 $ & $   0.00903 $ & $   0.00080 $ & $   9.14818 $ & $  $\\
$ 55480.61004 $ & $   0.00764 $ & $   0.00080 $ & $   9.14656 $ & $  $\\
$ 55480.61037 $ & $   0.00596 $ & $   0.00080 $ & $   9.14453 $ & $  $\\
$ 55480.61070 $ & $   0.00655 $ & $   0.00080 $ & $   9.14551 $ & $  $\\
$ 55480.61102 $ & $   0.00672 $ & $   0.00080 $ & $   9.14581 $ & $  $\\
$ 55480.61136 $ & $   0.00693 $ & $   0.00080 $ & $   9.14554 $ & $  $\\
$ 55480.61169 $ & $   0.01012 $ & $   0.00080 $ & $   9.14917 $ & $  $\\
$ 55480.61204 $ & $   0.00582 $ & $   0.00080 $ & $   9.14435 $ & $  $\\
$ 55480.61235 $ & $   0.00681 $ & $   0.00080 $ & $   9.14593 $ & $  $\\
$ 55480.61270 $ & $   0.00551 $ & $   0.00080 $ & $   9.14497 $ & $  $\\
$ 55480.61302 $ & $   0.00785 $ & $   0.00080 $ & $   9.14701 $ & $  $\\
$ 55480.61336 $ & $   0.00864 $ & $   0.00080 $ & $   9.14775 $ & $  $\\
$ 55480.61370 $ & $   0.00440 $ & $   0.00080 $ & $   9.14372 $ & $  $\\
$ 55480.61404 $ & $   0.00442 $ & $   0.00080 $ & $   9.14388 $ & $  $\\
$ 55480.61438 $ & $   0.00749 $ & $   0.00080 $ & $   9.14704 $ & $  $\\
$ 55480.61469 $ & $   0.00683 $ & $   0.00080 $ & $   9.14641 $ & $  $\\
$ 55480.61504 $ & $   0.00552 $ & $   0.00081 $ & $   9.14555 $ & $  $\\
$ 55480.61535 $ & $   0.00678 $ & $   0.00080 $ & $   9.14606 $ & $  $\\
$ 55480.61569 $ & $   0.00630 $ & $   0.00080 $ & $   9.14618 $ & $  $\\
$ 55480.61603 $ & $   0.00688 $ & $   0.00080 $ & $   9.14637 $ & $  $\\
$ 55480.61637 $ & $   0.00781 $ & $   0.00080 $ & $   9.14655 $ & $  $\\
$ 55480.61671 $ & $   0.00697 $ & $   0.00080 $ & $   9.14600 $ & $  $\\
$ 55480.61703 $ & $   0.00889 $ & $   0.00080 $ & $   9.14869 $ & $  $\\
$ 55480.61733 $ & $   0.00880 $ & $   0.00080 $ & $   9.14802 $ & $  $\\
$ 55480.61765 $ & $   0.00767 $ & $   0.00080 $ & $   9.14693 $ & $  $\\
$ 55480.61794 $ & $   0.00881 $ & $   0.00080 $ & $   9.14784 $ & $  $\\
$ 55480.61829 $ & $   0.00659 $ & $   0.00080 $ & $   9.14592 $ & $  $\\
$ 55480.61863 $ & $   0.00888 $ & $   0.00080 $ & $   9.14852 $ & $  $\\
$ 55480.61895 $ & $   0.00691 $ & $   0.00080 $ & $   9.14641 $ & $  $\\
$ 55480.61927 $ & $   0.00692 $ & $   0.00080 $ & $   9.14624 $ & $  $\\
$ 55480.61959 $ & $   0.00725 $ & $   0.00080 $ & $   9.14625 $ & $  $\\
$ 55480.61993 $ & $   0.00621 $ & $   0.00080 $ & $   9.14542 $ & $  $\\
$ 55480.62027 $ & $   0.00522 $ & $   0.00080 $ & $   9.14436 $ & $  $\\
$ 55480.62062 $ & $   0.00778 $ & $   0.00080 $ & $   9.14724 $ & $  $\\
$ 55480.62095 $ & $   0.00859 $ & $   0.00080 $ & $   9.14801 $ & $  $\\
$ 55480.62128 $ & $   0.00564 $ & $   0.00080 $ & $   9.14435 $ & $  $\\
$ 55480.62161 $ & $   0.00701 $ & $   0.00080 $ & $   9.14588 $ & $  $\\
$ 55480.62196 $ & $   0.00722 $ & $   0.00080 $ & $   9.14655 $ & $  $\\
$ 55480.62228 $ & $   0.00543 $ & $   0.00080 $ & $   9.14518 $ & $  $\\
$ 55480.62262 $ & $   0.00536 $ & $   0.00080 $ & $   9.14527 $ & $  $\\
$ 55480.62297 $ & $   0.00663 $ & $   0.00080 $ & $   9.14570 $ & $  $\\
$ 55480.62327 $ & $   0.00449 $ & $   0.00080 $ & $   9.14342 $ & $  $\\
$ 55480.62359 $ & $   0.00500 $ & $   0.00080 $ & $   9.14442 $ & $  $\\
$ 55480.62392 $ & $   0.00757 $ & $   0.00080 $ & $   9.14689 $ & $  $\\
$ 55480.62425 $ & $   0.00644 $ & $   0.00080 $ & $   9.14537 $ & $  $\\
$ 55480.62460 $ & $   0.00717 $ & $   0.00080 $ & $   9.14642 $ & $  $\\
$ 55480.62493 $ & $   0.00361 $ & $   0.00080 $ & $   9.14306 $ & $  $\\
$ 55480.62525 $ & $   0.00825 $ & $   0.00080 $ & $   9.14805 $ & $  $\\
$ 55480.62559 $ & $   0.00686 $ & $   0.00080 $ & $   9.14660 $ & $  $\\
$ 55480.62592 $ & $   0.00786 $ & $   0.00080 $ & $   9.14731 $ & $  $\\
$ 55480.62624 $ & $   0.00829 $ & $   0.00080 $ & $   9.14775 $ & $  $\\
$ 55480.62659 $ & $   0.00733 $ & $   0.00080 $ & $   9.14684 $ & $  $\\
$ 55480.62694 $ & $   0.00680 $ & $   0.00080 $ & $   9.14530 $ & $  $\\
$ 55480.62727 $ & $   0.00772 $ & $   0.00080 $ & $   9.14687 $ & $  $\\
$ 55480.62762 $ & $   0.00391 $ & $   0.00080 $ & $   9.14268 $ & $  $\\
$ 55480.62794 $ & $   0.00526 $ & $   0.00080 $ & $   9.14483 $ & $  $\\
$ 55480.62828 $ & $   0.00864 $ & $   0.00080 $ & $   9.14790 $ & $  $\\
$ 55480.62863 $ & $   0.00759 $ & $   0.00080 $ & $   9.14667 $ & $  $\\
$ 55480.62896 $ & $   0.00884 $ & $   0.00080 $ & $   9.14780 $ & $  $\\
$ 55480.62929 $ & $   0.00768 $ & $   0.00080 $ & $   9.14658 $ & $  $\\
$ 55480.62962 $ & $   0.00616 $ & $   0.00080 $ & $   9.14536 $ & $  $\\
$ 55480.62996 $ & $   0.00853 $ & $   0.00080 $ & $   9.14724 $ & $  $\\
$ 55480.63028 $ & $   0.00577 $ & $   0.00080 $ & $   9.14452 $ & $  $\\
$ 55480.63060 $ & $   0.00853 $ & $   0.00080 $ & $   9.14752 $ & $  $\\
$ 55480.63095 $ & $   0.00926 $ & $   0.00080 $ & $   9.14849 $ & $  $\\
$ 55480.63126 $ & $   0.00740 $ & $   0.00080 $ & $   9.14718 $ & $  $\\
$ 55480.63162 $ & $   0.00701 $ & $   0.00080 $ & $   9.14656 $ & $  $\\
$ 55480.63194 $ & $   0.00637 $ & $   0.00080 $ & $   9.14576 $ & $  $\\
$ 55480.63228 $ & $   0.00538 $ & $   0.00080 $ & $   9.14476 $ & $  $\\
$ 55480.63261 $ & $   0.00628 $ & $   0.00080 $ & $   9.14515 $ & $  $\\
$ 55480.63295 $ & $   0.00458 $ & $   0.00080 $ & $   9.14353 $ & $  $\\
$ 55480.63328 $ & $   0.00622 $ & $   0.00080 $ & $   9.14577 $ & $  $\\
$ 55480.63360 $ & $   0.00689 $ & $   0.00080 $ & $   9.14640 $ & $  $\\
$ 55480.63395 $ & $   0.01080 $ & $   0.00080 $ & $   9.15005 $ & $  $\\
$ 55480.63427 $ & $   0.00716 $ & $   0.00080 $ & $   9.14622 $ & $  $\\
$ 55480.63460 $ & $   0.00827 $ & $   0.00080 $ & $   9.14767 $ & $  $\\
$ 55480.63494 $ & $   0.00706 $ & $   0.00080 $ & $   9.14642 $ & $  $\\
$ 55480.63527 $ & $   0.00713 $ & $   0.00080 $ & $   9.14593 $ & $  $\\
$ 55480.63560 $ & $   0.00476 $ & $   0.00080 $ & $   9.14429 $ & $  $\\
$ 55480.63593 $ & $   0.00731 $ & $   0.00080 $ & $   9.14629 $ & $  $\\
$ 55480.63626 $ & $   0.00892 $ & $   0.00080 $ & $   9.14812 $ & $  $\\
$ 55480.63661 $ & $   0.00570 $ & $   0.00080 $ & $   9.14540 $ & $  $\\
$ 55480.63692 $ & $   0.00839 $ & $   0.00080 $ & $   9.14781 $ & $  $\\
$ 55480.63724 $ & $   0.00424 $ & $   0.00080 $ & $   9.14399 $ & $  $\\
$ 55480.63755 $ & $   0.00559 $ & $   0.00080 $ & $   9.14569 $ & $  $\\
$ 55480.63788 $ & $   0.00679 $ & $   0.00081 $ & $   9.14683 $ & $  $\\
$ 55480.63821 $ & $   0.00743 $ & $   0.00080 $ & $   9.14659 $ & $  $\\
$ 55480.63853 $ & $   0.00700 $ & $   0.00080 $ & $   9.14636 $ & $  $\\
$ 55480.63886 $ & $   0.01006 $ & $   0.00080 $ & $   9.14964 $ & $  $\\
$ 55480.63920 $ & $   0.00888 $ & $   0.00080 $ & $   9.14865 $ & $  $\\
$ 55480.63953 $ & $   0.00821 $ & $   0.00080 $ & $   9.14783 $ & $  $\\
$ 55480.63983 $ & $   0.00571 $ & $   0.00080 $ & $   9.14515 $ & $  $\\
$ 55480.64018 $ & $   0.00687 $ & $   0.00080 $ & $   9.14624 $ & $  $\\
$ 55480.64050 $ & $   0.00856 $ & $   0.00080 $ & $   9.14763 $ & $  $\\
$ 55480.64085 $ & $   0.00432 $ & $   0.00080 $ & $   9.14372 $ & $  $\\
$ 55480.64117 $ & $   0.00624 $ & $   0.00080 $ & $   9.14504 $ & $  $\\
$ 55480.64152 $ & $   0.00769 $ & $   0.00080 $ & $   9.14661 $ & $  $\\
$ 55480.64184 $ & $   0.00895 $ & $   0.00080 $ & $   9.14846 $ & $  $\\
$ 55480.64219 $ & $   0.00740 $ & $   0.00080 $ & $   9.14697 $ & $  $\\
$ 55480.64249 $ & $   0.00788 $ & $   0.00080 $ & $   9.14714 $ & $  $\\
$ 55480.64284 $ & $   0.00501 $ & $   0.00080 $ & $   9.14432 $ & $  $\\
$ 55480.64317 $ & $   0.00796 $ & $   0.00080 $ & $   9.14706 $ & $  $\\
$ 55480.64351 $ & $   0.00789 $ & $   0.00080 $ & $   9.14745 $ & $  $\\
$ 55480.64383 $ & $   0.00858 $ & $   0.00080 $ & $   9.14814 $ & $  $\\
$ 55480.64417 $ & $   0.00892 $ & $   0.00080 $ & $   9.14904 $ & $  $\\
$ 55480.64449 $ & $   0.00580 $ & $   0.00081 $ & $   9.14570 $ & $  $\\
$ 55480.64485 $ & $   0.00595 $ & $   0.00080 $ & $   9.14554 $ & $  $\\
$ 55480.64514 $ & $   0.00357 $ & $   0.00080 $ & $   9.14268 $ & $  $\\
$ 55480.64549 $ & $   0.00985 $ & $   0.00080 $ & $   9.14933 $ & $  $\\
$ 55480.64581 $ & $   0.00758 $ & $   0.00080 $ & $   9.14715 $ & $  $\\
$ 55480.64615 $ & $   0.00565 $ & $   0.00080 $ & $   9.14545 $ & $  $\\
$ 55480.64650 $ & $   0.00989 $ & $   0.00080 $ & $   9.14831 $ & $  $\\
$ 55480.64681 $ & $   0.00573 $ & $   0.00080 $ & $   9.14550 $ & $  $\\
$ 55480.64714 $ & $   0.00620 $ & $   0.00080 $ & $   9.14622 $ & $  $\\
$ 55480.64748 $ & $   0.00865 $ & $   0.00080 $ & $   9.14817 $ & $  $\\
$ 55480.64781 $ & $   0.00758 $ & $   0.00081 $ & $   9.14791 $ & $  $\\
$ 55480.64814 $ & $   0.00926 $ & $   0.00081 $ & $   9.15008 $ & $  $\\
$ 55480.64847 $ & $   0.00853 $ & $   0.00080 $ & $   9.14820 $ & $  $\\
$ 55480.64881 $ & $   0.00776 $ & $   0.00080 $ & $   9.14730 $ & $  $\\
$ 55480.64914 $ & $   0.00641 $ & $   0.00080 $ & $   9.14541 $ & $  $\\
$ 55480.64948 $ & $   0.01038 $ & $   0.00080 $ & $   9.15027 $ & $  $\\
$ 55480.64982 $ & $   0.00793 $ & $   0.00080 $ & $   9.14753 $ & $  $\\
$ 55480.65015 $ & $   0.00489 $ & $   0.00080 $ & $   9.14397 $ & $  $\\
$ 55480.65049 $ & $   0.01269 $ & $   0.00080 $ & $   9.15185 $ & $  $\\
$ 55480.65081 $ & $   0.00771 $ & $   0.00080 $ & $   9.14673 $ & $  $\\
$ 55480.65115 $ & $   0.00855 $ & $   0.00080 $ & $   9.14749 $ & $  $\\
$ 55480.65144 $ & $   0.00739 $ & $   0.00080 $ & $   9.14608 $ & $  $\\
$ 55480.65178 $ & $   0.00469 $ & $   0.00080 $ & $   9.14304 $ & $  $\\
$ 55480.65211 $ & $   0.00757 $ & $   0.00080 $ & $   9.14656 $ & $  $\\
$ 55480.65245 $ & $   0.00811 $ & $   0.00080 $ & $   9.14725 $ & $  $\\
$ 55480.65278 $ & $   0.00719 $ & $   0.00080 $ & $   9.14627 $ & $  $\\
$ 55480.65310 $ & $   0.00602 $ & $   0.00080 $ & $   9.14550 $ & $  $\\
$ 55480.65345 $ & $   0.00674 $ & $   0.00080 $ & $   9.14580 $ & $  $\\
$ 55480.65379 $ & $   0.00857 $ & $   0.00080 $ & $   9.14823 $ & $  $\\
$ 55480.65411 $ & $   0.00955 $ & $   0.00080 $ & $   9.14924 $ & $  $\\
$ 55480.65443 $ & $   0.00878 $ & $   0.00080 $ & $   9.14829 $ & $  $\\
$ 55480.65478 $ & $   0.00783 $ & $   0.00080 $ & $   9.14722 $ & $  $\\
$ 55480.65511 $ & $   0.00554 $ & $   0.00080 $ & $   9.14407 $ & $  $\\
$ 55480.65545 $ & $   0.00646 $ & $   0.00080 $ & $   9.14558 $ & $  $\\
$ 55480.65578 $ & $   0.00449 $ & $   0.00080 $ & $   9.14332 $ & $  $\\
$ 55480.65610 $ & $   0.00996 $ & $   0.00080 $ & $   9.14882 $ & $  $\\
$ 55480.65645 $ & $   0.00914 $ & $   0.00080 $ & $   9.14805 $ & $  $\\
$ 55480.65677 $ & $   0.00593 $ & $   0.00080 $ & $   9.14534 $ & $  $\\
$ 55480.65708 $ & $   0.00432 $ & $   0.00080 $ & $   9.14363 $ & $  $\\
$ 55480.65741 $ & $   0.00781 $ & $   0.00080 $ & $   9.14732 $ & $  $\\
$ 55480.65776 $ & $   0.00948 $ & $   0.00080 $ & $   9.14902 $ & $  $\\
$ 55480.65808 $ & $   0.00810 $ & $   0.00080 $ & $   9.14747 $ & $  $\\
$ 55480.65843 $ & $   0.00905 $ & $   0.00080 $ & $   9.14861 $ & $  $\\
$ 55480.65875 $ & $   0.00747 $ & $   0.00080 $ & $   9.14664 $ & $  $\\
$ 55480.65909 $ & $   0.00872 $ & $   0.00080 $ & $   9.14763 $ & $  $\\
$ 55480.65942 $ & $   0.00519 $ & $   0.00080 $ & $   9.14522 $ & $  $\\
$ 55480.65976 $ & $   0.00766 $ & $   0.00080 $ & $   9.14679 $ & $  $\\
$ 55480.66011 $ & $   0.00847 $ & $   0.00080 $ & $   9.14787 $ & $  $\\
$ 55480.66045 $ & $   0.00569 $ & $   0.00080 $ & $   9.14496 $ & $  $\\
$ 55480.66078 $ & $   0.00904 $ & $   0.00080 $ & $   9.14792 $ & $  $\\
$ 55480.66110 $ & $   0.00655 $ & $   0.00080 $ & $   9.14506 $ & $  $\\
$ 55480.66142 $ & $   0.00794 $ & $   0.00080 $ & $   9.14686 $ & $  $\\
$ 55480.66176 $ & $   0.00836 $ & $   0.00080 $ & $   9.14812 $ & $  $\\
$ 55480.66208 $ & $   0.00756 $ & $   0.00080 $ & $   9.14711 $ & $  $\\
$ 55480.66242 $ & $   0.00652 $ & $   0.00080 $ & $   9.14573 $ & $  $\\
$ 55480.66274 $ & $   0.00669 $ & $   0.00080 $ & $   9.14518 $ & $  $\\
$ 55480.66309 $ & $   0.00728 $ & $   0.00080 $ & $   9.14633 $ & $  $\\
$ 55480.66340 $ & $   0.00691 $ & $   0.00080 $ & $   9.14601 $ & $  $\\
$ 55480.66375 $ & $   0.00639 $ & $   0.00080 $ & $   9.14531 $ & $  $\\
$ 55480.66409 $ & $   0.00971 $ & $   0.00080 $ & $   9.14878 $ & $  $\\
$ 55480.66442 $ & $   0.00614 $ & $   0.00080 $ & $   9.14490 $ & $  $\\
$ 55480.66475 $ & $   0.00459 $ & $   0.00080 $ & $   9.14286 $ & $  $\\
$ 55480.66509 $ & $   0.00724 $ & $   0.00080 $ & $   9.14598 $ & $  $\\
$ 55480.66542 $ & $   0.00853 $ & $   0.00080 $ & $   9.14746 $ & $  $\\
$ 55480.66574 $ & $   0.00676 $ & $   0.00080 $ & $   9.14576 $ & $  $\\
$ 55480.66605 $ & $   0.00757 $ & $   0.00080 $ & $   9.14678 $ & $  $\\
$ 55480.66640 $ & $   0.00756 $ & $   0.00080 $ & $   9.14726 $ & $  $\\
$ 55480.66672 $ & $   0.00764 $ & $   0.00080 $ & $   9.14671 $ & $  $\\
$ 55480.66706 $ & $   0.00786 $ & $   0.00080 $ & $   9.14667 $ & $  $\\
$ 55480.66736 $ & $   0.00733 $ & $   0.00081 $ & $   9.14745 $ & $  $\\
$ 55480.66770 $ & $   0.00658 $ & $   0.00081 $ & $   9.14655 $ & $  $\\
$ 55480.66803 $ & $   0.00810 $ & $   0.00080 $ & $   9.14736 $ & $  $\\
$ 55480.66836 $ & $   0.00754 $ & $   0.00080 $ & $   9.14656 $ & $  $\\
$ 55480.66870 $ & $   0.00857 $ & $   0.00080 $ & $   9.14848 $ & $  $\\
$ 55480.66903 $ & $   0.01025 $ & $   0.00081 $ & $   9.14998 $ & $  $\\
$ 55480.66933 $ & $   0.00700 $ & $   0.00080 $ & $   9.14642 $ & $  $\\
$ 55480.66966 $ & $   0.01041 $ & $   0.00080 $ & $   9.14972 $ & $  $\\
$ 55480.67001 $ & $   0.00816 $ & $   0.00080 $ & $   9.14688 $ & $  $\\
$ 55480.67035 $ & $   0.00537 $ & $   0.00080 $ & $   9.14451 $ & $  $\\
$ 55480.67068 $ & $   0.00853 $ & $   0.00080 $ & $   9.14688 $ & $  $\\
$ 55480.67100 $ & $   0.00840 $ & $   0.00080 $ & $   9.14689 $ & $  $\\
$ 55480.67134 $ & $   0.00620 $ & $   0.00080 $ & $   9.14567 $ & $  $\\
$ 55480.67168 $ & $   0.01049 $ & $   0.00080 $ & $   9.14948 $ & $  $\\
$ 55480.67197 $ & $   0.00746 $ & $   0.00080 $ & $   9.14606 $ & $  $\\
$ 55480.67231 $ & $   0.00843 $ & $   0.00080 $ & $   9.14669 $ & $  $\\
$ 55480.67265 $ & $   0.00841 $ & $   0.00080 $ & $   9.14683 $ & $  $\\
$ 55480.67297 $ & $   0.00926 $ & $   0.00080 $ & $   9.14766 $ & $  $\\
$ 55480.67331 $ & $   0.00777 $ & $   0.00080 $ & $   9.14622 $ & $  $\\
$ 55480.67365 $ & $   0.00615 $ & $   0.00080 $ & $   9.14429 $ & $  $\\
$ 55480.67397 $ & $   0.00792 $ & $   0.00080 $ & $   9.14651 $ & $  $\\
$ 55480.67430 $ & $   0.00807 $ & $   0.00080 $ & $   9.14613 $ & $  $\\
$ 55480.67470 $ & $   0.00799 $ & $   0.00080 $ & $   9.14712 $ & $  $\\
$ 55480.67510 $ & $   0.00588 $ & $   0.00080 $ & $   9.14483 $ & $  $\\
$ 55480.67549 $ & $   0.00890 $ & $   0.00080 $ & $   9.14701 $ & $  $\\
$ 55480.67587 $ & $   0.00902 $ & $   0.00080 $ & $   9.14740 $ & $  $\\
$ 55480.67624 $ & $   0.00809 $ & $   0.00080 $ & $   9.14669 $ & $  $\\
$ 55480.67656 $ & $   0.00955 $ & $   0.00080 $ & $   9.14844 $ & $  $\\
$ 55480.67691 $ & $   0.00754 $ & $   0.00080 $ & $   9.14599 $ & $  $\\
$ 55480.67722 $ & $   0.01059 $ & $   0.00080 $ & $   9.14879 $ & $  $\\
$ 55480.67756 $ & $   0.00832 $ & $   0.00080 $ & $   9.14700 $ & $  $\\
$ 55480.67789 $ & $   0.00955 $ & $   0.00080 $ & $   9.14718 $ & $  $\\
$ 55480.67824 $ & $   0.00632 $ & $   0.00080 $ & $   9.14483 $ & $  $\\
$ 55480.67856 $ & $   0.00778 $ & $   0.00080 $ & $   9.14620 $ & $  $\\
$ 55480.67889 $ & $   0.00631 $ & $   0.00080 $ & $   9.14434 $ & $  $\\
$ 55480.67924 $ & $   0.00623 $ & $   0.00080 $ & $   9.14469 $ & $  $\\
$ 55480.67956 $ & $   0.00674 $ & $   0.00080 $ & $   9.14482 $ & $  $\\
$ 55480.67988 $ & $   0.00907 $ & $   0.00080 $ & $   9.14681 $ & $  $\\
$ 55480.68023 $ & $   0.00720 $ & $   0.00080 $ & $   9.14440 $ & $  $\\
$ 55480.68055 $ & $   0.00581 $ & $   0.00080 $ & $   9.14390 $ & $  $\\
$ 55480.68090 $ & $   0.00659 $ & $   0.00080 $ & $   9.14461 $ & $  $\\
$ 55480.68121 $ & $   0.00907 $ & $   0.00080 $ & $   9.14735 $ & $  $\\
$ 55480.68156 $ & $   0.00871 $ & $   0.00080 $ & $   9.14640 $ & $  $\\
$ 55480.68190 $ & $   0.00674 $ & $   0.00080 $ & $   9.14513 $ & $  $\\
$ 55480.68222 $ & $   0.00934 $ & $   0.00080 $ & $   9.14736 $ & $  $\\
$ 55480.68256 $ & $   0.00653 $ & $   0.00080 $ & $   9.14507 $ & $  $\\
$ 55480.68288 $ & $   0.00597 $ & $   0.00080 $ & $   9.14408 $ & $  $\\
$ 55480.68323 $ & $   0.00930 $ & $   0.00080 $ & $   9.14748 $ & $  $\\
$ 55480.68355 $ & $   0.00551 $ & $   0.00080 $ & $   9.14312 $ & $  $\\
$ 55480.68390 $ & $   0.00781 $ & $   0.00080 $ & $   9.14620 $ & $  $\\
$ 55480.68424 $ & $   0.00754 $ & $   0.00080 $ & $   9.14556 $ & $  $\\
$ 55480.68455 $ & $   0.00742 $ & $   0.00080 $ & $   9.14568 $ & $  $\\
$ 55480.68487 $ & $   0.00714 $ & $   0.00080 $ & $   9.14518 $ & $  $\\
$ 55480.68521 $ & $   0.00786 $ & $   0.00080 $ & $   9.14574 $ & $  $\\
$ 55480.68551 $ & $   0.00598 $ & $   0.00080 $ & $   9.14453 $ & $  $\\
$ 55480.68583 $ & $   0.01052 $ & $   0.00080 $ & $   9.14916 $ & $  $\\
$ 55480.68618 $ & $   0.00781 $ & $   0.00080 $ & $   9.14614 $ & $  $\\
$ 55480.68652 $ & $   0.00829 $ & $   0.00080 $ & $   9.14639 $ & $  $\\
$ 55480.68683 $ & $   0.00549 $ & $   0.00080 $ & $   9.14426 $ & $  $\\
$ 55480.68716 $ & $   0.00778 $ & $   0.00080 $ & $   9.14652 $ & $  $\\
$ 55480.68750 $ & $   0.00637 $ & $   0.00080 $ & $   9.14438 $ & $  $\\
$ 55480.68783 $ & $   0.00678 $ & $   0.00080 $ & $   9.14462 $ & $  $\\
$ 55480.68815 $ & $   0.00702 $ & $   0.00080 $ & $   9.14456 $ & $  $\\
$ 55480.68849 $ & $   0.00999 $ & $   0.00080 $ & $   9.14818 $ & $  $\\
$ 55480.68882 $ & $   0.00738 $ & $   0.00080 $ & $   9.14547 $ & $  $\\
$ 55480.68916 $ & $   0.00825 $ & $   0.00080 $ & $   9.14621 $ & $  $\\
$ 55480.68950 $ & $   0.00660 $ & $   0.00080 $ & $   9.14468 $ & $  $\\
$ 55480.68981 $ & $   0.00837 $ & $   0.00080 $ & $   9.14624 $ & $  $\\
$ 55480.69015 $ & $   0.01019 $ & $   0.00080 $ & $   9.14826 $ & $  $\\
$ 55480.69048 $ & $   0.00542 $ & $   0.00080 $ & $   9.14390 $ & $  $\\
$ 55480.69087 $ & $   0.00711 $ & $   0.00080 $ & $   9.14550 $ & $  $\\
$ 55480.69125 $ & $   0.00647 $ & $   0.00080 $ & $   9.14472 $ & $  $\\
$ 55480.69163 $ & $   0.00531 $ & $   0.00080 $ & $   9.14324 $ & $  $\\
$ 55480.69200 $ & $   0.00701 $ & $   0.00080 $ & $   9.14463 $ & $  $\\
$ 55480.69238 $ & $   0.00508 $ & $   0.00080 $ & $   9.14330 $ & $  $\\
$ 55480.69272 $ & $   0.00901 $ & $   0.00080 $ & $   9.14732 $ & $  $\\
$ 55480.69304 $ & $   0.00596 $ & $   0.00080 $ & $   9.14380 $ & $  $\\
$ 55480.69338 $ & $   0.00718 $ & $   0.00080 $ & $   9.14498 $ & $  $\\
$ 55480.69372 $ & $   0.00676 $ & $   0.00080 $ & $   9.14522 $ & $  $\\
$ 55480.69406 $ & $   0.00733 $ & $   0.00080 $ & $   9.14566 $ & $  $\\
$ 55480.69438 $ & $   0.00937 $ & $   0.00080 $ & $   9.14763 $ & $  $\\
$ 55480.69473 $ & $   0.00566 $ & $   0.00080 $ & $   9.14423 $ & $  $\\
$ 55480.69511 $ & $   0.00480 $ & $   0.00080 $ & $   9.14292 $ & $  $\\
$ 55480.69550 $ & $   0.00903 $ & $   0.00080 $ & $   9.14723 $ & $  $\\
$ 55480.69588 $ & $   0.01011 $ & $   0.00080 $ & $   9.14828 $ & $  $\\
$ 55480.69625 $ & $   0.00507 $ & $   0.00080 $ & $   9.14322 $ & $  $\\
$ 55480.69660 $ & $   0.00929 $ & $   0.00080 $ & $   9.14736 $ & $  $\\
$ 55480.69694 $ & $   0.00721 $ & $   0.00080 $ & $   9.14544 $ & $  $\\
$ 55480.69724 $ & $   0.00661 $ & $   0.00080 $ & $   9.14515 $ & $  $\\
$ 55480.69758 $ & $   0.00550 $ & $   0.00081 $ & $   9.14474 $ & $  $\\
$ 55480.69791 $ & $   0.00865 $ & $   0.00081 $ & $   9.14828 $ & $  $\\
$ 55480.69825 $ & $   0.01033 $ & $   0.00081 $ & $   9.15006 $ & $  $\\
$ 55480.69859 $ & $   0.00806 $ & $   0.00081 $ & $   9.14788 $ & $  $\\
$ 55480.69890 $ & $   0.00803 $ & $   0.00081 $ & $   9.14667 $ & $  $\\
$ 55480.69925 $ & $   0.00631 $ & $   0.00080 $ & $   9.14454 $ & $  $\\
$ 55480.69957 $ & $   0.00553 $ & $   0.00080 $ & $   9.14360 $ & $  $\\
$ 55480.69989 $ & $   0.00780 $ & $   0.00080 $ & $   9.14607 $ & $  $\\
$ 55480.70022 $ & $   0.00748 $ & $   0.00080 $ & $   9.14567 $ & $  $\\
$ 55480.70054 $ & $   0.00936 $ & $   0.00080 $ & $   9.14714 $ & $  $\\
$ 55480.70089 $ & $   0.00792 $ & $   0.00080 $ & $   9.14668 $ & $  $\\
$ 55480.70122 $ & $   0.00768 $ & $   0.00080 $ & $   9.14607 $ & $  $\\
$ 55480.70154 $ & $   0.00575 $ & $   0.00080 $ & $   9.14395 $ & $  $\\
$ 55480.70187 $ & $   0.00835 $ & $   0.00081 $ & $   9.14714 $ & $  $\\
$ 55480.70220 $ & $   0.00838 $ & $   0.00081 $ & $   9.14695 $ & $  $\\
$ 55480.70253 $ & $   0.00786 $ & $   0.00081 $ & $   9.14645 $ & $  $\\
$ 55480.70286 $ & $   0.00728 $ & $   0.00080 $ & $   9.14574 $ & $  $\\
$ 55480.70319 $ & $   0.00607 $ & $   0.00081 $ & $   9.14528 $ & $  $\\
$ 55480.70352 $ & $   0.00558 $ & $   0.00081 $ & $   9.14456 $ & $  $\\
$ 55480.70385 $ & $   0.00940 $ & $   0.00081 $ & $   9.14756 $ & $  $\\
$ 55480.70419 $ & $   0.00515 $ & $   0.00080 $ & $   9.14334 $ & $  $\\
$ 55480.70452 $ & $   0.00795 $ & $   0.00080 $ & $   9.14588 $ & $  $\\
$ 55480.70485 $ & $   0.00761 $ & $   0.00080 $ & $   9.14572 $ & $  $\\
$ 55480.70518 $ & $   0.00599 $ & $   0.00080 $ & $   9.14406 $ & $  $\\
$ 55480.70552 $ & $   0.00614 $ & $   0.00080 $ & $   9.14471 $ & $  $\\
$ 55480.70584 $ & $   0.00814 $ & $   0.00081 $ & $   9.14637 $ & $  $\\
$ 55480.70619 $ & $   0.00714 $ & $   0.00080 $ & $   9.14572 $ & $  $\\
$ 55480.70651 $ & $   0.00861 $ & $   0.00080 $ & $   9.14688 $ & $  $\\
$ 55480.70685 $ & $   0.00674 $ & $   0.00080 $ & $   9.14541 $ & $  $\\
$ 55480.70717 $ & $   0.00549 $ & $   0.00080 $ & $   9.14401 $ & $  $\\
$ 55480.70752 $ & $   0.00765 $ & $   0.00080 $ & $   9.14567 $ & $  $\\
$ 55480.70784 $ & $   0.00887 $ & $   0.00080 $ & $   9.14690 $ & $  $\\
$ 55480.70817 $ & $   0.00915 $ & $   0.00081 $ & $   9.14786 $ & $  $\\
$ 55480.70852 $ & $   0.00401 $ & $   0.00080 $ & $   9.14307 $ & $  $\\
$ 55480.70884 $ & $   0.01033 $ & $   0.00081 $ & $   9.14837 $ & $  $\\
$ 55480.70916 $ & $   0.00700 $ & $   0.00080 $ & $   9.14553 $ & $  $\\
$ 55480.70950 $ & $   0.00965 $ & $   0.00080 $ & $   9.14821 $ & $  $\\
$ 55480.70982 $ & $   0.00701 $ & $   0.00081 $ & $   9.14581 $ & $  $\\
$ 55480.71016 $ & $   0.00736 $ & $   0.00081 $ & $   9.14536 $ & $  $\\
$ 55480.71047 $ & $   0.00642 $ & $   0.00081 $ & $   9.14483 $ & $  $\\
$ 55480.71081 $ & $   0.00511 $ & $   0.00080 $ & $   9.14333 $ & $  $\\
$ 55480.71115 $ & $   0.00618 $ & $   0.00080 $ & $   9.14492 $ & $  $\\
$ 55480.71148 $ & $   0.00853 $ & $   0.00081 $ & $   9.14680 $ & $  $\\
$ 55480.71181 $ & $   0.00585 $ & $   0.00080 $ & $   9.14443 $ & $  $\\
$ 55480.71215 $ & $   0.00665 $ & $   0.00080 $ & $   9.14531 $ & $  $\\
$ 55480.71247 $ & $   0.00812 $ & $   0.00081 $ & $   9.14643 $ & $  $\\
$ 55480.71280 $ & $   0.00799 $ & $   0.00081 $ & $   9.14649 $ & $  $\\
$ 55480.71312 $ & $   0.00734 $ & $   0.00080 $ & $   9.14590 $ & $  $\\
$ 55480.71346 $ & $   0.00735 $ & $   0.00080 $ & $   9.14558 $ & $  $\\
$ 55480.71379 $ & $   0.00901 $ & $   0.00080 $ & $   9.14702 $ & $  $\\
$ 55480.71413 $ & $   0.00603 $ & $   0.00080 $ & $   9.14466 $ & $  $\\
$ 55480.71446 $ & $   0.01008 $ & $   0.00081 $ & $   9.14887 $ & $  $\\
$ 55480.71479 $ & $   0.01034 $ & $   0.00081 $ & $   9.14911 $ & $  $\\
$ 55480.71511 $ & $   0.00501 $ & $   0.00081 $ & $   9.14366 $ & $  $\\
$ 55480.71544 $ & $   0.00398 $ & $   0.00081 $ & $   9.14217 $ & $  $\\
$ 55480.71578 $ & $   0.00833 $ & $   0.00081 $ & $   9.14657 $ & $  $\\
$ 55480.71611 $ & $   0.00619 $ & $   0.00081 $ & $   9.14470 $ & $  $\\
$ 55480.71644 $ & $   0.00574 $ & $   0.00081 $ & $   9.14449 $ & $  $\\
$ 55480.71678 $ & $   0.00654 $ & $   0.00081 $ & $   9.14500 $ & $  $\\
$ 55480.71709 $ & $   0.00535 $ & $   0.00080 $ & $   9.14335 $ & $  $\\
$ 55480.71744 $ & $   0.00225 $ & $   0.00080 $ & $   9.14133 $ & $  $\\
$ 55480.71776 $ & $   0.00761 $ & $   0.00081 $ & $   9.14558 $ & $  $\\
$ 55480.71811 $ & $   0.01000 $ & $   0.00081 $ & $   9.14859 $ & $  $\\
$ 55480.71845 $ & $   0.00527 $ & $   0.00081 $ & $   9.14315 $ & $  $\\
$ 55480.71878 $ & $   0.00862 $ & $   0.00081 $ & $   9.14800 $ & $  $\\
$ 55480.71909 $ & $   0.00571 $ & $   0.00081 $ & $   9.14424 $ & $  $\\
$ 55480.71943 $ & $   0.00761 $ & $   0.00081 $ & $   9.14618 $ & $  $\\
$ 55480.71976 $ & $   0.00670 $ & $   0.00081 $ & $   9.14588 $ & $  $\\
$ 55480.72009 $ & $   0.00922 $ & $   0.00081 $ & $   9.14815 $ & $  $\\
$ 55480.72044 $ & $   0.00764 $ & $   0.00080 $ & $   9.14591 $ & $  $\\
$ 55480.72076 $ & $   0.00858 $ & $   0.00081 $ & $   9.14726 $ & $  $\\
$ 55480.72111 $ & $   0.00757 $ & $   0.00081 $ & $   9.14699 $ & $  $\\
$ 55480.72143 $ & $   0.00593 $ & $   0.00081 $ & $   9.14481 $ & $  $\\
$ 55480.72177 $ & $   0.00523 $ & $   0.00081 $ & $   9.14402 $ & $  $\\
$ 55480.72209 $ & $   0.00534 $ & $   0.00081 $ & $   9.14418 $ & $  $\\
$ 55480.72243 $ & $   0.00617 $ & $   0.00081 $ & $   9.14476 $ & $  $\\
$ 55480.72274 $ & $   0.00607 $ & $   0.00081 $ & $   9.14497 $ & $  $\\
$ 55480.72309 $ & $   0.01024 $ & $   0.00081 $ & $   9.14844 $ & $  $\\
$ 55480.72341 $ & $   0.00490 $ & $   0.00081 $ & $   9.14441 $ & $  $\\
$ 55480.72375 $ & $   0.00870 $ & $   0.00081 $ & $   9.14670 $ & $  $\\
$ 55480.72405 $ & $   0.00658 $ & $   0.00081 $ & $   9.14497 $ & $  $\\
$ 55480.72438 $ & $   0.00625 $ & $   0.00081 $ & $   9.14531 $ & $  $\\
$ 55480.72473 $ & $   0.00645 $ & $   0.00081 $ & $   9.14521 $ & $  $\\
$ 55480.72504 $ & $   0.00617 $ & $   0.00081 $ & $   9.14495 $ & $  $\\
$ 55480.72540 $ & $   0.00600 $ & $   0.00081 $ & $   9.14433 $ & $  $\\
$ 55480.72571 $ & $   0.00501 $ & $   0.00081 $ & $   9.14419 $ & $  $\\
$ 55480.72604 $ & $   0.00326 $ & $   0.00081 $ & $   9.14172 $ & $  $\\
$ 55480.72638 $ & $   0.00569 $ & $   0.00081 $ & $   9.14463 $ & $  $\\
$ 55480.72679 $ & $   0.00611 $ & $   0.00081 $ & $   9.14520 $ & $  $\\
$ 55480.72720 $ & $   0.00973 $ & $   0.00081 $ & $   9.14797 $ & $  $\\
$ 55480.72759 $ & $   0.00949 $ & $   0.00081 $ & $   9.14911 $ & $  $\\
$ 55480.72796 $ & $   0.00588 $ & $   0.00081 $ & $   9.14481 $ & $  $\\
$ 55480.72831 $ & $   0.00707 $ & $   0.00081 $ & $   9.14578 $ & $  $\\
$ 55480.72864 $ & $   0.00805 $ & $   0.00081 $ & $   9.14730 $ & $  $\\
$ 55480.72895 $ & $   0.00671 $ & $   0.00081 $ & $   9.14577 $ & $  $\\
$ 55480.72934 $ & $   0.00422 $ & $   0.00081 $ & $   9.14344 $ & $  $\\
$ 55480.72972 $ & $   0.00370 $ & $   0.00081 $ & $   9.14234 $ & $  $\\
$ 55480.73008 $ & $   0.00424 $ & $   0.00081 $ & $   9.14424 $ & $  $\\
$ 55480.73045 $ & $   0.01015 $ & $   0.00081 $ & $   9.14917 $ & $  $\\
$ 55480.73082 $ & $   0.00680 $ & $   0.00081 $ & $   9.14503 $ & $  $\\
$ 55480.73121 $ & $   0.00708 $ & $   0.00081 $ & $   9.14600 $ & $  $\\
$ 55480.73158 $ & $   0.00387 $ & $   0.00081 $ & $   9.14255 $ & $  $\\
$ 55480.73196 $ & $   0.00888 $ & $   0.00081 $ & $   9.14796 $ & $  $\\
$ 55480.73233 $ & $   0.00659 $ & $   0.00081 $ & $   9.14561 $ & $  $\\
$ 55480.73273 $ & $   0.00675 $ & $   0.00081 $ & $   9.14503 $ & $  $\\
$ 55480.73311 $ & $   0.00308 $ & $   0.00081 $ & $   9.14144 $ & $  $\\
$ 55480.73349 $ & $   0.00154 $ & $   0.00081 $ & $   9.14092 $ & $  $\\
$ 55480.73387 $ & $   0.00526 $ & $   0.00081 $ & $   9.14379 $ & $  $\\
$ 55480.73425 $ & $   0.00813 $ & $   0.00081 $ & $   9.14728 $ & $  $\\
$ 55480.73462 $ & $   0.00328 $ & $   0.00081 $ & $   9.14226 $ & $  $\\
$ 55480.73502 $ & $   0.00029 $ & $   0.00080 $ & $   9.13906 $ & $  $\\
$ 55480.73539 $ & $   0.00090 $ & $   0.00081 $ & $   9.13981 $ & $  $\\
$ 55480.73578 $ & $   0.00515 $ & $   0.00081 $ & $   9.14400 $ & $  $\\
$ 55480.73615 $ & $   0.00240 $ & $   0.00081 $ & $   9.14159 $ & $  $\\
$ 55480.73655 $ & $   0.00205 $ & $   0.00081 $ & $   9.14090 $ & $  $\\
$ 55480.73693 $ & $   0.00307 $ & $   0.00081 $ & $   9.14296 $ & $  $\\
$ 55480.73731 $ & $   0.00403 $ & $   0.00081 $ & $   9.14343 $ & $  $\\
$ 55480.73767 $ & $   0.00065 $ & $   0.00081 $ & $   9.13991 $ & $  $\\
$ 55480.73804 $ & $  -0.00094 $ & $   0.00081 $ & $   9.13818 $ & $  $\\
$ 55480.73842 $ & $  -0.00092 $ & $   0.00081 $ & $   9.13745 $ & $  $\\
$ 55480.73881 $ & $  -0.00115 $ & $   0.00081 $ & $   9.13820 $ & $  $\\
$ 55480.73920 $ & $   0.00046 $ & $   0.00081 $ & $   9.13962 $ & $  $\\
$ 55480.73957 $ & $   0.00241 $ & $   0.00081 $ & $   9.14123 $ & $  $\\
$ 55480.73995 $ & $  -0.00078 $ & $   0.00081 $ & $   9.13798 $ & $  $\\
$ 55480.74033 $ & $   0.00380 $ & $   0.00081 $ & $   9.14189 $ & $  $\\
$ 55480.74070 $ & $  -0.00232 $ & $   0.00081 $ & $   9.13673 $ & $  $\\
$ 55480.74107 $ & $   0.00191 $ & $   0.00081 $ & $   9.14077 $ & $  $\\
$ 55480.74141 $ & $   0.00041 $ & $   0.00081 $ & $   9.13952 $ & $  $\\
$ 55480.74208 $ & $   0.00469 $ & $   0.00081 $ & $   9.14422 $ & $  $\\
$ 55480.74241 $ & $  -0.00001 $ & $   0.00081 $ & $   9.14055 $ & $  $\\
$ 55480.74276 $ & $  -0.00332 $ & $   0.00081 $ & $   9.13702 $ & $  $\\
$ 55480.74307 $ & $   0.00381 $ & $   0.00081 $ & $   9.14389 $ & $  $\\
$ 55480.74341 $ & $  -0.00138 $ & $   0.00081 $ & $   9.13782 $ & $  $\\
$ 55480.74376 $ & $  -0.00326 $ & $   0.00081 $ & $   9.13583 $ & $  $\\
$ 55480.74414 $ & $  -0.00329 $ & $   0.00081 $ & $   9.13530 $ & $  $\\
$ 55480.74452 $ & $  -0.00348 $ & $   0.00081 $ & $   9.13531 $ & $  $\\
$ 55480.74481 $ & $   0.00306 $ & $   0.00081 $ & $   9.14201 $ & $  $\\
$ 55480.74516 $ & $  -0.00165 $ & $   0.00081 $ & $   9.13742 $ & $  $\\
$ 55480.74548 $ & $  -0.00150 $ & $   0.00081 $ & $   9.13711 $ & $  $\\
$ 55480.74580 $ & $   0.00088 $ & $   0.00081 $ & $   9.13995 $ & $  $\\
$ 55480.74613 $ & $   0.00199 $ & $   0.00081 $ & $   9.14173 $ & $  $\\
$ 55480.74678 $ & $   0.00193 $ & $   0.00081 $ & $   9.14166 $ & $  $\\
$ 55480.74710 $ & $  -0.00128 $ & $   0.00081 $ & $   9.13855 $ & $  $\\
$ 55480.74742 $ & $  -0.00076 $ & $   0.00082 $ & $   9.14022 $ & $  $\\
$ 55480.74777 $ & $   0.00176 $ & $   0.00081 $ & $   9.14104 $ & $  $\\
$ 55480.74812 $ & $   0.00047 $ & $   0.00081 $ & $   9.13981 $ & $  $\\
$ 55480.74845 $ & $   0.00359 $ & $   0.00082 $ & $   9.14420 $ & $  $\\
$ 55480.74878 $ & $   0.00158 $ & $   0.00081 $ & $   9.13967 $ & $  $\\
$ 55480.74911 $ & $   0.00027 $ & $   0.00081 $ & $   9.13889 $ & $  $\\
$ 55480.74943 $ & $   0.00329 $ & $   0.00081 $ & $   9.14218 $ & $  $\\
$ 55480.74975 $ & $   0.00223 $ & $   0.00081 $ & $   9.14090 $ & $  $\\
$ 55480.75009 $ & $   0.00098 $ & $   0.00081 $ & $   9.13916 $ & $  $\\
$ 55480.75042 $ & $   0.00261 $ & $   0.00081 $ & $   9.14153 $ & $  $\\
$ 55480.75111 $ & $  -0.00190 $ & $   0.00081 $ & $   9.13685 $ & $  $\\
$ 55480.75142 $ & $  -0.00076 $ & $   0.00081 $ & $   9.13799 $ & $  $\\
$ 55480.75175 $ & $   0.00302 $ & $   0.00081 $ & $   9.14145 $ & $  $\\
$ 55480.75208 $ & $   0.00213 $ & $   0.00081 $ & $   9.14087 $ & $  $\\
$ 55480.75241 $ & $  -0.00160 $ & $   0.00081 $ & $   9.13737 $ & $  $\\
$ 55480.75275 $ & $   0.00147 $ & $   0.00081 $ & $   9.14067 $ & $  $\\
$ 55480.75310 $ & $  -0.00153 $ & $   0.00081 $ & $   9.13747 $ & $  $\\
$ 55480.75342 $ & $  -0.00108 $ & $   0.00082 $ & $   9.13866 $ & $  $\\
$ 55480.75409 $ & $  -0.00421 $ & $   0.00081 $ & $   9.13510 $ & $  $\\
$ 55480.75442 $ & $  -0.00352 $ & $   0.00081 $ & $   9.13514 $ & $  $\\
$ 55480.75475 $ & $  -0.00509 $ & $   0.00081 $ & $   9.13372 $ & $  $\\
$ 55480.75509 $ & $   0.00284 $ & $   0.00081 $ & $   9.14191 $ & $  $\\
$ 55480.75541 $ & $   0.00132 $ & $   0.00081 $ & $   9.14081 $ & $  $\\
$ 55480.75609 $ & $  -0.00162 $ & $   0.00081 $ & $   9.13689 $ & $  $\\
$ 55480.75643 $ & $  -0.00057 $ & $   0.00081 $ & $   9.13804 $ & $  $\\
$ 55480.75674 $ & $  -0.00047 $ & $   0.00081 $ & $   9.13822 $ & $  $\\
$ 55480.75709 $ & $   0.00286 $ & $   0.00081 $ & $   9.14120 $ & $  $\\
$ 55480.75741 $ & $  -0.00128 $ & $   0.00081 $ & $   9.13756 $ & $  $\\
$ 55480.75774 $ & $   0.00370 $ & $   0.00081 $ & $   9.14244 $ & $  $\\
$ 55480.75808 $ & $  -0.00242 $ & $   0.00081 $ & $   9.13602 $ & $  $\\
$ 55480.75844 $ & $   0.00421 $ & $   0.00081 $ & $   9.14231 $ & $  $\\
$ 55480.75878 $ & $   0.00007 $ & $   0.00081 $ & $   9.13878 $ & $  $\\
$ 55480.75910 $ & $  -0.00146 $ & $   0.00081 $ & $   9.13640 $ & $  $\\
$ 55480.75943 $ & $  -0.00295 $ & $   0.00081 $ & $   9.13524 $ & $  $\\
$ 55480.75977 $ & $  -0.00230 $ & $   0.00081 $ & $   9.13626 $ & $  $\\
$ 55480.76009 $ & $   0.00455 $ & $   0.00081 $ & $   9.14333 $ & $  $\\
$ 55480.76043 $ & $   0.00269 $ & $   0.00081 $ & $   9.14192 $ & $  $\\
$ 55480.76076 $ & $   0.00042 $ & $   0.00081 $ & $   9.13900 $ & $  $\\
$ 55480.76110 $ & $   0.00150 $ & $   0.00081 $ & $   9.14006 $ & $  $\\
$ 55480.76187 $ & $   0.00204 $ & $   0.00081 $ & $   9.14067 $ & $  $\\
$ 55480.76225 $ & $   0.00226 $ & $   0.00081 $ & $   9.14072 $ & $  $\\
$ 55480.76263 $ & $   0.00019 $ & $   0.00081 $ & $   9.13860 $ & $  $\\
$ 55480.76301 $ & $   0.00202 $ & $   0.00081 $ & $   9.14132 $ & $  $\\
$ 55480.76334 $ & $  -0.00395 $ & $   0.00081 $ & $   9.13451 $ & $  $\\
$ 55480.76370 $ & $  -0.00066 $ & $   0.00081 $ & $   9.13855 $ & $  $\\
$ 55480.76408 $ & $  -0.00342 $ & $   0.00081 $ & $   9.13472 $ & $  $\\
$ 55480.76447 $ & $   0.00396 $ & $   0.00081 $ & $   9.14222 $ & $  $\\
$ 55480.76485 $ & $   0.00018 $ & $   0.00081 $ & $   9.13867 $ & $  $\\
$ 55480.76524 $ & $   0.00006 $ & $   0.00081 $ & $   9.13857 $ & $  $\\
$ 55480.76561 $ & $  -0.00153 $ & $   0.00081 $ & $   9.13635 $ & $  $\\
$ 55480.76599 $ & $   0.00016 $ & $   0.00081 $ & $   9.13890 $ & $  $\\
$ 55480.76636 $ & $  -0.00159 $ & $   0.00081 $ & $   9.13725 $ & $  $\\
$ 55480.76669 $ & $   0.00214 $ & $   0.00081 $ & $   9.14047 $ & $  $\\
$ 55480.76703 $ & $   0.00209 $ & $   0.00081 $ & $   9.14055 $ & $  $\\
$ 55480.76738 $ & $   0.00131 $ & $   0.00081 $ & $   9.14027 $ & $  $\\
$ 55480.76771 $ & $  -0.00296 $ & $   0.00081 $ & $   9.13443 $ & $  $\\
$ 55480.76804 $ & $  -0.00215 $ & $   0.00081 $ & $   9.13703 $ & $  $\\
$ 55480.76837 $ & $  -0.00090 $ & $   0.00081 $ & $   9.13812 $ & $  $\\
$ 55480.76904 $ & $   0.00194 $ & $   0.00081 $ & $   9.14114 $ & $  $\\
$ 55480.76938 $ & $   0.00353 $ & $   0.00082 $ & $   9.14259 $ & $  $\\
$ 55480.76969 $ & $  -0.00425 $ & $   0.00081 $ & $   9.13455 $ & $  $\\
$ 55480.77004 $ & $   0.00007 $ & $   0.00082 $ & $   9.13976 $ & $  $\\
$ 55480.77037 $ & $  -0.00362 $ & $   0.00081 $ & $   9.13572 $ & $  $\\
$ 55480.77070 $ & $  -0.00023 $ & $   0.00082 $ & $   9.13863 $ & $  $\\
$ 55480.77102 $ & $  -0.00062 $ & $   0.00081 $ & $   9.13725 $ & $  $\\
$ 55480.77136 $ & $  -0.00270 $ & $   0.00081 $ & $   9.13586 $ & $  $\\
$ 55480.77169 $ & $  -0.00167 $ & $   0.00082 $ & $   9.13725 $ & $  $\\
$ 55480.77203 $ & $  -0.00164 $ & $   0.00081 $ & $   9.13758 $ & $  $\\
$ 55480.77235 $ & $   0.00253 $ & $   0.00082 $ & $   9.14163 $ & $  $\\


==> data/HTR340-006_phfu_tab_short.tex <==
$ 55338.79359 $ & $   0.00011 $ & $   0.00080 $ & $  10.12720 $ & $ i$\\
$ 55338.79427 $ & $  -0.00108 $ & $   0.00080 $ & $  10.12640 $ & $ i$\\
$ 55338.79494 $ & $   0.00263 $ & $   0.00080 $ & $  10.12910 $ & $ i$\\
$ 55338.79563 $ & $  -0.00041 $ & $   0.00080 $ & $  10.12660 $ & $ i$\\
$ 55338.79633 $ & $   0.00158 $ & $   0.00080 $ & $  10.12850 $ & $ i$\\
$ 55338.79701 $ & $   0.00036 $ & $   0.00079 $ & $  10.12720 $ & $ i$\\
$ 55338.79769 $ & $  -0.00243 $ & $   0.00079 $ & $  10.12440 $ & $ i$\\
$ 55338.79837 $ & $  -0.00305 $ & $   0.00079 $ & $  10.12340 $ & $ i$\\
$ 55338.79905 $ & $   0.00184 $ & $   0.00079 $ & $  10.12940 $ & $ i$\\
$ 55338.79969 $ & $   0.00187 $ & $   0.00079 $ & $  10.12900 $ & $ i$\\


==> data/HTR340-006_rvtable.old.tex <==
$ 1339.92722 $ & $  -126.48 $ & $    50.92 $ & \nodata      & \nodata      & \nodata      & $   0.188 $ & Subaru \\
$ 1339.93516 $ & $  -169.23 $ & $    57.36 $ & \nodata      & \nodata      & \nodata      & $   0.190 $ & Subaru \\
$ 1339.94290 $ & $  -171.93 $ & $    44.53 $ & \nodata      & \nodata      & \nodata      & $   0.191 $ & Subaru \\
$ 1341.11630 $ & $  -214.92 $ & $    47.11 $ & \nodata      & \nodata      & \nodata      & $   0.406 $ & Subaru \\
$ 1341.12058 $ & $  -172.99 $ & $    47.32 $ & \nodata      & \nodata      & \nodata      & $   0.407 $ & Subaru \\
$ 1341.12485 $ & $  -161.36 $ & $    43.00 $ & \nodata      & \nodata      & \nodata      & $   0.408 $ & Subaru \\
$ 1374.12069 $ & $  -183.38 $ & $    11.37 $ & $    -2.85 $ & $     6.57 $ & $    0.1760 $ & $   0.459 $ & Keck \\
$ 1374.85735 $ & \nodata      & \nodata      & $    -9.20 $ & $     4.18 $ & $    0.1730 $ & $   0.594 $ & Keck \\
$ 1374.86800 $ & $   -67.58 $ & $    11.89 $ & $   -25.52 $ & $     9.34 $ & $    0.1760 $ & $   0.596 $ & Keck \\
$ 1375.95203 $ & $   298.62 $ & $    10.24 $ & $   -15.73 $ & $     4.46 $ & $    0.1780 $ & $   0.795 $ & Keck \\
$ 1378.12823 $ & $  -252.97 $ & $    12.71 $ & $   -13.52 $ & $     7.86 $ & $    0.1740 $ & $   0.194 $ & Keck \\
$ 1379.07458 $ & $  -214.25 $ & $    12.73 $ & $   -10.85 $ & $     3.72 $ & $    0.1760 $ & $   0.368 $ & Keck \\
$ 1379.56536 $ & $  -142.37 $ & $    61.60 $ & \nodata      & \nodata      & \nodata      & $   0.458 $ & FIES \\
$ 1380.13344 $ & $  -124.08 $ & $    13.51 $ & $    60.87 $ & $    20.44 $ & $    0.1800 $ & $   0.562 $ & Keck \\
$ 1380.49378 $ & $    23.56 $ & $    58.70 $ & \nodata      & \nodata      & \nodata      & $   0.628 $ & FIES \\
$ 1381.11125 $ & $   122.44 $ & $    14.71 $ & $    -9.04 $ & $    12.64 $ & $    0.1750 $ & $   0.741 $ & Keck \\
$ 1381.55600 $ & $   289.45 $ & $    46.50 $ & \nodata      & \nodata      & \nodata      & $   0.823 $ & FIES \\
$ 1383.47949 $ & $   -89.26 $ & $    56.00 $ & \nodata      & \nodata      & \nodata      & $   0.175 $ & FIES \\
$ 1384.48968 $ & $  -154.52 $ & $    50.60 $ & \nodata      & \nodata      & \nodata      & $   0.361 $ & FIES \\
$ 1400.85414 $ & $  -134.48 $ & $    15.43 $ & $    27.38 $ & $     7.53 $ & $    0.1670 $ & $   0.362 $ & Keck \\
$ 1403.82567 $ & $   503.82 $ & $    15.18 $ & $    38.35 $ & $     6.14 $ & $    0.1730 $ & $   0.907 $ & Keck \\
$ 1404.83902 $ & $    10.81 $ & $    14.05 $ & $     0.79 $ & $     7.25 $ & $    0.1740 $ & $   0.093 $ & Keck \\
$ 1415.04513 $ & $   314.29 $ & $    14.03 $ & $     2.76 $ & $     8.29 $ & $    0.1680 $ & $   0.965 $ & Keck \\
$ 1423.66787 $ & $  -105.00 $ & $    78.50 $ & \nodata      & \nodata      & \nodata      & $   0.546 $ & FIES \\
$ 1424.64318 $ & $    51.88 $ & $   139.40 $ & \nodata      & \nodata      & \nodata      & $   0.725 $ & FIES \\
$ 1425.57489 $ & $   484.91 $ & $    48.70 $ & \nodata      & \nodata      & \nodata      & $   0.896 $ & FIES \\
$ 1426.64513 $ & $  -144.21 $ & $    57.60 $ & \nodata      & \nodata      & \nodata      & $   0.092 $ & FIES \\
$ 1464.85484 $ & $  -105.90 $ & $    15.03 $ & $   -11.41 $ & $    11.10 $ & $    0.1640 $ & $   0.099 $ & Keck \\
$ 1465.94874 $ & $  -256.10 $ & $    13.70 $ & $   -19.33 $ & $     6.92 $ & $    0.1630 $ & $   0.300 $ & Keck \\
$ 1467.71998 $ & $    -6.16 $ & $    13.61 $ & $   -12.70 $ & $     8.00 $ & $    0.1640 $ & $   0.625 $ & Keck \\


==> data/HTR340-006_rvtable.tex <==
$ 1339.92722 $ & $  -158.62 $ & $    50.92 $ & \nodata      & \nodata      & \nodata      & $   0.188 $ & Subaru \\
$ 1339.93516 $ & $  -201.37 $ & $    57.36 $ & \nodata      & \nodata      & \nodata      & $   0.190 $ & Subaru \\
$ 1339.94290 $ & $  -204.06 $ & $    44.53 $ & \nodata      & \nodata      & \nodata      & $   0.191 $ & Subaru \\
$ 1341.11630 $ & $  -246.80 $ & $    47.11 $ & \nodata      & \nodata      & \nodata      & $   0.406 $ & Subaru \\
$ 1341.12058 $ & $  -204.87 $ & $    47.32 $ & \nodata      & \nodata      & \nodata      & $   0.407 $ & Subaru \\
$ 1341.12485 $ & $  -193.24 $ & $    43.00 $ & \nodata      & \nodata      & \nodata      & $   0.408 $ & Subaru \\
$ 1374.12069 $ & $  -196.46 $ & $    11.37 $ & $    -2.85 $ & $     6.57 $ & $    0.176 $ & $   0.459 $ & Keck \\
$ 1374.85735 $ & \nodata      & \nodata      & $    -9.20 $ & $     4.18 $ & $    0.173 $ & $   0.594 $ & Keck \\
$ 1374.86800 $ & $   -80.49 $ & $    11.89 $ & $   -25.52 $ & $     9.34 $ & $    0.176 $ & $   0.596 $ & Keck \\
$ 1375.95203 $ & $   285.94 $ & $    10.24 $ & $   -15.73 $ & $     4.46 $ & $    0.178 $ & $   0.795 $ & Keck \\
$ 1378.12823 $ & $  -265.18 $ & $    12.71 $ & $   -13.52 $ & $     7.86 $ & $    0.174 $ & $   0.194 $ & Keck \\
$ 1379.07458 $ & $  -226.26 $ & $    12.73 $ & $   -10.85 $ & $     3.72 $ & $    0.176 $ & $   0.368 $ & Keck \\
$ 1379.56536 $ & $  -162.68 $ & $    61.60 $ & \nodata      & \nodata      & \nodata      & $   0.458 $ & FIES \\
$ 1380.13344 $ & $  -135.85 $ & $    13.51 $ & $    60.87 $ & $    20.44 $ & $    0.180 $ & $   0.562 $ & Keck \\
$ 1380.49378 $ & $     3.45 $ & $    58.70 $ & \nodata      & \nodata      & \nodata      & $   0.628 $ & FIES \\
$ 1381.11125 $ & $   110.87 $ & $    14.71 $ & $    -9.04 $ & $    12.64 $ & $    0.175 $ & $   0.741 $ & Keck \\
$ 1381.55600 $ & $   269.57 $ & $    46.50 $ & \nodata      & \nodata      & \nodata      & $   0.823 $ & FIES \\
$ 1383.47949 $ & $  -108.72 $ & $    56.00 $ & \nodata      & \nodata      & \nodata      & $   0.176 $ & FIES \\
$ 1384.48968 $ & $  -173.76 $ & $    50.60 $ & \nodata      & \nodata      & \nodata      & $   0.361 $ & FIES \\
$ 1400.85414 $ & $  -141.78 $ & $    15.43 $ & $    27.38 $ & $     7.53 $ & $    0.167 $ & $   0.362 $ & Keck \\
$ 1403.82567 $ & $   497.16 $ & $    15.18 $ & $    38.35 $ & $     6.14 $ & $    0.173 $ & $   0.907 $ & Keck \\
$ 1404.83902 $ & $     4.37 $ & $    14.05 $ & $     0.79 $ & $     7.25 $ & $    0.174 $ & $   0.093 $ & Keck \\
$ 1415.04513 $ & $   310.06 $ & $    14.03 $ & $     2.76 $ & $     8.29 $ & $    0.168 $ & $   0.965 $ & Keck \\
$ 1423.66787 $ & $  -115.78 $ & $    78.50 $ & \nodata      & \nodata      & \nodata      & $   0.546 $ & FIES \\
$ 1424.64318 $ & $    41.31 $ & $   139.40 $ & \nodata      & \nodata      & \nodata      & $   0.725 $ & FIES \\
$ 1425.57489 $ & $   474.54 $ & $    48.70 $ & \nodata      & \nodata      & \nodata      & $   0.896 $ & FIES \\
$ 1426.64513 $ & $  -154.35 $ & $    57.60 $ & \nodata      & \nodata      & \nodata      & $   0.092 $ & FIES \\
$ 1464.85484 $ & $   -99.38 $ & $    15.03 $ & $   -11.41 $ & $    11.10 $ & $    0.164 $ & $   0.100 $ & Keck \\
$ 1465.94874 $ & $  -249.34 $ & $    13.70 $ & $   -19.33 $ & $     6.92 $ & $    0.163 $ & $   0.300 $ & Keck \\
$ 1467.71998 $ & $     0.98 $ & $    13.61 $ & $   -12.70 $ & $     8.00 $ & $    0.164 $ & $   0.625 $ & Keck \\


==> data/HTR364-003_phfu_tab.tex <==
$ 55578.68612 $ & $   0.00994 $ & $   0.00115 $ & $  11.35390 $ & $ i$\\
$ 55578.68766 $ & $   0.01221 $ & $   0.00104 $ & $  11.35670 $ & $ i$\\
$ 55578.68921 $ & $   0.01203 $ & $   0.00101 $ & $  11.35720 $ & $ i$\\
$ 55578.69075 $ & $   0.00982 $ & $   0.00097 $ & $  11.35550 $ & $ i$\\
$ 55578.69228 $ & $   0.01192 $ & $   0.00099 $ & $  11.35670 $ & $ i$\\
$ 55578.69383 $ & $   0.01272 $ & $   0.00113 $ & $  11.35760 $ & $ i$\\
$ 55578.69504 $ & $   0.01154 $ & $   0.00113 $ & $  11.35620 $ & $ i$\\
$ 55578.69622 $ & $   0.01243 $ & $   0.00115 $ & $  11.35790 $ & $ i$\\
$ 55578.69742 $ & $   0.01048 $ & $   0.00114 $ & $  11.35540 $ & $ i$\\
$ 55578.69863 $ & $   0.00959 $ & $   0.00114 $ & $  11.35430 $ & $ i$\\
$ 55578.69984 $ & $   0.00796 $ & $   0.00114 $ & $  11.35340 $ & $ i$\\
$ 55578.70105 $ & $   0.00997 $ & $   0.00114 $ & $  11.35530 $ & $ i$\\
$ 55578.70227 $ & $   0.01148 $ & $   0.00112 $ & $  11.35660 $ & $ i$\\
$ 55578.70346 $ & $   0.01108 $ & $   0.00112 $ & $  11.35560 $ & $ i$\\
$ 55578.70465 $ & $   0.00957 $ & $   0.00113 $ & $  11.35480 $ & $ i$\\
$ 55578.70585 $ & $   0.00998 $ & $   0.00112 $ & $  11.35550 $ & $ i$\\
$ 55578.70706 $ & $   0.01105 $ & $   0.00112 $ & $  11.35610 $ & $ i$\\
$ 55578.70826 $ & $   0.01143 $ & $   0.00113 $ & $  11.35800 $ & $ i$\\
$ 55578.70947 $ & $   0.01155 $ & $   0.00110 $ & $  11.35670 $ & $ i$\\
$ 55578.71067 $ & $   0.01219 $ & $   0.00110 $ & $  11.35840 $ & $ i$\\
$ 55578.71188 $ & $   0.00561 $ & $   0.00112 $ & $  11.35130 $ & $ i$\\
$ 55578.71308 $ & $   0.01041 $ & $   0.00112 $ & $  11.35660 $ & $ i$\\
$ 55578.71427 $ & $   0.00937 $ & $   0.00111 $ & $  11.35610 $ & $ i$\\
$ 55578.71548 $ & $   0.00790 $ & $   0.00113 $ & $  11.35440 $ & $ i$\\
$ 55578.71670 $ & $   0.01149 $ & $   0.00111 $ & $  11.35740 $ & $ i$\\
$ 55578.71791 $ & $   0.00821 $ & $   0.00108 $ & $  11.35470 $ & $ i$\\
$ 55578.71912 $ & $   0.00850 $ & $   0.00111 $ & $  11.35470 $ & $ i$\\
$ 55578.72031 $ & $   0.01361 $ & $   0.00111 $ & $  11.36010 $ & $ i$\\
$ 55578.72150 $ & $   0.00916 $ & $   0.00113 $ & $  11.35590 $ & $ i$\\
$ 55578.72271 $ & $   0.00923 $ & $   0.00111 $ & $  11.35670 $ & $ i$\\
$ 55578.72392 $ & $   0.01093 $ & $   0.00110 $ & $  11.35760 $ & $ i$\\
$ 55578.72513 $ & $   0.00835 $ & $   0.00111 $ & $  11.35450 $ & $ i$\\
$ 55578.72629 $ & $   0.00447 $ & $   0.00111 $ & $  11.35190 $ & $ i$\\
$ 55578.72749 $ & $   0.00891 $ & $   0.00112 $ & $  11.35580 $ & $ i$\\
$ 55578.72871 $ & $   0.00940 $ & $   0.00112 $ & $  11.35650 $ & $ i$\\
$ 55578.72993 $ & $   0.00819 $ & $   0.00110 $ & $  11.35460 $ & $ i$\\
$ 55578.73111 $ & $   0.00622 $ & $   0.00112 $ & $  11.35330 $ & $ i$\\
$ 55578.73232 $ & $   0.00216 $ & $   0.00107 $ & $  11.34920 $ & $ i$\\
$ 55578.73352 $ & $   0.00614 $ & $   0.00110 $ & $  11.35250 $ & $ i$\\
$ 55578.73473 $ & $   0.00329 $ & $   0.00110 $ & $  11.34980 $ & $ i$\\
$ 55578.73595 $ & $   0.00218 $ & $   0.00110 $ & $  11.34940 $ & $ i$\\
$ 55578.73716 $ & $   0.00159 $ & $   0.00111 $ & $  11.34840 $ & $ i$\\
$ 55578.73837 $ & $   0.00154 $ & $   0.00110 $ & $  11.34810 $ & $ i$\\
$ 55578.73956 $ & $  -0.00239 $ & $   0.00109 $ & $  11.34450 $ & $ i$\\
$ 55578.74076 $ & $   0.00097 $ & $   0.00114 $ & $  11.34830 $ & $ i$\\
$ 55578.74197 $ & $  -0.00071 $ & $   0.00109 $ & $  11.34610 $ & $ i$\\
$ 55578.74317 $ & $   0.00003 $ & $   0.00106 $ & $  11.34620 $ & $ i$\\
$ 55578.74438 $ & $  -0.00228 $ & $   0.00109 $ & $  11.34460 $ & $ i$\\
$ 55578.74559 $ & $  -0.00178 $ & $   0.00109 $ & $  11.34420 $ & $ i$\\
$ 55578.74679 $ & $   0.00225 $ & $   0.00111 $ & $  11.34850 $ & $ i$\\
$ 55578.74801 $ & $  -0.00245 $ & $   0.00110 $ & $  11.34340 $ & $ i$\\
$ 55578.74921 $ & $   0.00231 $ & $   0.00108 $ & $  11.34920 $ & $ i$\\
$ 55578.75041 $ & $   0.00061 $ & $   0.00106 $ & $  11.34760 $ & $ i$\\
$ 55578.75162 $ & $   0.00198 $ & $   0.00107 $ & $  11.34870 $ & $ i$\\
$ 55578.75282 $ & $   0.00125 $ & $   0.00109 $ & $  11.34730 $ & $ i$\\
$ 55578.75403 $ & $  -0.00151 $ & $   0.00109 $ & $  11.34510 $ & $ i$\\
$ 55578.75524 $ & $  -0.00219 $ & $   0.00107 $ & $  11.34400 $ & $ i$\\
$ 55578.75672 $ & $  -0.00031 $ & $   0.00108 $ & $  11.34680 $ & $ i$\\
$ 55578.75794 $ & $   0.00297 $ & $   0.00105 $ & $  11.34990 $ & $ i$\\
$ 55578.75928 $ & $   0.00106 $ & $   0.00108 $ & $  11.34780 $ & $ i$\\
$ 55578.76067 $ & $  -0.00004 $ & $   0.00107 $ & $  11.34700 $ & $ i$\\
$ 55578.76187 $ & $   0.00208 $ & $   0.00109 $ & $  11.34880 $ & $ i$\\
$ 55578.76311 $ & $   0.00000 $ & $   0.00106 $ & $  11.34610 $ & $ i$\\
$ 55578.76430 $ & $   0.00060 $ & $   0.00108 $ & $  11.34770 $ & $ i$\\
$ 55578.76551 $ & $   0.00046 $ & $   0.00109 $ & $  11.34760 $ & $ i$\\
$ 55578.76673 $ & $  -0.00065 $ & $   0.00113 $ & $  11.34600 $ & $ i$\\
$ 55578.76793 $ & $   0.00194 $ & $   0.00112 $ & $  11.34810 $ & $ i$\\
$ 55578.76911 $ & $   0.00098 $ & $   0.00109 $ & $  11.34770 $ & $ i$\\
$ 55578.77030 $ & $   0.00164 $ & $   0.00111 $ & $  11.34800 $ & $ i$\\
$ 55578.77148 $ & $  -0.00205 $ & $   0.00108 $ & $  11.34390 $ & $ i$\\
$ 55578.77270 $ & $  -0.00029 $ & $   0.00109 $ & $  11.34620 $ & $ i$\\
$ 55578.77390 $ & $   0.00123 $ & $   0.00106 $ & $  11.34650 $ & $ i$\\
$ 55578.77507 $ & $   0.00204 $ & $   0.00106 $ & $  11.34820 $ & $ i$\\
$ 55578.77625 $ & $  -0.00013 $ & $   0.00105 $ & $  11.34590 $ & $ i$\\
$ 55578.77745 $ & $   0.00248 $ & $   0.00106 $ & $  11.34850 $ & $ i$\\
$ 55578.77866 $ & $  -0.00098 $ & $   0.00105 $ & $  11.34550 $ & $ i$\\
$ 55578.77985 $ & $   0.00025 $ & $   0.00109 $ & $  11.34570 $ & $ i$\\
$ 55578.78105 $ & $   0.00075 $ & $   0.00111 $ & $  11.34690 $ & $ i$\\
$ 55578.78223 $ & $  -0.00290 $ & $   0.00113 $ & $  11.34310 $ & $ i$\\
$ 55578.78344 $ & $   0.00015 $ & $   0.00111 $ & $  11.34690 $ & $ i$\\
$ 55578.78465 $ & $  -0.00012 $ & $   0.00107 $ & $  11.34630 $ & $ i$\\
$ 55578.78586 $ & $  -0.00087 $ & $   0.00107 $ & $  11.34480 $ & $ i$\\
$ 55578.78701 $ & $   0.00179 $ & $   0.00106 $ & $  11.34770 $ & $ i$\\
$ 55578.78823 $ & $   0.00033 $ & $   0.00103 $ & $  11.34610 $ & $ i$\\
$ 55578.78941 $ & $  -0.00123 $ & $   0.00098 $ & $  11.34450 $ & $ i$\\
$ 55578.79062 $ & $   0.00014 $ & $   0.00097 $ & $  11.34610 $ & $ i$\\
$ 55578.79183 $ & $   0.00063 $ & $   0.00099 $ & $  11.34750 $ & $ i$\\
$ 55578.79304 $ & $  -0.00051 $ & $   0.00097 $ & $  11.34590 $ & $ i$\\
$ 55578.79425 $ & $  -0.00003 $ & $   0.00097 $ & $  11.34620 $ & $ i$\\
$ 55578.79545 $ & $  -0.00132 $ & $   0.00097 $ & $  11.34490 $ & $ i$\\
$ 55578.79665 $ & $  -0.00022 $ & $   0.00096 $ & $  11.34620 $ & $ i$\\
$ 55578.79787 $ & $   0.00237 $ & $   0.00096 $ & $  11.34890 $ & $ i$\\
$ 55578.79908 $ & $  -0.00033 $ & $   0.00097 $ & $  11.34620 $ & $ i$\\
$ 55578.80028 $ & $  -0.00164 $ & $   0.00096 $ & $  11.34470 $ & $ i$\\
$ 55578.80148 $ & $  -0.00224 $ & $   0.00095 $ & $  11.34430 $ & $ i$\\
$ 55578.80267 $ & $  -0.00146 $ & $   0.00095 $ & $  11.34490 $ & $ i$\\
$ 55578.80388 $ & $  -0.00108 $ & $   0.00094 $ & $  11.34500 $ & $ i$\\
$ 55578.80507 $ & $  -0.00211 $ & $   0.00095 $ & $  11.34410 $ & $ i$\\
$ 55578.80627 $ & $  -0.00010 $ & $   0.00096 $ & $  11.34550 $ & $ i$\\
$ 55578.80748 $ & $   0.00229 $ & $   0.00097 $ & $  11.34820 $ & $ i$\\
$ 55578.80869 $ & $  -0.00046 $ & $   0.00097 $ & $  11.34530 $ & $ i$\\
$ 55578.80989 $ & $   0.00017 $ & $   0.00096 $ & $  11.34630 $ & $ i$\\
$ 55578.81110 $ & $  -0.00178 $ & $   0.00096 $ & $  11.34370 $ & $ i$\\
$ 55578.81230 $ & $  -0.00019 $ & $   0.00095 $ & $  11.34520 $ & $ i$\\
$ 55578.81348 $ & $   0.00004 $ & $   0.00096 $ & $  11.34590 $ & $ i$\\
$ 55578.81469 $ & $  -0.00014 $ & $   0.00095 $ & $  11.34550 $ & $ i$\\
$ 55578.81608 $ & $   0.00187 $ & $   0.00094 $ & $  11.34800 $ & $ i$\\
$ 55578.81739 $ & $   0.00206 $ & $   0.00094 $ & $  11.34720 $ & $ i$\\
$ 55578.81875 $ & $   0.00127 $ & $   0.00095 $ & $  11.34630 $ & $ i$\\
$ 55578.81999 $ & $  -0.00096 $ & $   0.00095 $ & $  11.34480 $ & $ i$\\
$ 55585.83194 $ & $   0.00207 $ & $   0.00096 $ & $  10.04880 $ & $ i$\\
$ 55585.83247 $ & $   0.00176 $ & $   0.00097 $ & $  10.04820 $ & $ i$\\
$ 55585.83295 $ & $   0.00284 $ & $   0.00100 $ & $  10.04940 $ & $ i$\\
$ 55585.83344 $ & $  -0.00117 $ & $   0.00100 $ & $  10.04550 $ & $ i$\\
$ 55585.83392 $ & $   0.00126 $ & $   0.00097 $ & $  10.04730 $ & $ i$\\
$ 55585.83443 $ & $  -0.00058 $ & $   0.00099 $ & $  10.04620 $ & $ i$\\
$ 55585.83493 $ & $  -0.00335 $ & $   0.00100 $ & $  10.04270 $ & $ i$\\
$ 55585.83542 $ & $  -0.00306 $ & $   0.00098 $ & $  10.04360 $ & $ i$\\
$ 55585.83592 $ & $  -0.00107 $ & $   0.00100 $ & $  10.04540 $ & $ i$\\
$ 55585.83641 $ & $   0.00057 $ & $   0.00099 $ & $  10.04710 $ & $ i$\\
$ 55585.83689 $ & $  -0.00047 $ & $   0.00097 $ & $  10.04540 $ & $ i$\\
$ 55585.83738 $ & $  -0.00017 $ & $   0.00099 $ & $  10.04640 $ & $ i$\\
$ 55585.83788 $ & $   0.00181 $ & $   0.00096 $ & $  10.04780 $ & $ i$\\
$ 55585.83838 $ & $   0.00344 $ & $   0.00098 $ & $  10.04910 $ & $ i$\\
$ 55585.83888 $ & $  -0.00216 $ & $   0.00100 $ & $  10.04390 $ & $ i$\\
$ 55585.83936 $ & $  -0.00272 $ & $   0.00098 $ & $  10.04310 $ & $ i$\\
$ 55585.83987 $ & $  -0.00269 $ & $   0.00096 $ & $  10.04370 $ & $ i$\\
$ 55585.84036 $ & $  -0.00096 $ & $   0.00097 $ & $  10.04550 $ & $ i$\\
$ 55585.84086 $ & $   0.00029 $ & $   0.00099 $ & $  10.04670 $ & $ i$\\
$ 55585.84134 $ & $   0.00050 $ & $   0.00097 $ & $  10.04650 $ & $ i$\\
$ 55585.84186 $ & $  -0.00127 $ & $   0.00099 $ & $  10.04500 $ & $ i$\\
$ 55585.84235 $ & $   0.00277 $ & $   0.00103 $ & $  10.04970 $ & $ i$\\
$ 55585.84284 $ & $   0.00144 $ & $   0.00099 $ & $  10.04820 $ & $ i$\\
$ 55585.84333 $ & $   0.00011 $ & $   0.00097 $ & $  10.04640 $ & $ i$\\
$ 55585.84383 $ & $  -0.00246 $ & $   0.00095 $ & $  10.04380 $ & $ i$\\
$ 55585.84432 $ & $  -0.00205 $ & $   0.00097 $ & $  10.04410 $ & $ i$\\
$ 55585.84480 $ & $   0.00031 $ & $   0.00098 $ & $  10.04700 $ & $ i$\\
$ 55585.84580 $ & $   0.00348 $ & $   0.00098 $ & $  10.04980 $ & $ i$\\
$ 55585.84630 $ & $   0.00160 $ & $   0.00098 $ & $  10.04800 $ & $ i$\\
$ 55585.84680 $ & $  -0.00131 $ & $   0.00098 $ & $  10.04550 $ & $ i$\\
$ 55585.84731 $ & $   0.00159 $ & $   0.00099 $ & $  10.04820 $ & $ i$\\
$ 55585.84780 $ & $  -0.00078 $ & $   0.00097 $ & $  10.04530 $ & $ i$\\
$ 55585.84829 $ & $  -0.00109 $ & $   0.00098 $ & $  10.04520 $ & $ i$\\
$ 55585.84879 $ & $  -0.00148 $ & $   0.00099 $ & $  10.04480 $ & $ i$\\
$ 55585.84929 $ & $   0.00037 $ & $   0.00097 $ & $  10.04620 $ & $ i$\\
$ 55585.84979 $ & $  -0.00168 $ & $   0.00096 $ & $  10.04530 $ & $ i$\\
$ 55585.85027 $ & $   0.00206 $ & $   0.00097 $ & $  10.04890 $ & $ i$\\
$ 55585.85077 $ & $   0.00163 $ & $   0.00096 $ & $  10.04750 $ & $ i$\\
$ 55585.85126 $ & $  -0.00038 $ & $   0.00099 $ & $  10.04660 $ & $ i$\\
$ 55585.85174 $ & $   0.00064 $ & $   0.00097 $ & $  10.04730 $ & $ i$\\
$ 55585.85223 $ & $  -0.00003 $ & $   0.00095 $ & $  10.04650 $ & $ i$\\
$ 55585.85274 $ & $   0.00235 $ & $   0.00096 $ & $  10.04850 $ & $ i$\\
$ 55585.85323 $ & $   0.00143 $ & $   0.00095 $ & $  10.04810 $ & $ i$\\
$ 55585.85373 $ & $  -0.00452 $ & $   0.00095 $ & $  10.04130 $ & $ i$\\
$ 55585.85421 $ & $   0.00180 $ & $   0.00095 $ & $  10.04850 $ & $ i$\\
$ 55585.85471 $ & $   0.00460 $ & $   0.00095 $ & $  10.05060 $ & $ i$\\
$ 55585.85520 $ & $   0.00081 $ & $   0.00097 $ & $  10.04670 $ & $ i$\\
$ 55585.85570 $ & $   0.00006 $ & $   0.00095 $ & $  10.04690 $ & $ i$\\
$ 55585.85619 $ & $  -0.00022 $ & $   0.00096 $ & $  10.04600 $ & $ i$\\
$ 55585.85669 $ & $   0.00019 $ & $   0.00095 $ & $  10.04610 $ & $ i$\\
$ 55585.85718 $ & $   0.00182 $ & $   0.00097 $ & $  10.04900 $ & $ i$\\
$ 55585.85768 $ & $  -0.00096 $ & $   0.00095 $ & $  10.04480 $ & $ i$\\
$ 55585.85815 $ & $  -0.00141 $ & $   0.00095 $ & $  10.04480 $ & $ i$\\
$ 55585.85864 $ & $  -0.00126 $ & $   0.00096 $ & $  10.04510 $ & $ i$\\
$ 55585.85914 $ & $   0.00034 $ & $   0.00096 $ & $  10.04650 $ & $ i$\\
$ 55585.85963 $ & $  -0.00149 $ & $   0.00097 $ & $  10.04450 $ & $ i$\\
$ 55585.86012 $ & $  -0.00280 $ & $   0.00096 $ & $  10.04340 $ & $ i$\\
$ 55585.86062 $ & $   0.00549 $ & $   0.00099 $ & $  10.05210 $ & $ i$\\
$ 55585.86112 $ & $   0.00071 $ & $   0.00097 $ & $  10.04610 $ & $ i$\\
$ 55585.86162 $ & $  -0.00314 $ & $   0.00095 $ & $  10.04300 $ & $ i$\\
$ 55585.86210 $ & $   0.00189 $ & $   0.00097 $ & $  10.04790 $ & $ i$\\
$ 55585.86258 $ & $  -0.00208 $ & $   0.00096 $ & $  10.04450 $ & $ i$\\
$ 55585.86308 $ & $  -0.00205 $ & $   0.00099 $ & $  10.04410 $ & $ i$\\
$ 55585.86357 $ & $   0.00028 $ & $   0.00098 $ & $  10.04660 $ & $ i$\\
$ 55585.86406 $ & $   0.00096 $ & $   0.00095 $ & $  10.04660 $ & $ i$\\
$ 55585.86456 $ & $  -0.00046 $ & $   0.00095 $ & $  10.04520 $ & $ i$\\
$ 55585.86507 $ & $   0.00177 $ & $   0.00097 $ & $  10.04770 $ & $ i$\\
$ 55585.86556 $ & $  -0.00034 $ & $   0.00097 $ & $  10.04600 $ & $ i$\\
$ 55585.86604 $ & $  -0.00180 $ & $   0.00097 $ & $  10.04410 $ & $ i$\\
$ 55585.86653 $ & $  -0.00181 $ & $   0.00097 $ & $  10.04420 $ & $ i$\\
$ 55585.86704 $ & $  -0.00108 $ & $   0.00097 $ & $  10.04500 $ & $ i$\\
$ 55585.86753 $ & $   0.00254 $ & $   0.00096 $ & $  10.04910 $ & $ i$\\
$ 55585.86802 $ & $  -0.00183 $ & $   0.00097 $ & $  10.04440 $ & $ i$\\
$ 55585.86851 $ & $   0.00134 $ & $   0.00099 $ & $  10.04730 $ & $ i$\\
$ 55585.86901 $ & $  -0.00005 $ & $   0.00098 $ & $  10.04560 $ & $ i$\\
$ 55585.86951 $ & $   0.00146 $ & $   0.00095 $ & $  10.04740 $ & $ i$\\
$ 55585.86999 $ & $   0.00035 $ & $   0.00097 $ & $  10.04610 $ & $ i$\\
$ 55585.87048 $ & $   0.00038 $ & $   0.00095 $ & $  10.04640 $ & $ i$\\
$ 55585.87098 $ & $  -0.00311 $ & $   0.00098 $ & $  10.04310 $ & $ i$\\
$ 55585.87148 $ & $  -0.00090 $ & $   0.00098 $ & $  10.04570 $ & $ i$\\
$ 55585.87196 $ & $   0.00096 $ & $   0.00095 $ & $  10.04740 $ & $ i$\\
$ 55585.87247 $ & $  -0.00102 $ & $   0.00097 $ & $  10.04500 $ & $ i$\\
$ 55585.87296 $ & $  -0.00158 $ & $   0.00096 $ & $  10.04440 $ & $ i$\\
$ 55585.87345 $ & $   0.00218 $ & $   0.00099 $ & $  10.04830 $ & $ i$\\
$ 55585.87393 $ & $  -0.00140 $ & $   0.00098 $ & $  10.04480 $ & $ i$\\
$ 55585.87442 $ & $   0.00513 $ & $   0.00097 $ & $  10.05130 $ & $ i$\\
$ 55585.87492 $ & $   0.00136 $ & $   0.00097 $ & $  10.04750 $ & $ i$\\
$ 55585.87542 $ & $  -0.00003 $ & $   0.00097 $ & $  10.04580 $ & $ i$\\
$ 55585.87591 $ & $   0.00114 $ & $   0.00097 $ & $  10.04730 $ & $ i$\\
$ 55585.87641 $ & $   0.00058 $ & $   0.00098 $ & $  10.04550 $ & $ i$\\
$ 55585.87690 $ & $   0.00106 $ & $   0.00098 $ & $  10.04710 $ & $ i$\\
$ 55585.87739 $ & $  -0.00058 $ & $   0.00096 $ & $  10.04580 $ & $ i$\\
$ 55585.87787 $ & $   0.00284 $ & $   0.00096 $ & $  10.04850 $ & $ i$\\
$ 55585.87836 $ & $  -0.00312 $ & $   0.00100 $ & $  10.04250 $ & $ i$\\
$ 55585.87886 $ & $   0.00378 $ & $   0.00097 $ & $  10.04910 $ & $ i$\\
$ 55585.87937 $ & $   0.00269 $ & $   0.00099 $ & $  10.04840 $ & $ i$\\
$ 55585.87985 $ & $   0.00488 $ & $   0.00100 $ & $  10.05050 $ & $ i$\\
$ 55585.88035 $ & $   0.00239 $ & $   0.00097 $ & $  10.04830 $ & $ i$\\
$ 55585.88084 $ & $   0.00414 $ & $   0.00098 $ & $  10.04940 $ & $ i$\\
$ 55585.88134 $ & $   0.00504 $ & $   0.00102 $ & $  10.05030 $ & $ i$\\
$ 55585.88181 $ & $   0.00487 $ & $   0.00098 $ & $  10.05070 $ & $ i$\\
$ 55585.88231 $ & $   0.00595 $ & $   0.00095 $ & $  10.05120 $ & $ i$\\
$ 55585.88280 $ & $   0.00590 $ & $   0.00099 $ & $  10.05210 $ & $ i$\\
$ 55585.88330 $ & $   0.00532 $ & $   0.00100 $ & $  10.05110 $ & $ i$\\
$ 55585.88379 $ & $   0.00568 $ & $   0.00097 $ & $  10.05120 $ & $ i$\\
$ 55585.88429 $ & $   0.00534 $ & $   0.00095 $ & $  10.05050 $ & $ i$\\
$ 55585.88479 $ & $   0.00639 $ & $   0.00096 $ & $  10.05190 $ & $ i$\\
$ 55585.88528 $ & $   0.00943 $ & $   0.00097 $ & $  10.05510 $ & $ i$\\
$ 55585.88576 $ & $   0.00599 $ & $   0.00098 $ & $  10.05160 $ & $ i$\\
$ 55585.88625 $ & $   0.00566 $ & $   0.00098 $ & $  10.05100 $ & $ i$\\
$ 55585.88674 $ & $   0.00795 $ & $   0.00097 $ & $  10.05400 $ & $ i$\\
$ 55585.88725 $ & $   0.00868 $ & $   0.00097 $ & $  10.05450 $ & $ i$\\
$ 55585.88774 $ & $   0.00880 $ & $   0.00098 $ & $  10.05440 $ & $ i$\\
$ 55585.88824 $ & $   0.01009 $ & $   0.00097 $ & $  10.05630 $ & $ i$\\
$ 55585.88873 $ & $   0.01111 $ & $   0.00096 $ & $  10.05670 $ & $ i$\\
$ 55585.88922 $ & $   0.00570 $ & $   0.00098 $ & $  10.05130 $ & $ i$\\
$ 55585.88970 $ & $   0.01113 $ & $   0.00098 $ & $  10.05690 $ & $ i$\\
$ 55585.89019 $ & $   0.01124 $ & $   0.00100 $ & $  10.05660 $ & $ i$\\
$ 55585.89071 $ & $   0.00957 $ & $   0.00098 $ & $  10.05450 $ & $ i$\\
$ 55585.89120 $ & $   0.01062 $ & $   0.00099 $ & $  10.05620 $ & $ i$\\
$ 55585.89169 $ & $   0.00859 $ & $   0.00098 $ & $  10.05370 $ & $ i$\\
$ 55585.89218 $ & $   0.00622 $ & $   0.00101 $ & $  10.05160 $ & $ i$\\
$ 55585.89268 $ & $   0.00892 $ & $   0.00097 $ & $  10.05420 $ & $ i$\\
$ 55585.89315 $ & $   0.00916 $ & $   0.00100 $ & $  10.05490 $ & $ i$\\
$ 55585.89365 $ & $   0.01212 $ & $   0.00099 $ & $  10.05730 $ & $ i$\\
$ 55585.89414 $ & $   0.00790 $ & $   0.00098 $ & $  10.05320 $ & $ i$\\
$ 55585.89465 $ & $   0.01155 $ & $   0.00099 $ & $  10.05730 $ & $ i$\\
$ 55585.89515 $ & $   0.01190 $ & $   0.00096 $ & $  10.05700 $ & $ i$\\
$ 55585.89563 $ & $   0.01023 $ & $   0.00100 $ & $  10.05580 $ & $ i$\\
$ 55585.89613 $ & $   0.00792 $ & $   0.00100 $ & $  10.05310 $ & $ i$\\
$ 55585.89661 $ & $   0.01063 $ & $   0.00098 $ & $  10.05580 $ & $ i$\\
$ 55585.89711 $ & $   0.00897 $ & $   0.00097 $ & $  10.05390 $ & $ i$\\
$ 55585.89759 $ & $   0.00920 $ & $   0.00100 $ & $  10.05410 $ & $ i$\\
$ 55585.89808 $ & $   0.01213 $ & $   0.00100 $ & $  10.05730 $ & $ i$\\
$ 55585.89858 $ & $   0.01032 $ & $   0.00098 $ & $  10.05530 $ & $ i$\\
$ 55585.89908 $ & $   0.01034 $ & $   0.00099 $ & $  10.05540 $ & $ i$\\
$ 55585.89957 $ & $   0.01033 $ & $   0.00099 $ & $  10.05570 $ & $ i$\\
$ 55585.90006 $ & $   0.01042 $ & $   0.00097 $ & $  10.05570 $ & $ i$\\
$ 55585.90056 $ & $   0.00806 $ & $   0.00100 $ & $  10.05340 $ & $ i$\\
$ 55585.90104 $ & $   0.01057 $ & $   0.00096 $ & $  10.05580 $ & $ i$\\
$ 55585.90154 $ & $   0.01121 $ & $   0.00096 $ & $  10.05660 $ & $ i$\\
$ 55585.90203 $ & $   0.00796 $ & $   0.00096 $ & $  10.05250 $ & $ i$\\
$ 55585.90254 $ & $   0.00945 $ & $   0.00099 $ & $  10.05450 $ & $ i$\\
$ 55585.90304 $ & $   0.00911 $ & $   0.00096 $ & $  10.05390 $ & $ i$\\
$ 55585.90352 $ & $   0.01130 $ & $   0.00097 $ & $  10.05690 $ & $ i$\\
$ 55585.90401 $ & $   0.01409 $ & $   0.00096 $ & $  10.05890 $ & $ i$\\
$ 55585.90450 $ & $   0.00892 $ & $   0.00096 $ & $  10.05380 $ & $ i$\\
$ 55585.90499 $ & $   0.01382 $ & $   0.00096 $ & $  10.05880 $ & $ i$\\
$ 55585.90548 $ & $   0.00830 $ & $   0.00096 $ & $  10.05390 $ & $ i$\\
$ 55585.90598 $ & $   0.00941 $ & $   0.00096 $ & $  10.05470 $ & $ i$\\
$ 55585.90648 $ & $   0.01248 $ & $   0.00097 $ & $  10.05790 $ & $ i$\\
$ 55585.90698 $ & $   0.00591 $ & $   0.00099 $ & $  10.05060 $ & $ i$\\
$ 55585.90746 $ & $   0.01174 $ & $   0.00101 $ & $  10.05680 $ & $ i$\\
$ 55585.90796 $ & $   0.00718 $ & $   0.00097 $ & $  10.05190 $ & $ i$\\
$ 55585.90845 $ & $   0.00848 $ & $   0.00099 $ & $  10.05350 $ & $ i$\\
$ 55585.90894 $ & $   0.00638 $ & $   0.00098 $ & $  10.05070 $ & $ i$\\
$ 55585.90942 $ & $   0.01164 $ & $   0.00100 $ & $  10.05680 $ & $ i$\\
$ 55585.90992 $ & $   0.00869 $ & $   0.00099 $ & $  10.05360 $ & $ i$\\
$ 55585.91043 $ & $   0.01236 $ & $   0.00100 $ & $  10.05740 $ & $ i$\\
$ 55585.91092 $ & $   0.01262 $ & $   0.00101 $ & $  10.05740 $ & $ i$\\
$ 55585.91140 $ & $   0.00849 $ & $   0.00101 $ & $  10.05320 $ & $ i$\\
$ 55585.91189 $ & $   0.01076 $ & $   0.00102 $ & $  10.05550 $ & $ i$\\
$ 55585.91238 $ & $   0.01231 $ & $   0.00112 $ & $  10.05770 $ & $ i$\\
$ 55585.91287 $ & $   0.01145 $ & $   0.00099 $ & $  10.05630 $ & $ i$\\
$ 55585.91337 $ & $   0.00777 $ & $   0.00097 $ & $  10.05300 $ & $ i$\\
$ 55585.91387 $ & $   0.01009 $ & $   0.00097 $ & $  10.05560 $ & $ i$\\
$ 55585.91437 $ & $   0.01106 $ & $   0.00101 $ & $  10.05550 $ & $ i$\\
$ 55585.91487 $ & $   0.01535 $ & $   0.00109 $ & $  10.06000 $ & $ i$\\
$ 55585.91536 $ & $   0.01524 $ & $   0.00103 $ & $  10.05980 $ & $ i$\\
$ 55585.91584 $ & $   0.00940 $ & $   0.00101 $ & $  10.05370 $ & $ i$\\
$ 55585.91634 $ & $   0.01090 $ & $   0.00097 $ & $  10.05590 $ & $ i$\\
$ 55585.91682 $ & $   0.01218 $ & $   0.00096 $ & $  10.05660 $ & $ i$\\
$ 55585.91731 $ & $   0.01164 $ & $   0.00098 $ & $  10.05620 $ & $ i$\\
$ 55585.91781 $ & $   0.01146 $ & $   0.00096 $ & $  10.05630 $ & $ i$\\
$ 55585.91831 $ & $   0.00643 $ & $   0.00096 $ & $  10.05100 $ & $ i$\\
$ 55585.91881 $ & $   0.01173 $ & $   0.00096 $ & $  10.05590 $ & $ i$\\
$ 55585.91929 $ & $   0.00985 $ & $   0.00102 $ & $  10.05420 $ & $ i$\\
$ 55585.91978 $ & $   0.01086 $ & $   0.00097 $ & $  10.05560 $ & $ i$\\
$ 55585.92027 $ & $   0.00944 $ & $   0.00098 $ & $  10.05370 $ & $ i$\\
$ 55585.92077 $ & $   0.01148 $ & $   0.00101 $ & $  10.05650 $ & $ i$\\
$ 55585.92126 $ & $   0.01150 $ & $   0.00101 $ & $  10.05610 $ & $ i$\\
$ 55585.92175 $ & $   0.01122 $ & $   0.00102 $ & $  10.05570 $ & $ i$\\
$ 55585.92225 $ & $   0.01284 $ & $   0.00105 $ & $  10.05740 $ & $ i$\\
$ 55585.92274 $ & $   0.00812 $ & $   0.00098 $ & $  10.05230 $ & $ i$\\
$ 55629.61605 $ & $  -0.00259 $ & $   0.00130 $ & $  11.31800 $ & $ i$\\
$ 55629.61679 $ & $  -0.00226 $ & $   0.00128 $ & $  11.31860 $ & $ i$\\
$ 55629.61773 $ & $   0.00229 $ & $   0.00129 $ & $  11.32370 $ & $ i$\\
$ 55629.61846 $ & $  -0.00139 $ & $   0.00128 $ & $  11.32000 $ & $ i$\\
$ 55629.61936 $ & $  -0.00036 $ & $   0.00129 $ & $  11.32080 $ & $ i$\\
$ 55629.62009 $ & $   0.00262 $ & $   0.00129 $ & $  11.32380 $ & $ i$\\
$ 55629.62103 $ & $   0.00060 $ & $   0.00127 $ & $  11.32220 $ & $ i$\\
$ 55629.62176 $ & $   0.00238 $ & $   0.00128 $ & $  11.32310 $ & $ i$\\
$ 55629.62269 $ & $  -0.00092 $ & $   0.00128 $ & $  11.32030 $ & $ i$\\
$ 55629.62342 $ & $   0.00062 $ & $   0.00127 $ & $  11.32260 $ & $ i$\\
$ 55629.62434 $ & $  -0.00272 $ & $   0.00127 $ & $  11.31900 $ & $ i$\\
$ 55629.62507 $ & $  -0.00008 $ & $   0.00127 $ & $  11.32160 $ & $ i$\\
$ 55629.62600 $ & $  -0.00027 $ & $   0.00127 $ & $  11.32120 $ & $ i$\\
$ 55629.62674 $ & $   0.00236 $ & $   0.00127 $ & $  11.32510 $ & $ i$\\
$ 55629.62766 $ & $   0.00158 $ & $   0.00128 $ & $  11.32390 $ & $ i$\\
$ 55629.62840 $ & $   0.00102 $ & $   0.00127 $ & $  11.32280 $ & $ i$\\
$ 55629.62932 $ & $  -0.00192 $ & $   0.00127 $ & $  11.31970 $ & $ i$\\
$ 55629.63006 $ & $  -0.00096 $ & $   0.00126 $ & $  11.32100 $ & $ i$\\
$ 55629.63098 $ & $  -0.00149 $ & $   0.00127 $ & $  11.32010 $ & $ i$\\
$ 55629.63171 $ & $  -0.00209 $ & $   0.00126 $ & $  11.32030 $ & $ i$\\
$ 55629.63265 $ & $   0.00085 $ & $   0.00127 $ & $  11.32240 $ & $ i$\\
$ 55629.63338 $ & $   0.00151 $ & $   0.00127 $ & $  11.32400 $ & $ i$\\
$ 55629.63429 $ & $   0.00268 $ & $   0.00127 $ & $  11.32440 $ & $ i$\\
$ 55629.63502 $ & $  -0.00203 $ & $   0.00126 $ & $  11.32080 $ & $ i$\\
$ 55629.63595 $ & $   0.00475 $ & $   0.00127 $ & $  11.32640 $ & $ i$\\
$ 55629.63669 $ & $   0.00234 $ & $   0.00127 $ & $  11.32490 $ & $ i$\\
$ 55629.63762 $ & $   0.00343 $ & $   0.00127 $ & $  11.32490 $ & $ i$\\
$ 55629.63834 $ & $   0.00211 $ & $   0.00127 $ & $  11.32470 $ & $ i$\\
$ 55629.63927 $ & $   0.00434 $ & $   0.00127 $ & $  11.32560 $ & $ i$\\
$ 55629.64001 $ & $   0.00275 $ & $   0.00127 $ & $  11.32510 $ & $ i$\\
$ 55629.64096 $ & $   0.00536 $ & $   0.00126 $ & $  11.32770 $ & $ i$\\
$ 55629.64169 $ & $   0.00274 $ & $   0.00127 $ & $  11.32490 $ & $ i$\\
$ 55629.64259 $ & $   0.00616 $ & $   0.00127 $ & $  11.32840 $ & $ i$\\
$ 55629.64332 $ & $   0.00700 $ & $   0.00127 $ & $  11.32900 $ & $ i$\\
$ 55629.64422 $ & $   0.00510 $ & $   0.00127 $ & $  11.32790 $ & $ i$\\
$ 55629.64495 $ & $   0.00442 $ & $   0.00127 $ & $  11.32670 $ & $ i$\\
$ 55629.64589 $ & $   0.00797 $ & $   0.00127 $ & $  11.33070 $ & $ i$\\
$ 55629.64663 $ & $   0.00798 $ & $   0.00126 $ & $  11.33060 $ & $ i$\\
$ 55629.64755 $ & $   0.00843 $ & $   0.00126 $ & $  11.33080 $ & $ i$\\
$ 55629.64827 $ & $   0.00873 $ & $   0.00127 $ & $  11.33130 $ & $ i$\\
$ 55629.64924 $ & $   0.00831 $ & $   0.00127 $ & $  11.33050 $ & $ i$\\
$ 55629.64998 $ & $   0.00664 $ & $   0.00126 $ & $  11.32910 $ & $ i$\\
$ 55629.65090 $ & $   0.00984 $ & $   0.00127 $ & $  11.33230 $ & $ i$\\
$ 55629.65162 $ & $   0.00502 $ & $   0.00126 $ & $  11.32710 $ & $ i$\\
$ 55629.65253 $ & $   0.00888 $ & $   0.00126 $ & $  11.33180 $ & $ i$\\
$ 55629.65325 $ & $   0.00861 $ & $   0.00126 $ & $  11.33090 $ & $ i$\\
$ 55629.65417 $ & $   0.00606 $ & $   0.00126 $ & $  11.32820 $ & $ i$\\
$ 55629.65489 $ & $   0.00845 $ & $   0.00125 $ & $  11.33080 $ & $ i$\\
$ 55629.65581 $ & $   0.00870 $ & $   0.00126 $ & $  11.33100 $ & $ i$\\
$ 55629.65655 $ & $   0.00536 $ & $   0.00125 $ & $  11.32820 $ & $ i$\\
$ 55629.65750 $ & $   0.01125 $ & $   0.00126 $ & $  11.33420 $ & $ i$\\
$ 55629.65823 $ & $   0.01051 $ & $   0.00125 $ & $  11.33320 $ & $ i$\\
$ 55629.65915 $ & $   0.01009 $ & $   0.00126 $ & $  11.33290 $ & $ i$\\
$ 55629.65988 $ & $   0.00801 $ & $   0.00126 $ & $  11.33080 $ & $ i$\\
$ 55629.66081 $ & $   0.00918 $ & $   0.00125 $ & $  11.33220 $ & $ i$\\
$ 55629.66155 $ & $   0.01061 $ & $   0.00126 $ & $  11.33380 $ & $ i$\\
$ 55629.66247 $ & $   0.00640 $ & $   0.00125 $ & $  11.32950 $ & $ i$\\
$ 55629.66319 $ & $   0.01178 $ & $   0.00126 $ & $  11.33510 $ & $ i$\\
$ 55629.66411 $ & $   0.01055 $ & $   0.00125 $ & $  11.33290 $ & $ i$\\
$ 55629.66484 $ & $   0.00814 $ & $   0.00125 $ & $  11.33050 $ & $ i$\\
$ 55629.66580 $ & $   0.01306 $ & $   0.00126 $ & $  11.33640 $ & $ i$\\
$ 55629.66653 $ & $   0.00950 $ & $   0.00126 $ & $  11.33200 $ & $ i$\\
$ 55629.66745 $ & $   0.01073 $ & $   0.00125 $ & $  11.33360 $ & $ i$\\
$ 55629.66818 $ & $   0.01141 $ & $   0.00124 $ & $  11.33410 $ & $ i$\\
$ 55629.66911 $ & $   0.01299 $ & $   0.00125 $ & $  11.33630 $ & $ i$\\
$ 55629.66985 $ & $   0.00799 $ & $   0.00125 $ & $  11.33100 $ & $ i$\\
$ 55629.67076 $ & $   0.01133 $ & $   0.00125 $ & $  11.33460 $ & $ i$\\
$ 55629.67149 $ & $   0.01179 $ & $   0.00125 $ & $  11.33490 $ & $ i$\\
$ 55629.67239 $ & $   0.00867 $ & $   0.00125 $ & $  11.33150 $ & $ i$\\
$ 55629.67312 $ & $   0.01227 $ & $   0.00125 $ & $  11.33490 $ & $ i$\\
$ 55629.67407 $ & $   0.01058 $ & $   0.00125 $ & $  11.33360 $ & $ i$\\
$ 55629.67480 $ & $   0.01152 $ & $   0.00125 $ & $  11.33480 $ & $ i$\\
$ 55629.67574 $ & $   0.01075 $ & $   0.00125 $ & $  11.33370 $ & $ i$\\
$ 55629.67646 $ & $   0.01297 $ & $   0.00125 $ & $  11.33570 $ & $ i$\\
$ 55629.67739 $ & $   0.01150 $ & $   0.00126 $ & $  11.33470 $ & $ i$\\
$ 55629.67813 $ & $   0.01308 $ & $   0.00126 $ & $  11.33580 $ & $ i$\\
$ 55629.67904 $ & $   0.01248 $ & $   0.00125 $ & $  11.33560 $ & $ i$\\
$ 55629.67977 $ & $   0.01316 $ & $   0.00126 $ & $  11.33630 $ & $ i$\\
$ 55629.68070 $ & $   0.00955 $ & $   0.00125 $ & $  11.33300 $ & $ i$\\
$ 55629.68143 $ & $   0.01100 $ & $   0.00125 $ & $  11.33400 $ & $ i$\\
$ 55629.68237 $ & $   0.00817 $ & $   0.00125 $ & $  11.33150 $ & $ i$\\
$ 55629.68311 $ & $   0.01118 $ & $   0.00125 $ & $  11.33460 $ & $ i$\\
$ 55629.68401 $ & $   0.01198 $ & $   0.00126 $ & $  11.33510 $ & $ i$\\
$ 55629.68473 $ & $   0.00682 $ & $   0.00125 $ & $  11.32990 $ & $ i$\\
$ 55629.68567 $ & $   0.01129 $ & $   0.00125 $ & $  11.33380 $ & $ i$\\
$ 55629.68641 $ & $   0.01279 $ & $   0.00125 $ & $  11.33660 $ & $ i$\\
$ 55629.68733 $ & $   0.01074 $ & $   0.00125 $ & $  11.33390 $ & $ i$\\
$ 55629.68806 $ & $   0.01065 $ & $   0.00126 $ & $  11.33330 $ & $ i$\\
$ 55629.68899 $ & $   0.01190 $ & $   0.00125 $ & $  11.33530 $ & $ i$\\
$ 55629.68972 $ & $   0.00978 $ & $   0.00125 $ & $  11.33320 $ & $ i$\\
$ 55629.69066 $ & $   0.01078 $ & $   0.00126 $ & $  11.33370 $ & $ i$\\
$ 55629.69140 $ & $   0.01070 $ & $   0.00126 $ & $  11.33350 $ & $ i$\\
$ 55629.69231 $ & $   0.00970 $ & $   0.00125 $ & $  11.33360 $ & $ i$\\
$ 55629.69305 $ & $   0.00836 $ & $   0.00125 $ & $  11.33100 $ & $ i$\\
$ 55629.69398 $ & $   0.01050 $ & $   0.00126 $ & $  11.33260 $ & $ i$\\
$ 55629.69471 $ & $   0.01154 $ & $   0.00126 $ & $  11.33380 $ & $ i$\\
$ 55629.69563 $ & $   0.01013 $ & $   0.00126 $ & $  11.33240 $ & $ i$\\
$ 55629.69636 $ & $   0.01153 $ & $   0.00127 $ & $  11.33400 $ & $ i$\\
$ 55629.69729 $ & $   0.01190 $ & $   0.00126 $ & $  11.33470 $ & $ i$\\
$ 55629.69804 $ & $   0.01193 $ & $   0.00126 $ & $  11.33520 $ & $ i$\\
$ 55629.69898 $ & $   0.01078 $ & $   0.00126 $ & $  11.33470 $ & $ i$\\
$ 55629.69972 $ & $   0.01068 $ & $   0.00126 $ & $  11.33440 $ & $ i$\\
$ 55629.70063 $ & $   0.01075 $ & $   0.00126 $ & $  11.33390 $ & $ i$\\
$ 55629.70137 $ & $   0.01261 $ & $   0.00126 $ & $  11.33650 $ & $ i$\\
$ 55629.70230 $ & $   0.01140 $ & $   0.00126 $ & $  11.33460 $ & $ i$\\
$ 55629.70303 $ & $   0.01104 $ & $   0.00126 $ & $  11.33480 $ & $ i$\\
$ 55629.70393 $ & $   0.01269 $ & $   0.00126 $ & $  11.33590 $ & $ i$\\
$ 55629.70467 $ & $   0.01250 $ & $   0.00126 $ & $  11.33650 $ & $ i$\\
$ 55629.70559 $ & $   0.01355 $ & $   0.00125 $ & $  11.33690 $ & $ i$\\
$ 55629.70631 $ & $   0.01374 $ & $   0.00126 $ & $  11.33730 $ & $ i$\\
$ 55629.70729 $ & $   0.01150 $ & $   0.00125 $ & $  11.33440 $ & $ i$\\
$ 55629.70802 $ & $   0.01328 $ & $   0.00126 $ & $  11.33730 $ & $ i$\\
$ 55629.70895 $ & $   0.01147 $ & $   0.00126 $ & $  11.33460 $ & $ i$\\
$ 55629.70968 $ & $   0.01344 $ & $   0.00125 $ & $  11.33650 $ & $ i$\\
$ 55629.71062 $ & $   0.01166 $ & $   0.00125 $ & $  11.33500 $ & $ i$\\
$ 55629.71134 $ & $   0.00789 $ & $   0.00125 $ & $  11.33120 $ & $ i$\\
$ 55629.71228 $ & $   0.01410 $ & $   0.00125 $ & $  11.33770 $ & $ i$\\
$ 55629.71302 $ & $   0.00799 $ & $   0.00125 $ & $  11.33060 $ & $ i$\\
$ 55629.71394 $ & $   0.01135 $ & $   0.00126 $ & $  11.33370 $ & $ i$\\
$ 55629.71467 $ & $   0.01016 $ & $   0.00126 $ & $  11.33340 $ & $ i$\\
$ 55629.71564 $ & $   0.01138 $ & $   0.00126 $ & $  11.33480 $ & $ i$\\
$ 55629.71636 $ & $   0.01396 $ & $   0.00125 $ & $  11.33750 $ & $ i$\\
$ 55629.71730 $ & $   0.01294 $ & $   0.00125 $ & $  11.33590 $ & $ i$\\
$ 55629.71803 $ & $   0.00987 $ & $   0.00125 $ & $  11.33330 $ & $ i$\\
$ 55629.71894 $ & $   0.01162 $ & $   0.00126 $ & $  11.33470 $ & $ i$\\
$ 55629.71966 $ & $   0.01140 $ & $   0.00125 $ & $  11.33470 $ & $ i$\\
$ 55629.72057 $ & $   0.01203 $ & $   0.00126 $ & $  11.33500 $ & $ i$\\
$ 55629.72131 $ & $   0.00952 $ & $   0.00125 $ & $  11.33380 $ & $ i$\\
$ 55629.72224 $ & $   0.01171 $ & $   0.00126 $ & $  11.33560 $ & $ i$\\
$ 55629.72296 $ & $   0.01181 $ & $   0.00125 $ & $  11.33580 $ & $ i$\\
$ 55629.72389 $ & $   0.00969 $ & $   0.00125 $ & $  11.33330 $ & $ i$\\
$ 55629.72464 $ & $   0.01276 $ & $   0.00125 $ & $  11.33600 $ & $ i$\\
$ 55629.72555 $ & $   0.01120 $ & $   0.00125 $ & $  11.33510 $ & $ i$\\
$ 55629.72628 $ & $   0.01316 $ & $   0.00126 $ & $  11.33630 $ & $ i$\\
$ 55629.72722 $ & $   0.01188 $ & $   0.00125 $ & $  11.33520 $ & $ i$\\
$ 55629.72795 $ & $   0.01215 $ & $   0.00125 $ & $  11.33540 $ & $ i$\\
$ 55629.72887 $ & $   0.01007 $ & $   0.00125 $ & $  11.33400 $ & $ i$\\
$ 55629.72960 $ & $   0.01001 $ & $   0.00125 $ & $  11.33330 $ & $ i$\\
$ 55629.73053 $ & $   0.01321 $ & $   0.00125 $ & $  11.33650 $ & $ i$\\
$ 55629.73126 $ & $   0.01230 $ & $   0.00125 $ & $  11.33550 $ & $ i$\\
$ 55629.73217 $ & $   0.00775 $ & $   0.00124 $ & $  11.33170 $ & $ i$\\
$ 55629.73291 $ & $   0.01233 $ & $   0.00126 $ & $  11.33550 $ & $ i$\\
$ 55629.73382 $ & $   0.01125 $ & $   0.00126 $ & $  11.33500 $ & $ i$\\
$ 55629.73455 $ & $   0.01439 $ & $   0.00125 $ & $  11.33810 $ & $ i$\\
$ 55629.73546 $ & $   0.01235 $ & $   0.00126 $ & $  11.33580 $ & $ i$\\
$ 55629.73620 $ & $   0.00793 $ & $   0.00125 $ & $  11.33290 $ & $ i$\\
$ 55629.73712 $ & $   0.00730 $ & $   0.00125 $ & $  11.33090 $ & $ i$\\
$ 55629.73785 $ & $   0.01323 $ & $   0.00125 $ & $  11.33680 $ & $ i$\\
$ 55629.73878 $ & $   0.01453 $ & $   0.00124 $ & $  11.33850 $ & $ i$\\
$ 55629.73951 $ & $   0.01089 $ & $   0.00124 $ & $  11.33490 $ & $ i$\\
$ 55629.74044 $ & $   0.01271 $ & $   0.00125 $ & $  11.33580 $ & $ i$\\
$ 55629.74116 $ & $   0.01054 $ & $   0.00125 $ & $  11.33460 $ & $ i$\\
$ 55629.74208 $ & $   0.00960 $ & $   0.00124 $ & $  11.33280 $ & $ i$\\
$ 55629.74282 $ & $   0.01177 $ & $   0.00125 $ & $  11.33530 $ & $ i$\\
$ 55629.74374 $ & $   0.01210 $ & $   0.00125 $ & $  11.33610 $ & $ i$\\
$ 55629.74447 $ & $   0.00989 $ & $   0.00125 $ & $  11.33350 $ & $ i$\\
$ 55629.74540 $ & $   0.01372 $ & $   0.00126 $ & $  11.33670 $ & $ i$\\
$ 55629.74614 $ & $   0.01089 $ & $   0.00125 $ & $  11.33460 $ & $ i$\\
$ 55629.74706 $ & $   0.01010 $ & $   0.00125 $ & $  11.33350 $ & $ i$\\
$ 55629.74778 $ & $   0.00870 $ & $   0.00126 $ & $  11.33110 $ & $ i$\\
$ 55629.74872 $ & $   0.00849 $ & $   0.00126 $ & $  11.33190 $ & $ i$\\
$ 55629.74946 $ & $   0.01028 $ & $   0.00126 $ & $  11.33330 $ & $ i$\\
$ 55629.75037 $ & $   0.00954 $ & $   0.00125 $ & $  11.33260 $ & $ i$\\
$ 55629.75113 $ & $   0.01233 $ & $   0.00126 $ & $  11.33630 $ & $ i$\\
$ 55629.75204 $ & $   0.01086 $ & $   0.00126 $ & $  11.33400 $ & $ i$\\
$ 55629.75278 $ & $   0.01334 $ & $   0.00126 $ & $  11.33640 $ & $ i$\\
$ 55629.75370 $ & $   0.00860 $ & $   0.00126 $ & $  11.33180 $ & $ i$\\
$ 55629.75444 $ & $   0.01048 $ & $   0.00126 $ & $  11.33340 $ & $ i$\\
$ 55629.75535 $ & $   0.01103 $ & $   0.00126 $ & $  11.33420 $ & $ i$\\
$ 55629.75609 $ & $   0.00751 $ & $   0.00126 $ & $  11.33150 $ & $ i$\\
$ 55629.75703 $ & $   0.00641 $ & $   0.00126 $ & $  11.33020 $ & $ i$\\
$ 55629.75776 $ & $   0.00712 $ & $   0.00125 $ & $  11.33110 $ & $ i$\\
$ 55629.75870 $ & $   0.01229 $ & $   0.00127 $ & $  11.33550 $ & $ i$\\
$ 55629.75944 $ & $   0.00989 $ & $   0.00126 $ & $  11.33400 $ & $ i$\\
$ 55629.76036 $ & $   0.01111 $ & $   0.00126 $ & $  11.33490 $ & $ i$\\
$ 55629.76110 $ & $   0.01146 $ & $   0.00126 $ & $  11.33530 $ & $ i$\\
$ 55629.76203 $ & $   0.00951 $ & $   0.00126 $ & $  11.33330 $ & $ i$\\
$ 55629.76276 $ & $   0.00790 $ & $   0.00126 $ & $  11.33170 $ & $ i$\\
$ 55629.76368 $ & $   0.00974 $ & $   0.00126 $ & $  11.33340 $ & $ i$\\
$ 55629.76441 $ & $   0.01009 $ & $   0.00126 $ & $  11.33310 $ & $ i$\\
$ 55629.76535 $ & $   0.01377 $ & $   0.00127 $ & $  11.33770 $ & $ i$\\
$ 55629.76608 $ & $   0.01057 $ & $   0.00127 $ & $  11.33380 $ & $ i$\\
$ 55629.76702 $ & $   0.00999 $ & $   0.00127 $ & $  11.33410 $ & $ i$\\
$ 55629.76775 $ & $   0.00720 $ & $   0.00126 $ & $  11.33170 $ & $ i$\\
$ 55629.76867 $ & $   0.01084 $ & $   0.00126 $ & $  11.33480 $ & $ i$\\
$ 55629.76941 $ & $   0.00812 $ & $   0.00126 $ & $  11.33200 $ & $ i$\\
$ 55629.77030 $ & $   0.00892 $ & $   0.00127 $ & $  11.33180 $ & $ i$\\
$ 55629.77102 $ & $   0.00847 $ & $   0.00126 $ & $  11.33240 $ & $ i$\\
$ 55629.77194 $ & $   0.00944 $ & $   0.00127 $ & $  11.33270 $ & $ i$\\
$ 55629.77268 $ & $   0.00903 $ & $   0.00126 $ & $  11.33290 $ & $ i$\\
$ 55629.77360 $ & $   0.01091 $ & $   0.00127 $ & $  11.33470 $ & $ i$\\
$ 55629.77434 $ & $   0.00733 $ & $   0.00126 $ & $  11.33060 $ & $ i$\\
$ 55629.77527 $ & $   0.01108 $ & $   0.00127 $ & $  11.33390 $ & $ i$\\
$ 55629.77600 $ & $   0.00896 $ & $   0.00127 $ & $  11.33300 $ & $ i$\\
$ 55629.77690 $ & $   0.01000 $ & $   0.00127 $ & $  11.33260 $ & $ i$\\
$ 55629.77763 $ & $   0.00946 $ & $   0.00127 $ & $  11.33350 $ & $ i$\\
$ 55629.77855 $ & $   0.00743 $ & $   0.00127 $ & $  11.33150 $ & $ i$\\
$ 55629.77928 $ & $   0.01110 $ & $   0.00127 $ & $  11.33390 $ & $ i$\\
$ 55629.78020 $ & $   0.01079 $ & $   0.00127 $ & $  11.33400 $ & $ i$\\
$ 55629.78094 $ & $   0.00899 $ & $   0.00126 $ & $  11.33250 $ & $ i$\\
$ 55629.78188 $ & $   0.00643 $ & $   0.00126 $ & $  11.33000 $ & $ i$\\
$ 55629.78259 $ & $   0.01184 $ & $   0.00126 $ & $  11.33480 $ & $ i$\\
$ 55629.78352 $ & $   0.00617 $ & $   0.00128 $ & $  11.32890 $ & $ i$\\
$ 55629.78426 $ & $   0.00615 $ & $   0.00126 $ & $  11.33070 $ & $ i$\\
$ 55629.78518 $ & $   0.00661 $ & $   0.00126 $ & $  11.33040 $ & $ i$\\
$ 55629.78592 $ & $   0.00657 $ & $   0.00127 $ & $  11.32980 $ & $ i$\\
$ 55629.78684 $ & $   0.00713 $ & $   0.00126 $ & $  11.33030 $ & $ i$\\
$ 55629.78756 $ & $   0.00507 $ & $   0.00126 $ & $  11.32810 $ & $ i$\\
$ 55629.78849 $ & $   0.00440 $ & $   0.00126 $ & $  11.32770 $ & $ i$\\
$ 55629.78921 $ & $   0.00359 $ & $   0.00126 $ & $  11.32630 $ & $ i$\\
$ 55629.79015 $ & $   0.00241 $ & $   0.00126 $ & $  11.32600 $ & $ i$\\
$ 55629.79089 $ & $   0.00003 $ & $   0.00125 $ & $  11.32330 $ & $ i$\\
$ 55629.79181 $ & $  -0.00091 $ & $   0.00127 $ & $  11.32230 $ & $ i$\\
$ 55629.79254 $ & $   0.00482 $ & $   0.00127 $ & $  11.32720 $ & $ i$\\
$ 55629.79346 $ & $   0.00219 $ & $   0.00127 $ & $  11.32480 $ & $ i$\\
$ 55629.79418 $ & $   0.00235 $ & $   0.00127 $ & $  11.32560 $ & $ i$\\
$ 55629.79508 $ & $  -0.00036 $ & $   0.00127 $ & $  11.32260 $ & $ i$\\
$ 55629.79582 $ & $   0.00072 $ & $   0.00129 $ & $  11.32330 $ & $ i$\\
$ 55629.79674 $ & $  -0.00039 $ & $   0.00127 $ & $  11.32310 $ & $ i$\\
$ 55629.79748 $ & $   0.00002 $ & $   0.00127 $ & $  11.32360 $ & $ i$\\
$ 55629.79843 $ & $  -0.00145 $ & $   0.00128 $ & $  11.32160 $ & $ i$\\
$ 55629.79916 $ & $   0.00094 $ & $   0.00127 $ & $  11.32420 $ & $ i$\\
$ 55629.80008 $ & $   0.00013 $ & $   0.00127 $ & $  11.32350 $ & $ i$\\
$ 55629.80082 $ & $  -0.00226 $ & $   0.00127 $ & $  11.32090 $ & $ i$\\
$ 55629.80175 $ & $  -0.00277 $ & $   0.00127 $ & $  11.32050 $ & $ i$\\
$ 55629.80249 $ & $   0.00099 $ & $   0.00127 $ & $  11.32450 $ & $ i$\\
$ 55629.80341 $ & $  -0.00006 $ & $   0.00127 $ & $  11.32390 $ & $ i$\\
$ 55629.80414 $ & $   0.00088 $ & $   0.00127 $ & $  11.32460 $ & $ i$\\
$ 55629.80579 $ & $   0.00132 $ & $   0.00127 $ & $  11.32550 $ & $ i$\\
$ 55629.80674 $ & $  -0.00286 $ & $   0.00127 $ & $  11.32150 $ & $ i$\\
$ 55629.80746 $ & $  -0.00034 $ & $   0.00127 $ & $  11.32320 $ & $ i$\\
$ 55629.80840 $ & $  -0.00181 $ & $   0.00128 $ & $  11.32230 $ & $ i$\\
$ 55629.80913 $ & $  -0.00145 $ & $   0.00127 $ & $  11.32190 $ & $ i$\\
$ 55629.81006 $ & $   0.00030 $ & $   0.00127 $ & $  11.32410 $ & $ i$\\
$ 55629.81080 $ & $  -0.00046 $ & $   0.00128 $ & $  11.32290 $ & $ i$\\
$ 55629.81172 $ & $  -0.00278 $ & $   0.00127 $ & $  11.32120 $ & $ i$\\
$ 55629.81246 $ & $  -0.00351 $ & $   0.00128 $ & $  11.32140 $ & $ i$\\
$ 55629.81338 $ & $  -0.00217 $ & $   0.00128 $ & $  11.32230 $ & $ i$\\
$ 55629.81411 $ & $  -0.00034 $ & $   0.00129 $ & $  11.32380 $ & $ i$\\
$ 55629.81505 $ & $   0.00262 $ & $   0.00128 $ & $  11.32740 $ & $ i$\\
$ 55629.81576 $ & $   0.00178 $ & $   0.00128 $ & $  11.32590 $ & $ i$\\
$ 55629.81668 $ & $   0.00117 $ & $   0.00128 $ & $  11.32640 $ & $ i$\\
$ 55629.81741 $ & $  -0.00282 $ & $   0.00128 $ & $  11.32290 $ & $ i$\\
$ 55629.81837 $ & $   0.00343 $ & $   0.00129 $ & $  11.32820 $ & $ i$\\
$ 55629.81911 $ & $   0.00121 $ & $   0.00129 $ & $  11.32540 $ & $ i$\\
$ 55629.82001 $ & $  -0.00119 $ & $   0.00128 $ & $  11.32260 $ & $ i$\\
$ 55629.82075 $ & $  -0.00082 $ & $   0.00129 $ & $  11.32330 $ & $ i$\\
$ 55629.82168 $ & $   0.00389 $ & $   0.00130 $ & $  11.32770 $ & $ i$\\
$ 55629.82241 $ & $   0.00228 $ & $   0.00130 $ & $  11.32610 $ & $ i$\\
$ 55629.82337 $ & $   0.00200 $ & $   0.00131 $ & $  11.32510 $ & $ i$\\
$ 55629.82410 $ & $  -0.00039 $ & $   0.00132 $ & $  11.32320 $ & $ i$\\
$ 55629.82503 $ & $  -0.00099 $ & $   0.00130 $ & $  11.32240 $ & $ i$\\
$ 55629.82575 $ & $  -0.00103 $ & $   0.00129 $ & $  11.32040 $ & $ i$\\
$ 55629.82667 $ & $   0.00007 $ & $   0.00130 $ & $  11.32420 $ & $ i$\\
$ 55629.82739 $ & $  -0.00015 $ & $   0.00130 $ & $  11.32400 $ & $ i$\\
$ 55629.82833 $ & $   0.00058 $ & $   0.00131 $ & $  11.32480 $ & $ i$\\
$ 55629.82907 $ & $  -0.00009 $ & $   0.00130 $ & $  11.32430 $ & $ i$\\
$ 55629.82999 $ & $  -0.00114 $ & $   0.00130 $ & $  11.32300 $ & $ i$\\
$ 55629.83073 $ & $   0.00364 $ & $   0.00130 $ & $  11.32880 $ & $ i$\\
$ 55629.83167 $ & $  -0.00048 $ & $   0.00130 $ & $  11.32470 $ & $ i$\\
$ 55629.83239 $ & $   0.00297 $ & $   0.00129 $ & $  11.32750 $ & $ i$\\
$ 55629.83333 $ & $   0.00159 $ & $   0.00129 $ & $  11.32590 $ & $ i$\\
$ 55629.83407 $ & $   0.00053 $ & $   0.00131 $ & $  11.32410 $ & $ i$\\
$ 55629.83499 $ & $  -0.00142 $ & $   0.00131 $ & $  11.32210 $ & $ i$\\
$ 55629.83573 $ & $  -0.00066 $ & $   0.00131 $ & $  11.32260 $ & $ i$\\
$ 55629.83665 $ & $  -0.00122 $ & $   0.00131 $ & $  11.32280 $ & $ i$\\
$ 55629.83738 $ & $  -0.00168 $ & $   0.00131 $ & $  11.32150 $ & $ i$\\


==> data/HTR364-003_phfu_tab_short.tex <==
$ 55578.68612 $ & $   0.00996 $ & $   0.00115 $ & $  11.35390 $ & $ i$\\
$ 55578.68766 $ & $   0.01222 $ & $   0.00104 $ & $  11.35670 $ & $ i$\\
$ 55578.68921 $ & $   0.01205 $ & $   0.00101 $ & $  11.35720 $ & $ i$\\
$ 55578.69075 $ & $   0.00983 $ & $   0.00097 $ & $  11.35550 $ & $ i$\\
$ 55578.69228 $ & $   0.01193 $ & $   0.00099 $ & $  11.35670 $ & $ i$\\
$ 55578.69383 $ & $   0.01274 $ & $   0.00113 $ & $  11.35760 $ & $ i$\\
$ 55578.69504 $ & $   0.01155 $ & $   0.00113 $ & $  11.35620 $ & $ i$\\
$ 55578.69622 $ & $   0.01243 $ & $   0.00115 $ & $  11.35790 $ & $ i$\\
$ 55578.69742 $ & $   0.01049 $ & $   0.00114 $ & $  11.35540 $ & $ i$\\
$ 55578.69863 $ & $   0.00960 $ & $   0.00114 $ & $  11.35430 $ & $ i$\\


==> data/HTR364-003_rvtable.tex <==
$ 1466.12094 $ & $   -92.77 $ & $     2.40 $ & $    -7.06 $ & $     3.64 $ & $    0.129 $ & $   0.139 $ & Keck \\
$ 1468.11371 $ & $   111.39 $ & $     1.86 $ & $     4.37 $ & $     2.92 $ & $    0.129 $ & $   0.686 $ & Keck \\
$ 1468.12932 $ & \nodata      & \nodata      & $     0.45 $ & $     2.76 $ & $    0.129 $ & $   0.690 $ & Keck \\
$ 1470.12970 $ & $  -118.71 $ & $     2.72 $ & $     2.26 $ & $     2.07 $ & $    0.124 $ & $   0.239 $ & Keck \\
$ 1482.73469 $\tablenotemark{d} & $   106.37 $ & $    10.20 $ & $     7.70 $ & $     9.60 $ & \nodata      & $   0.695 $ & FIES \\
$ 1483.74899 $\tablenotemark{d} & $    39.07 $ & $    10.70 $ & $   -17.40 $ & $     6.50 $ & \nodata      & $   0.973 $ & FIES \\
$ 1486.74544 $\tablenotemark{d} & $    97.37 $ & $     8.50 $ & $     8.90 $ & $     8.30 $ & \nodata      & $   0.795 $ & FIES \\
$ 1488.74737 $\tablenotemark{d} & $  -152.93 $ & $    16.90 $ & $    24.70 $ & $    17.20 $ & \nodata      & $   0.344 $ & FIES \\
$ 1490.72460 $\tablenotemark{d} & $    78.27 $ & $     8.50 $ & $   -23.80 $ & $     6.40 $ & \nodata      & $   0.886 $ & FIES \\
$ 1501.03468 $ & $   117.01 $ & $     2.39 $ & $     9.98 $ & $     2.63 $ & $    0.127 $ & $   0.713 $ & Keck \\
$ 1523.09695 $ & $   126.39 $ & $     2.09 $ & $     0.65 $ & $     4.88 $ & $    0.134 $ & $   0.763 $ & Keck \\
$ 1529.15460 $ & $   -55.78 $ & $     2.32 $ & $   -11.07 $ & $     2.00 $ & $    0.129 $ & $   0.424 $ & Keck \\
$ 1545.14866 $ & $   103.29 $ & $     3.12 $ & $     9.13 $ & $     3.56 $ & $    0.125 $ & $   0.810 $ & Keck \\

